From Optimal Transport to Efficient Mechanisms for the $m$-Capacitated Facilities Location Problem with Bayesian Agent

In this paper, we study of the $m$-Capacitated Facility Location Problem ($m$-CFLP) on the line from a Bayesian Mechanism Design perspective and propose a novel class of mechanisms: the \textit{Extended Ranking Mechanisms} (ERMs). We first show that an ERM is truthful if and only if it satisfies a system of inequalities that depends on the capacities of the facilities we need to place. We then establish a connection between the $m$-CFLP and a norm minimization problem in the Wasserstein space, which enables us to show that if the number of agent goes to infinity the limit of the ratio between the expected Social Cost of an ERM and the expected optimal Social Cost is finite and characterize its value. Noticeably, our method generalizes to encompass other truthful mechanisms and other metrics, such as the $l_p$ and Maximum costs. We conclude our theoretical analysis by characterizing the optimal ERM tailored to a $m$-CFLP and a distribution $\mu$, that is the ERM whose limit Bayesian approximation ratio is the lowest compared to all other feasible ERMs. We consider mainly two frameworks: (i) in the first framework, the total facility capacity matches the number of agents, (ii) in the second framework, $m=2$. When we consider the Maximum Cost, we retrieve the optimal ERM for every $\mu$, while for the Social Cost, we characterize the solution when the measure $\mu$ is symmetric. Lastly, we numerically compare the performance of the ERMs against other truthful mechanisms and evaluate how quickly the Bayesian approximation ratio converges to its limit.

==> higherdimensionalERM.tex <==
\section{Extension to Higher Dimension}
\label{sec:higherdim}
% 
In this section, we study under which assumptions it is possible to adapt the ERM to define a mechanism capable of locating $m$ capacitated facilities in higher dimensional spaces.
% 
In this case, we denote with $x^{(i)}\in\erre^d$ the position of the $i$-th agent.
% 
We denote with $x^{(i)}_\ell$ the $\ell$-th coordinate of $x^{(i)}$.
% 
Given a p.c.v. $\vec q\in[0,1]^m$ and a permutation $\pi\in\mathcal{S}_m$, we denote with $y^{(j)}$ the position of the facility whose capacity is $q_{\pi(j)}$.
% 
We denote with $y^{(j)}_r$ the $r$-th coordinate of the location $y^{(j)}$.
% 
Lastly, we denote with $\Gamma\subset [n]\times [m]$ the agents-to-facility matching.
% 

\begin{mechanism}
    Let $\vec q\in[0,1]^m$ be a p.c.v. and $\pi\in\mathcal{S}_m$ be a permutation. 
    % 
    Given $d$ $m$-dimensional vectors $\vec v^{(j)}\in[0,1]^m$, the High-dimensional Extended Ranking Mechanism (HERM) associated with $\vec V=\{\vec v^{(j)}\}_{j\in[m]}$ is a mechanism whose routine is defined as follows
    \begin{enumerate}[label=(\roman*)]
        \item the mechanism gathers the reports of the $n$ agents, namely $\{x^{(i)}\}$.
        \item For every $l\in[d]$, it defines the vectors $\vec z^{(l)}$ containing the $l$-th coordinate of all the agents' reports.
        \item Then the mechanism defines the position of  $j$-th facility, namely $y^{(j)}$, by setting $y_i^{(j)}=z_{\floor{v_j^{(i)} (n-1)}+1}^{(i)}$. then it assigns to this location the capacity $q_{\pi(j)}$.
        \item Finally, every agent is assigned to the facility that is closer to the position they reported.
    \end{enumerate}
\end{mechanism}

Unlike what happens for the mechanisms used for the $m$-FLP, applying truthful $1$-dimensional mechanisms along each set of coordinates does not guarantee that the resulting mechanism is truthful.
% 
This is due to the fact that, in the $m$-CFLP, we need to place the facilities and also assign the agents to them.
% 
While the line has a total ordering over them, this is no longer true for higher dimensional spaces, as the next example shows.

\begin{example}
    Let us consider the following instance $q_1=q_2=0.7$, $n=20$, and $m=2$.
    % 
    Let us consider the vector $\vec v=(0.5,0.55)$.
    % 
    Notice that the ERM induced by $\vec v$ is truthful and well-defined.
    % 
    However, the HERM induced by $\vec V=\{\vec v,\vec v\}$ and $\pi=Id$ does not always return a feasible facility location.
    % 
    Consider for example the instance $\vec x ^{(1)}=\dots=\vec x^{(9)}=(-1,1.5)$, $\vec x^{(10)}=(0,1)$, $\vec x^{(11)}=(1,0)$, and $\vec x^{(12)}=\dots=\vec x^{(20)}=(1.5,-1)$.
    % 
    It is easy to check that the HERM induced by $\vec V$ places the facilities at $\vec y^{(1)}=(0,0)$ and $\vec y^{(2)}=(1,1)$, hence at least $18$ agents are closer to $\vec y^{(1)}$ than to $\vec y^{(2)}$.
    % 
    Finally, notice that both the capacities of the facilities are equal to $14$, thus the output of the HERM is not feasible, even though the ERM associated with $\vec v$ and $Id$ is feasible (see Theorem \ref{}).
    % 
    It is also worth of notice that the ERM induced by $\vec v$ coincides with the Innerpoint mechanism, proving that trivially extending one dimensional truthful mechanisms do not define a truthful and feasibile mechanism.
\end{example}

In what follows, we characterize the set of conditions under which the HERM are truthful.
% 
For the sake of simplicity, we consider only the case in which $d=2$, when $d>2$, the conditions are easy to generalize.
% 


\subsection{Case $m=2$}

First, we assume that we have to facilities to prove.
% 
In example \ref{}, we have shown that there are instances in which all the agents are closer to the same facility.
% 
The next theorem shows that this is always the case for HERM induced by $\vec V$ such that $v^{(1)}_1\neq v_1^{(2)}$ and $v^{(1)}_2\neq v^{(2)}_2$.
% 

\begin{theorem}
\label{thm:feasiblitycondhigherdim}
    Let $\vec q\in [0,1]^2$ a p.c.v. and let $\pi\in\mathcal{S}_m$ be a permutation.
    % 
    Then the HERM induced by $\vec V=\{\vec v^{(1)},\vec v^{(2)}\}$ and $\pi$ is feasible if and only if one of the following two holds
    % 
    \begin{itemize}
        \item $v_1^{(1)}=v_1^{(2)}$, $v_2^{(2)}\le q_{\pi(1)}$, and $1-v_2^{(1)}\le q_{\pi(2)}$; or
        \item $v_2^{(1)}=v_2^{(2)}$, $v_1^{(2)}\le q_{\pi(1)}$, and $1-v_1^{(1)}\le q_{\pi(2)}$.
    \end{itemize}
    % 
\end{theorem}

\begin{proof}
    blablabla
\end{proof}

% 
We now study the Bayesian approximation ratio of any feasible HERM.
% 
We recall that for higher dimensional problems, the cost
% 

\begin{theorem}
\label{thm:higherdimensionalSC}
    Given $\vec q\in[0,1]^2$, let $\pi\in\mathcal{S}_m$ and $\vec V$ induce a feasible HERM according to the conditions of Theorem \ref{thm:feasiblitycondhigherdim}.
    % 
    We denote with $\mu\in\PP(\erre^2)$ be a probability measure and let $\mu_1$ and $\mu$ be the marginal of $\mu$ with respect to the first and second variable, respectively.
    % 
    Then, we have that
    \begin{equation}
        \lim_{n\to\infty}\frac{\EE[\SCo_{(\pi,\vec V)}(\vec x)]}{\EE[\SCo_{opt}(\vec x)]}=\frac{W_1(\mu,\nu_{\vec V})}{W_1(\mu,\nu_2)},
    \end{equation}
    where $\nu_{\vec V}=\alpha\delta_{\vec y_1}+(1-\alpha)\delta_{\vec y^{(2)}}$ with $\vec y^{(i)}=(F_{\mu_1}^{[-1]}(\vec v_1^{(i)}),F_{\mu_2}^{[-1]}(\vec v_2^{(i)}))$, and 
    \[
        \alpha=\begin{cases}
                    F_{\mu_2}(\frac{y_2^{(1)}+y_2^{(2)}}{2}) \quad &\text{if } \quad v_1^{(1)}=v_1^{(2)}\\
                    F_{\mu_1}(\frac{y_1^{(1)}+y_1^{(2)}}{2}) \quad &\text{if } \quad v_2^{(1)}=v_2^{(2)}
                \end{cases}.
    \]
    While $\nu_2$ is the solution to $\min_{\sigma\in\mathcal{S}_2}\min_{\nu\in\PP_{2,\sigma}(\erre^2)}W_1(\mu,\nu)$.
    %
\end{theorem}

\begin{proof}
    sad
\end{proof}


Before we move to analyse the case in which we have more than $2$ facilities to place, we want to stress two points
\begin{enumerate}
    \item We can extend everything to other mechanisms that can places two capacitated facilities on a line.
    \item Theorem \ref{thm:higherdimensionalSC} is stated only for the Social Cost, however, following the arguments used in Section \ref{sect:extlpMC}, it is possible to extend the theorem to encompass the $l_p$ cost and the Maximum Cost. Again, notice that in order to have a bounded limit Bayesian approximation ratio, we need to assume that either
    \[
        \int_{\erre^d}|x|^pd\mu<+\infty
    \]
    or that the support of $\mu$ is compact.
\end{enumerate}


\subsection{Case $m>2$}




==> main.tex <==
% \documentclass[twoside,11pt]{article}
% \usepackage{jair, theapa, rawfonts}

% \jairheading{1}{1993}{1-15}{6/91}{9/91}
% \ShortHeadings{Minimizing Conflicts: A Heuristic Repair Method}
% {Minton, Philips, Johnston, \& Laird}
% \firstpageno{25}

% % Language setting
% % Replace `english' with e.g. `spanish' to change the document language
% \usepackage[english]{babel}

% % % Set page size and margins
% % % Replace `letterpaper' with `a4paper' for UK/EU standard size
% % \usepackage[letterpaper,top=2cm,bottom=2cm,left=3cm,right=3cm,marginparwidth=1.75cm]{geometry}

% \usepackage[utf8]{inputenc}
% \usepackage{amsmath}
% \usepackage{amsthm}
% \usepackage{multicol}
% \usepackage{amsmath}
% \usepackage{amsthm}
% \usepackage{amssymb}
% \usepackage[inline]{enumitem}
% \usepackage{algpseudocode} 
% \usepackage{algorithm}
% \usepackage[mathcal]{euscript}
% \usepackage[english]{babel}
% \usepackage{adjustbox}
% \usepackage[T1]{fontenc}
% % \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography
% \usepackage{tikz}
% \usetikzlibrary{positioning}
% \usepackage{graphicx}
% \usepackage[nottoc,notlot,notlof]{tocbibind}
% \usepackage{caption}
% \usepackage{subcaption}
% \usepackage{mathabx}

% % \usepackage{hyperref}
% \usepackage{multirow}

% \sloppy

% % \title{Example Article Title}

% % \author[1]{First Author}
% % \author[2]{Second Author}
% % \affil[1]{Address of first author}
% % \affil[2]{Address of second author}

% % \keywords{Keyword1, Keyword2, Keyword3}



% \newtheorem{theorem}{Theorem}
% \newtheorem{proposition}{Proposition}
% \newtheorem{corollary}{Corollary}
% \newtheorem{lemma}{Lemma}
% \newtheorem{remark}{Remark} 
% \newtheorem{prop}{Property}
% \newtheorem{problem}{Problem}
% \newtheorem{example}{Example}
% \newtheorem{definition}{Definition}

% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}





% \newcommand{\HRule}{\rule{.9\linewidth}{.6pt}}



% %%%%%%%%%%%%% INSIEMI %%%%%%%%%%%%%%%%

% \input{mathinput}




% \begin{document}

% \title{Minimizing Conflicts: A Heuristic Repair Method for
%        Constraint-Satisfaction and Scheduling Problems}

% \author{\name Steven Minton \email minton@ptolemy.arc.nasa.gov \\
%        \name Andy Philips \email philips@ptolemy.arc.nasa.gov \\
%        \addr NASA Ames Research Center, Mail Stop: 244-7,\\
%        Moffett Field, CA  94035 USA
%        \AND
%        \name Mark D. Johnston \email johnston@stsci.edu \\
%        \addr Space Telescope Science Institute,
%        3700 San Martin Drive,\\
%        Baltimore, MD 21218 USA
%        \AND
%        \name Philip Laird \email laird@ptolemy.arc.nasa.gov \\
%        \addr NASA Ames Research Center,
%        AI Research Branch, Mail Stop: 269-2,\\
%        Moffett Field, CA  94035 USA}

% % For research notes, remove the comment character in the line below.
% % \researchnote



% \maketitle

% \begin{abstract}
% In this paper, we initiate the study of the $m$-Capacitated Facility Location Problem ($m$-CFLP) within a Bayesian Mechanism Design framework. 
% % 
% We consider the case in which every agent's private information is their position on a line and assume that every agent's position is independently drawn from a common and known distribution $\mu$.
% % 
% In this context, we propose the Extended Ranking Mechanisms (ERMs), a truthful generalization of the recently introduced Ranking Mechanisms, that allows to handle problems where the total facility capacity exceeds the number of agents.
% % 
% Our primary results pertain to the study of the efficiency guarantees of the ERMs.
% % 
% In particular, we demonstrate that the limit of the ratio between the expected Social Cost of an ERM and the expected optimal Social Cost is finite.
% % 
% En route to these results, we reveal that the optimal Social Cost and the Social Cost of any ERMs can be expressed as the objective value of a suitable norm minimization problem in the Wasserstein space.
% % 
% We then tackle the problem of determining an optimal ERM tailored to a $m$-CFLP and a distribution $\mu$.
% % 
% Specifically, we aim to identify an ERM whose limit Bayesian approximation ratio is the lowest compared to all other ERMs.
% % 
% We detail how to retrieve an optimal ERM in two frameworks: \begin{enumerate*}[label=(\roman*)] \item when the total facility capacity matches the number of agents and \item when $\mu$ is the uniform distribution and we have two facilities to place.
% \end{enumerate*}
% % 
% Lastly, we conduct extensive numerical experiments to compare the performance of the ERMs against other truthful mechanisms and to evaluate the convergence speed of the Bayesian approximation ratio.
% % 
% In summary, all our findings highlight that a well-tuned ERM consistently outperforms all other known mechanisms, making it a valid choice for solving the $m$-CFLP within a Bayesian framework.
% \end{abstract}



% \section{Introduction}

% Mechanism Design seeks to establish protocols for aggregating the private information of a set of agents to optimize a global objective. 
%     % 
%     Nonetheless, optimizing a communal goal solely based on reported preferences frequently leads to undesirable manipulation driven by the agents' self-interested behaviour. 
%     % 
%     Hence, a key property that a mechanism should possess is \textit{truthfulness}, which ensures that no agent can gain an advantage by misrepresenting their private information. 
%     % 
%     Unfortunately, this stringent condition often clashes with the goal of optimizing the communal objective, leading to suboptimal outcomes from a truthful mechanism. 
%     % 
%     To quantify the efficiency loss entailed by a truthful mechanism, Nisan and Ronen introduced the concept of \textit{approximation ratio}, which represents the maximum ratio between the objective achieved by the truthful mechanism and the optimal objective attainable across all possible agents' reports \cite{nisan1999algorithmic}.
%     % 
%     A prominent problem in Mechanism Design is the $m$-Facility Location Problem ($m$-FLP) \cite{brandt2016handbook,chan2021mechanism}.
%     % 
%     In its fundamental guise, the $m$-FLP involves locating $m$ facilities amidst $n$ self-interested agents.
%     % 
%     Each agent requires access to a facility, making it preferable for a facility to be located as close as possible to their position. 
%     % 
%     Furthermore, each facility can accommodate any number of agents, thus the agents can select which facility to use devoid of any concern about possible overload.
%     % 
%     A natural extension of the $m$-FLP is the $m$-Capacitated Facility Location Problem ($m$-CFLP), in which every facility has a capacity limit.
%     % 
%     The capacity limit constraints the amount of agents that the facility can serve.
%     % 
%     In this case, the solution does not only elicit the positions of the facilities, but it also specifies to which facility every agent is assigned to, ensuring that no facility is overloaded.
%     % 
%     To the best of our knowledge, there are very few works that analyzed the Mechanism Design aspects of the $m$-CFLP.
%     % 
%     Moreover, all the existing results are conducted in the classic worst-case analysis, where the designer has no information on the agents and therefore aims to define mechanisms that work well on every possible input, regardless of the likelihood of the input. 
%     % 
%     This type of analysis is, however, too pessimistic and gives little insight into how to select a mechanism for a specific task.
%     % 
%     For example, there are currently no mechanisms capable of locating more than two capacitated facilities while achieving a finite approximation ratio.
% % 
%     Furthermore, even if we restrict our attention to the case where $m=2$, the approximation ratio of all the known truthful mechanisms depends linearly on the number of agents \cite{aziz2020facility}, making these efficiency guarantees less meaningful as the scale of the problem increases.
%     % 
%     In this paper, we overcome these issues by studying the $m$-CFLP from a Bayesian viewpoint.
%     % 
%     In Bayesian Mechanism Design, every agent's location is a random variable whose law is known to the designer \cite{hartline2010bayesian} thus the scope of the mechanism is not to minimize the cost in the worst possible case but rather to define truthful routines that work well in expectation.



% \subsection{Our Contribution}

% Our contribution is as follows: 
% \begin{enumerate}[leftmargin=*]
%     \item We define and study the Extended Ranking Mechanisms (ERMs), a generalization of the class of Ranking Mechanisms introduced in \cite{aziz2020facility}.
%     % 
%     Our extension allows to tackle a broader framework in which the combined capacity of the facilities surpasses the total amount of agents. 
%     % 
%     Moreover, a Ranking Mechanism is truthful if and only if it places all the facilities at, at most, two locations, while a ERM does not necessarily require such constraint to ensure truthfulness.
%     % 
%     See Section~\ref{sec:ERM}.
%     % 
%     \item We then delve into a Bayesian Framework to examine the asymptotic performances of the ERMs.
%     % 
%     We consider the case in which every agent's position is represented by a set of i.i.d. random variables.
%     % 
%     Our investigation reveals that $m$-CFLP is equivalent to a norm minimization problem over a subset of the Wasserstein space \cite{villani2009optimal}.
%     % 
%     By leveraging the properties of the Wasserstein distance, we then establish the convergence of the Bayesian approximation ratio, i.e., the ratio between the expected cost incurred by the mechanism and the expected optimal cost, as the number of agents tends toward infinity. 
%     % 
%     This is our primary result, as seen in Theorem \ref{thm:limitBAR}.
%     %  
%     We also compute this limit and show that it depends solely on the specifics of the problem, namely, the probability distribution $\mu$ describing the agents, the vector $\vec q$ determining the capacities of the facilities, and the characteristics of the mechanism.
%     % 
%     See Section \ref{sec:analysis}.
%     %
%     \item After that, we tackle the problem of identifying an optimal ERM tailored to the $m$-CFLP with agents distributed according to $\mu$ given the capacities determined by $\vec q$.
%     % 
%     First, we show that an optimal ERM always exists and characterize it as a solution to a minimization problem.
%     % 
%     Subsequently, we narrow our focus on two specific scenarios: \begin{enumerate*} [label=(\roman*)]
%         \item \textit{no-spare capacity} framework in which the total capacity of the facilities matches the total number of agents, and
%         \item the $2$-CFLP for a population of agents distributed according to a uniform distribution.
%     \end{enumerate*}
%     % 
%     See Section \ref{sec:para}.
%     %
%     \item Finally, we validate our findings through extensive numerical experiments in Section~\ref{sec:experiment}. 
%     % 
%     In particular, we compare the performances of the ERMs with the performances of other truthful mechanisms, such as the InnerGap Mechanism \cite{ijcai2022p75} and the Extended Endpoint Mechanism \cite{aziz2020facility}.
%     % 
%     From our experiments, we observe that a well-tuned ERM outperforms all the other mechanisms whenever $n\ge 20$.
%     % 
%     From these comparisons, we also observe that the limit Bayesian approximation ratio is a reliable estimation of the Bayesian approximation ratio of the ERM when the number of agents is greater than $20$.
% \end{enumerate}
% Our outcomes shed light on how to outline a mechanism depending on the problem, contributing to a better understanding of the strategic aspects of the $m$-CFLP in a Bayesian framework.
% % 
% % Due to space limits, all the missing proofs are deferred to Appendix \ref{app:missingproof}.
% % 
% % All the missing proofs and missing materials are available in the full version of the paper (see \url{https://arxiv.org/pdf/2312.16034.pdf}, \cite{auricchio2023extended}).


% \subsection{Related Work}

% The $m$-Facility Location Problem ($m$-FLP) and its variations are significant issues in various practical domains, such as disaster relief \cite{doi:10.1080/13675560701561789}, supply chain management \cite{MELO2009401}, healthcare \cite{ahmadi2017survey}, clustering \cite{hastie2009elements}, and public facilities accessibility \cite{barda1990multicriteria}.
% %
% Procaccia and Tennenholtz initially delved into the Mechanism Design study of the $m$-FLP, laying the groundwork for this field in their pioneering work \cite{procaccia2013approximate}.
% %
% Following that, a range of mechanisms with constant approximation ratios for placing one or two facilities on trees \cite{DBLP:conf/sigecom/FeldmanW13,DBLP:conf/atal/FilimonovM21}, circles \cite{DBLP:conf/sigecom/LuSWZ10,DBLP:conf/sigecom/LuSWZ10,DBLP:conf/wine/LuWZ09}, general graphs \cite{10.2307/40800845,DBLP:conf/sigecom/DokowFMN12}, and metric spaces \cite{DBLP:conf/sagt/Meir19,DBLP:conf/sigecom/TangYZ20} were introduced.
% % 
% Despite the generality of the underlying space, it is important to stress that all these positive results are confined to the case in which we have at most two facilities to place and/or the number of agents is limited.
% % 
% Moreover, different works tried to generalize the initial framework proposed in \cite{procaccia2013approximate}, by considering different agents' preferences \cite{church1978locating,MEI201846}, different costs \cite{feigenbaum2017approximately}, and additional constraints \cite{DBLP:conf/aaai/Filos-RatsikasL15,feldman2016voting}.
% % 

% % 
% In this paper, we analyze the $m$-Capacitated Facility Location Problem ($m$-CFLP), a variant of the $m$-FLP in which each facility can accommodate a finite number of agents.
% % 
% The Mechanism Design aspects of the $m$-CFLP have only recently begun to attract attention.
% %
% Indeed, the game theoretical framework for the $m$-CFLP that we consider was introduced in \cite{aziz2020facility}.
% %
% This work defined and studied various truthful mechanisms, like the InnerPoint Mechanism, the Extended Endpoint Mechanism, and the Ranking Mechanisms.
% %
% A more theoretical study of the problem was then presented in \cite{ijcai2022p75}, demonstrating that no mechanism can position more than two capacitated facilities while adhering to truthfulness, anonymity, and Pareto optimality.
% %
% Additionally, another paper dealing with Mechanism Design aspects of the $m$-CFLP is \cite{aziz2020capacity}.
% %
% However, it explores a different framework where only one facility needs to be placed and is unable to serve all agents.
% % 
% To the best of our knowledge, all the results on the $m$-CFLP concerned the classic Mechanism Design framework that evaluates the performances of the mechanism based on worst-case analysis. 
% % 
% In this paper, we consider an alternative approach: the Bayesian Mechanism Design perspective.
% % 
% Unlike traditional Mechanism Design, where the designer lacks information about agent types, in the Bayesian Mechanism Design framework each agent's type follows a known probability distribution \cite{hartline2013bayesian,chawla2014bayesian}.
% % 
% In this framework, we are able to determine a probability distribution over the set of all the possible inputs of the mechanism, enabling us to consider the expected cost of a mechanism.
% % 
% Bayesian Mechanism Design has been applied to investigate routing games \cite{gairing2005selfish}, facility location problems \cite{zampetakis2023bayesian}, combinatorial mechanisms using $\epsilon$-greedy mechanisms \cite{lucier2010price}, and, notably, auction mechanism design \cite{chawla2009sequential,chawla2007algorithmic,hartline2009simple,yan2011mechanism,ensthaler2014bayesian}.
% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{Preliminaries}
% \label{sec:preliminaries}

% % 
% In this section, we fix the notations on the $m$-CFLP, Bayesian Mechanism Design, and Optimal Transport (OT). 
% % 
% \paragraph{The \texorpdfstring{$m$}{m}-Capacitated Facility Location Problem.}

% Given a set of self-interested agents $[n]:=\{1,\dots,n\}$, we denote with $\vec x \in \erre^n$ the vector containing the agents' positions.
% % 
% Likewise, given $m\in\mathbb{N}$, we denote with $\vec c\in \mathbb{N}^m$ the vector containing the capacities of the facilities, namely $\vec c=(c_1,\dots,c_m)$.
% % 
% In this setting, a facility location is defined by three objects:
% \begin{enumerate*}[label=(\roman*)]
%     \item a $m$-dimensional vector $\vec y=(y_1,\dots,y_m)$ whose entries are $m$ positions on the line, 
%     \item a permutation $\pi\in\mathcal{S}_m$ that decides the capacity of the facility built at $y_j$, so that $c_{\pi(j)}$ is the capacity of the facility built at $y_j$, and
%     \item a matching $\Gamma\subset [n]\times [m]$ that determines how the agents are assigned to facilities, i.e. $(i,j)\in\Gamma$ if and only if the agent at $x_i$ is assigned to $y_j$. Due to the capacity constraints, the degree of vertex $j\in[m]$ according to $\Gamma$ is at most $c_{\pi(j)}$. Similarly, every agent is assigned to only one facility, thus the degree of every $i\in[n]$ according to $\Gamma$ is $1$.
% \end{enumerate*} 
% % 

% % 
% Given the positions of the facilities $\vec y$ and a matching $\Gamma$, we define the cost of an agent positioned in $x_i$ as $d_{i,\Gamma}(x_i,\vec y)=|x_i-y_j|$, where $(i,j)$ is the unique edge in $\Gamma$ adjacent to $i$.
% % 
% Given a matching $\Gamma$ and a permutation $\pi \in \mathcal{S}_m$, a cost function is a map $C_\Gamma:\erre^n\times \erre^m\to [0,+\infty)$ that associates to $(\vec x , \vec y)$ the overall cost of placing the facilities at the positions in $\vec y$ following the permutation $\pi$ and assigning the agents positioned at $\vec x$ according to $\Gamma$.\footnote{In what follows, we omit $\Gamma$ from the indexes of $d$ and $C$ when it is clear from the context which matching we are considering.}
% % 
% Given a vector $\vec x\in\erre^n$ containing the agents' positions, the $m$-\textit{Capacitated Facility Location Problem} with respect to the cost $C$, consists in finding the locations for $m$ facilities, a permutation $\pi$, and the matching $\Gamma$ that minimize the function $\vec y \to C(\vec x,\vec y)$.
% % 
% The most studied cost function is the \textit{Social Cost} ($\SCo$), which is defined as the sum of all the agents' costs.
% % 
% Since multiplying the cost function by a constant does not affect the approximation ratio results, throughout the paper we consider the Social Cost rescaled by the total number of agents, that is 
% \[
% \SCo(\vec x, \vec y)=\frac{1}{n}\sum_{i\in[n]}d_{i,\Gamma}(x_i,\vec y).
% \]
% % 
% Another important class of cost functions are the \textit{$l_p$ cost} which is defined as 
% \[
% C_{l_p}(\vec x, \vec y):=\Big(\frac{1}{n}\sum_{i=1}^{n}d_{i,\Gamma}(x_i,\vec y)^p\Big)^{\frac{1}{p}}
% \]
% and the \textit{Maximum Cost} which is defined as 
% \[
% \MCo(\vec x, \vec y):=\max_{i\in [n]}d_{i,\Gamma}(x_i,\vec y).
% \]




% \paragraph{Mechanism Design and the Worst-Case Analysis.}

% An \textit{$m$-facility location mechanism} is a function $f$ that takes the agents' reports $\vec x$ in input and returns a set of $m$ positions $\vec y$ on the line, a permutation $\pi\in\mathcal{S}_m$, and a matching $\Gamma$ to allocate the agents to the facilities. 
% % 
% In general, an agent may misreport its position if it would result in a set of facility locations such that the agent's incurred cost is smaller than reporting truthfully.
% % 
% A mechanism $f$ is said to be \textit{truthful} (or \textit{strategy-proof}) if, for every agent, its cost is minimized when it reports its true position. That is, $d_i(x_i,f(\vec x))\le d_i(x_i,f(\vec x_{-i},x_i'))$ for any misreport $x_i'\in \erre$, where $\vec x_{-i}$ is the vector $\vec x$ without its $i$-th component.
% % 
% Although deploying a truthful mechanism prevents agents from getting a benefit by misreporting their positions, this leads to a loss of efficiency.
% % 
% To evaluate this efficiency loss, Nisan and Ronen introduced the notion of approximation ratio \cite{nisan1999algorithmic}.
% % 
% Given a truthful mechanism $f$, its approximation ratio with respect to the Social Cost is defined as 
% %
% \begin{equation}
%     % \label{eq:worstcaseapproximationratio}
%     ar(f):=\sup_{\vec x \in \mathbb{R}^{n}}\frac{SC_{f}(\vec x)}{SC_{opt}(\vec x)},
% \end{equation}
% where $SC_f(\vec x)$ is the Social Cost of placing the facilities and assigning the agents to them following the output of $f$, while $SC_{opt}(\vec x)$ is the optimal Social Cost achievable when the agents' report is $\vec x$.
% % 
% The definition of the approximation ratio with respect to the $l_p$ cost or the Maximum Costs are defined similarly.
% % 

% % 
% The \textit{Ranking Mechanisms} are a class of mechanisms for the $m$-CFLP that work under the assumption that the total capacity of the facilities matches the number of agents, \cite{aziz2020facility}.
% % 
% Each Ranking Mechanism is defined by two parameters: a permutation $\pi\in\mathcal{S}_m$ and a vector $\vec t=(t_1,\dots,t_m)\in[n]^m$. 
% % 
% Given $\pi$ and $\vec t$ the routine of the Ranking Mechanism is as follows:
% \begin{enumerate*}[label=(\roman*)]
%     \item given $\vec x$ the vector containing the agents' reports ordered non-decreasingly, then the mechanism places the facility with capacity $c_{\pi(j)}$ at $x_{t_j}$.
%     \item The agents are assigned to the facility from left to right while respecting the capacity constraints.
% \end{enumerate*}
% % 
% It was shown in \cite{aziz2020facility} that a Ranking Mechanism is truthful if and only if every $t_j$ admits at most two different values.
% % 
% Moreover, the approximation ratio of these mechanisms is bounded only when the number of agents is even, the number of facilities to places is $2$, and the two facilities have the same capacity.
% % 
% In this case, the mechanism is also called InnerPoint Mechanism (IM) and its approximation ratio is $\frac{n}{2}-1$.




% \paragraph{Bayesian Mechanism Design.}
% %
% In Bayesian Mechanism Design, we assume that the agents' types follow a probability distribution and study the performance of mechanisms from a probabilistic viewpoint \cite{hartline2010bayesian,hartline2013bayesian}.
% % 
% Every agent's type is then described by a random variable $X_i$.
% % 
% In what follows, we assume that every $X_i$ is identically distributed according to a law $\mu$ and independent from the other random variables.
% % 
% A mechanism $f$ is said to be truthful if, for every agent $i$, it holds
% \begin{equation}
%     \EE_{\vec X_{-i}}[d_i(x_i,f(x_i,\vec X_{-i}))]\le \EE_{\vec X_{-i}}[d_i(x_i,f(x_i',\vec X_{-i}))] \quad\quad\quad \forall x_i\in\erre,
% \end{equation}
% where $x_i$ agent $i$'s true type, $\vec X_{-i}$ is the $(n-1)$-dimensional random vector that describes the other agents' type, and $\EE_{\vec X_{-i}}$ is the expectation with respect to the joint distribution of $\vec X_{-i}$.
% % 
% Given $\beta\in\erre$, a mechanism $f$ is a $\beta$-approximation if $\EE[SC_f(\vec X_n)]\le \beta\,\EE[SC_{opt}(\vec X_n)]$ holds, so that the lower $\beta$ is, the better the mechanism is.
% % 
% To unify the notation, we define the Bayesian approximation ratio for the Social Cost as the ratio between the expected Social Cost of a mechanism and the expected Social Cost of the optimal solution.
% % 
% More formally, given a mechanism $f$, its Bayesian approximation ratio with respect to the Social Cost is defined as follows 
% % 
% \begin{equation}
% \label{eq:B_ar}    
%     B_{ar,1}^{(n)}(f):=\frac{\EE[SC_f(\vec X_n)]}{\EE[SC_{opt}(\vec X_n)]},
% \end{equation}
% % 
% where the expected value is taken over the joint distribution of the vector $\vec X_n := (X_1,\dots,X_n)$.
% % 
% Notice that, if $B_{ar,1}^{(n)}(f)<+\infty$, then $f$ is a $B_{ar,1}^{(n)}(f)$-approximation.
% % 
% Similarly, we define the Bayesian approximation ratio of $f$ with respect to the Maximum Cost and the $l_p$-Costs.
% % 
% For the sake of consistency, we denote the Bayesian approximation ratio of $f$ with respect to the $l_p$ cost with $B_{ar,p}^{(n)}(f)$ and the Bayesian approximation ratio with respect to the Maximum Cost with $B_{ar,\infty}^{(n)}(f)$.
% % 
% Since we consider only truthful mechanisms, in what follows we use $\vec x$ to denote the vector containing the agents' reports and the agents' real position interchangeably.
% % 
% Moreover, we use the capital letter $\vec X_n$ to denote the random vector describing the agents' types.
% % 
% % % 
% % In Bayesian Mechanism Design, every agent's type is described by a random variable $X_i$.
% % % 
% % In what follows, we assume that every $X_i$ is identically distributed according to a law $\mu$ and independent from the other random variables.
% % % 
% % In this framework, a mechanism is truthful if, for every agent $i$, it holds
% % \begin{equation}
% %     \EE_{\vec X_{-i}}[d_i(x_i,f(x_i,\vec X_{-i}))]\le \EE_{\vec X_{-i}}[d_i(x_i,f(x_i',\vec X_{-i}))],\; \forall x_i\in\erre,
% % \end{equation}
% % where $x_i$ agent $i$'s true type, $\vec X_{-i}$ is the $(n-1)$-dimensional random vector that describes the other agents' type, and $\EE_{\vec X_{-i}}$ is the expectation with respect to the joint distribution of $\vec X_{-i}$.
% % % 
% % It is easy to see that if a mechanism is truthful in the classic Mechanism Design framework, it is also truthful in the Bayesian framework.
% % % 
% % Given $\beta\in\erre$, a mechanism $f$ is a $\beta$-approximation if it holds $\EE[SC_f(\vec X_n)]\le \beta\,\EE[SC_{opt}(\vec X_n)]$, where $\EE$ is the expectation with respect to the joint distribution of $\vec X_n$.
% % % 
% % Similarly to what happens for the approximation ratio, the lower $\beta$ is, the better the mechanism is.
% % % 
% % To unify the notation, we define the \textit{Bayesian approximation ratio} of a mechanism $f$ as the ratio between the expected Social Cost of a mechanism and the expected optimal Social Cost.
% % % 
% % More formally, given a mechanism $f$, its Bayesian approximation ratio with respect to the Social Cost is defined as follows 
% % % 
% % \begin{equation}
% % \label{eq:B_ar}    
% %     B_{ar}(f):=\frac{\EE[SC_f(\vec X_n)]}{\EE[SC_{opt}(\vec X_n)]},
% % \end{equation}
% % % 
% % where the expected value is taken over the joint distribution of the vector $\vec X_n := (X_1,\dots,X_n)$.
% % % 
% % Notice that, if $B_{ar}(f)<+\infty$, then $f$ is a $B_{ar}(f)$-approximation.
% % 
% % Since we consider only truthful mechanisms, in what follows we use $\vec x$ to denote the vector containing the agents' reports and the agents' real position interchangeably.
% % % 
% % In what follows, we use the capital letter $\vec X_n$ to denote the random vector describing the agents' types while the.
% % 


% \paragraph{Basic Notions on Optimal Transport.}
% % 
% In the following, we denote with $\PP(\erre)$ the set of probability measures over $\erre$. 
% % 
% Given a measure $\gamma\in\PP(\erre)$, we denote with $spt(\gamma)\subset \erre$ the support of $\gamma$, that is, the smallest closed set $C\subset \erre$ such that $\gamma(C)=1$.
% % 
% Furthermore, we denote with $\PP_k(\erre)$ the set of probability measures over $\erre$ whose support consists of $k$ points. 
% % 
% That is, $\nu\in\PP_k(\erre)$ if and only if $\nu=\sum_{j=1}^k \nu_j\delta_{x_j}$, where $x_j\in \erre$ for every $j\in [k]$, $\nu_j\ge 0$ are real values such that $\sum_{j=1}^k\nu_j=1$, and $\delta_{x_j}$ is the Dirac's delta centered in $x_j$.
% % 
% Given two measures $\alpha,\beta\in\PP(\erre)$ and $p\in [1,+\infty]$, the $p$-th order Wasserstein distance between $\alpha$ and $\beta$ is defined as 
% % 
% \begin{equation}
%     \label{eq:wass_p}
%     W_p^p(\alpha,\beta)=\min_{\pi\in\Pi(\alpha,\beta)}\int_{\erre\times \erre}|x-y|^pd\pi,
% \end{equation}
% where $\Pi(\alpha,\beta)$ is the set of probability measures over $\erre\times \erre$ whose first marginal is equal to $\alpha$ and the second marginal is equal to $\beta$ \cite{kantorovich2006translocation}.
% % 
% When $p=+\infty$, we set $W_\infty(\alpha,\beta)=\min_{\pi\in\Pi(\alpha,\beta)}\max_{(x,y)\in spt(\pi)} |x-y|.$
% % 
% It is well-known that, for every $p\in [1,\infty]$, $W_p$ is a metric over $\PP(\erre)$.
% % 
% For a complete introduction to the Optimal Transport theory, we refer the reader to \cite{villani2009optimal} and \cite{santambrogio2015optimal}.

% % \paragraph{The Wasserstein Distance.}

% % Let us denote with $\PP(\erre)$ the set of probability measures over $\erre$.
% % % 
% % Given $\gamma\in\PP(\erre)$, we denote with $spt(\gamma)\subset \erre$ the support of $\gamma$ and with $med(\gamma)$ the smallest median of $\gamma$.
% % % 
% % We denote with $\PP_m(\erre)$ the set of probability measures over $\erre$ whose support contains at most $m$ points, thus a measure $\nu\in\PP_m(\erre)$ is such that $\nu=\sum_{j=1}^m \nu_j\delta_{x_j}$, where $x_j\in \erre$ for all $j\in [m]$, $\nu_j$ are non-negative values satisfying $\sum_{j=1}^m\nu_j=1$, and $\delta_{x_j}$ is the Dirac delta measure centered at $x_j$.
% % % 
% % Given two measures $\alpha,\beta\in\PP(\erre)$, the Wasserstein distance between $\alpha$ and $\beta$ is defined as $W_1(\alpha,\beta)=\min_{\pi\in\Pi(\alpha,\beta)}\int_{\erre\times \erre}|x-y|d\pi,$
% % % 
% % % \begin{equation}
% % %     % \label{eq:wass_p}
% % %     W_1(\alpha,\beta)=\min_{\pi\in\Pi(\alpha,\beta)}\int_{\erre\times \erre}|x-y|d\pi,
% % % \end{equation}
% % where $\Pi(\alpha,\beta)$ is the set of probability measures over $\erre\times \erre$ whose first marginal is equal to $\alpha$ and the second marginal is equal to $\beta$ \cite{kantorovich2006translocation}.
% % % 
% % For a comprehensive introduction to Optimal Transport theory, we refer to \cite{villani2009optimal} and \cite{santambrogio2015optimal}.


% % \paragraph*{The Percentile Mechanisms.}

% % % 
% % The class of \textit{percentile mechanisms} has been introduced in \cite{sui2013analysis}. 
% % % 
% % Given a vector $\vec v=(v_1,v_2,\dots,v_k)$, such that $0\le v_1\le v_2\le \dots\le v_k\le 1$, the percentile mechanism induced by $\vec v$, namely $\PMp$, proceeds as follows:
% % % 
% % % \begin{enumerate*}[label=(\roman*)]
% % %     \item The mechanism designer collects all the reports of the agents, namely $\{x_1,x_2,\dots,x_n\}$.
% % %     % 
% % %     Without loss of generality, let us assume that the reports are already ordered in non-decreasing order, i.e. $x_i\le x_{i+1}$.
% % %     % 
% % %     \item The designer places the $k$ facilities at the positions $y_j=x_{i_j}$, where $i_j=\floor{(n-1)v_j}+1$.
% % % \end{enumerate*}
% % % 
% % Notice that, if the values $x_i$ are sampled from a distribution, the output of any percentile mechanism is composed by the $(\floor{(n-1)v_j}+1)$-th order statistics of the sample.
% % % 



% % As established in \cite{sui2013analysis}, percentile mechanisms are truthful if the cost of an agent placed at $x_i$ is $c_i=\min_{j\in [m]}|x_i-y_j|$, where $y_j$ are the position of the facilities. 
% % % 
% % Thus, when $k>2$, the approximation ratio of any percentile mechanism becomes unbounded regardless of the cost considered since the percentile mechanisms are also anonymous and deterministic.
% % %
% % In other words, for every percentile vector $\vec{v}$ and regardless of the objective function considered, $ar(\PMp) = +\infty$.
% % %
% % Moreover, it is worth noting that since percentile mechanisms are truthful in the classic setting, they also retain their truthfulness within the Bayesian framework \cite{hartline2013bayesian}.
% % %
% % Therefore, throughout this paper, there is no need to distinguish between the agents' types and their reported information.
% % % 

% % \section{The Bayesian Framework}

% % All the mechanisms considered so far either have an unbounded approximation ratio or its approximation ratio is not bounded with respect to the number of agents.
% % % 
% % In what follows, we study the performances of these mechanisms in a Bayesian Framework.
% % % 
% % In contrast with the classic worst case analysis, we show that all the ratio between the expected cost of each of the aforementioned mechanisms and the expected optimal cost is bounded and it converges to a constant value as the number of agents increases.


% \paragraph{Basic Assumptions.}
% % 
% Finally, we layout the basic assumptions of our framework.
% % 
% In what follows, we tacitly assume that the underlying distribution $\mu$ satisfies all the following properties:
% % 
% \begin{enumerate*}[label=(\roman*)]
% \item The measure $\mu$ is absolutely continuous. We denote with $\rho_\mu$ its density.
% \item The support of $\mu$ is an interval, which can be bounded or not, and that $\rho_\mu$ is strictly positive on the interior of the support.
% \item The density function  $\rho_\mu$ is differentiable on the support of $\mu$.
% \item The probability measure $\mu$ has finite first moment, i.e. $\int_\erre |x|d\mu < +\infty$.
% \end{enumerate*}
% % 
% Notice that, according to this set of assumptions, the cumulative distribution function (c.d.f.) of $\mu$, namely $F_\mu$, is locally bijective.
% % 
% % In particular, we have that its pseudo-inverse function, namely $F^{[-1]}_\mu$, is well-defined on $(0,1)$.
% % 

% \section{The Extended Ranking Mechanisms}
% \label{sec:ERM}

% % 
% Since our study aims to examine the behaviour of the mechanism as the number of agents goes to infinity, expressing the problem in terms of absolute capacities is unsuitable.
% % 
% For this reason, we need to rephrase the specifics of the $m$-CFLP in terms of percentages.
% % 
% In particular, instead of considering a collection of capacities $c_j\in\mathbb{N}$ for each $j\in [m]$, we shift our focus to the percentage capacity vector (p.c.v.) $\vec q\in(0,1)^m$.
% % 
% Each value $q_j$ corresponds to the percentage of agents that the $j$-th facility can accommodate.
% % 
% Given $\vec q$ and a number of agents $n$, we recover the absolute capacity of the $j$-th facility by setting $c_j=\floor{q_j(n-1)}+1$.
% % 
% Conversely, when we are given the absolute capacities $c_j$ for a given number of agents $n$, the corresponding p.c.v. is $q_j=\frac{c_j}{n}$.
% % 
% Without loss of generality, we assume that the entries of $\vec q$ are ordered non-increasingly.
% % 

% % {\color{teal} (M: I think it might be better to briefly introduce the classic ranking mechanism, such as its parameters, $\pi$ and $\vec{p}$, which would be useful for people like me who knew nothing about RM before to understand ERM.)}

% \begin{mechanism}[Extended Ranking Mechanisms (ERMs)]
%     Let $\vec q=(q_1,\dots,q_m)$ be a p.c.v..
%     % 
%     Given a permutation $\pi\in\mathcal{S}_m$ and an non-decreasingly ordered vector $\vec v=(p_1,\dots,p_m)\in [0,1]^m$, that is $p_j\le p_{j+1}$, the routine of the ERM associated with $\pi$ and $\vec v$, namely $\RM$, is as follows:
%     \begin{enumerate*}[label=(\roman*)]
%         \item First, we collect the reports of the agents and order them non-decreasingly. We denote with $\vec x$ the ordered vector containing the agents' reports, thus $x_i\le x_{i+1}$.
%         % 
%         \item Second, we elicit $m$ positions on the line by setting $y_j=x_{\floor{p_j(n-1)}+1}$ for every $j\in [m]$ and place the facility with capacity $q_{\pi(j)}$ at $y_j$.
%         \item Finally, we assign every agent to the facility closer to the position they reported (break ties arbitrarily without overloading the facilities).
%         \end{enumerate*}
% \end{mechanism}

% % 
% Notice that, in the routine of the ERM, the vector $\vec v$ plays the role that $\vec t$ plays in the routine of a Ranking Mechanism. 
% % 
% Indeed, the main difference between the Ranking Mechanisms and our generalization lies in how the mechanism matches the agents to the facilities.
% % 
% While the Ranking Mechanisms assign the agents monotonically from left to right, the ERM assigns every agent to the facility that is closer to their report.
% % 
% Depending on the pair $(\pi,\vec v)$ and $\vec q$, however, the matching returned by the ERM might overload some of the facilities.
% % 
% We say that a couple $(\pi,\vec v)$ induces a \textit{feasible} ERM if, for every $n\in\mathbb{N}$ and every $\vec x\in\erre^n$, the output of $\RM$ is a facility location for the $m$-CFLP induced by $\vec q$.
% % 
% Given a p.c.v. $\vec q$, the set of parameters $(\pi,\vec v)$ that induce a feasible ERM is characterizable through a system of inequalities.
% % 
% For the sake of simplicity, we first consider the case in which $\vec v$ does not have two equal entries, that is $p_j\neq p_l$ for every $j\neq l$.
% % 

% \begin{theorem}
% \label{thm:RM_feasible}
%     Given $\vec q$ and $\vec v$ such that $p_j\neq p_i$ for every $j\neq i\in[m]$, then $\RM$ is feasible if and only if the following system of inequalities are satisfied 
%     \begin{equation}
%     \label{eq:feas_system}
%     \begin{cases}
%         q_{\pi(1)}\ge p_2\\%-\frac{1}{n}\\
%         q_{\pi(2)}\ge p_3-p_1\\%-\frac{1}{n}\\
%         \quad\quad\vdots\\
%         q_{\pi(m-1)}\ge p_{m}-p_{m-2}\\%-\frac{1}{n}\\
%         q_{\pi(m)}\ge 1-p_{m-1}
%     \end{cases}.
% \end{equation}
% \end{theorem}
% % 

% \begin{proof}
% % [Proof of Theorem \ref{thm:RM_feasible}]
% % 
% Let $\vec x$ be the vector that contains the agents' reports ordered in a non-decreasing order.
% % 
% First, we show that every time the system \eqref{eq:feas_system} holds, then $\RM$ does not overload any facility.
% % 
% By definition of $\RM$, we have that every agent is assigned to its closest facility.
% % 
% Furthermore, every facility shares its position with an agent, depending on the vector $\vec v$. 
% % 
% Let us now focus the $j$-th facility, which, by definition, it is placed at $y_j=x_{\floor{p_j (n-1)}+1}$.
% % 
% Without loss of generality, let us assume that $1<j<m$, thus there are two facilities, namely $y_{j-1}$ and $y_{j+1}$, such that $y_{j-1} \le y_j\le y_{j+1}$.
% % 
% The maximum number of agents whose report is closer to $y_j$ is $\floor{p_{j+1}(n-1)}-\floor{p_{j-1}(n-1)}-1$.
% % 
% Since the capacity of the $j$-th facility is $\floor{q_{\pi(j)} (n-1)}+1$, we have that the facility at $y_j$ cannot be overloaded if and only if $\floor{q_{\pi(j)}(n-1)}+1\ge \floor{p_{j+1}(n-1)}-\floor{p_{j-1}(n-1)}-1$.
% % 
% We now show that the latter condition is implied by $q_{\pi(j)}\ge p_{j+1}-p_{j-1}$ or, equivalently, $q_{\pi(j)}(n-1)\ge (p_{j+1}-p_{j-1})(n-1)$.
% % 
% Indeed, it is easy to see that $\floor{q_{\pi(j)}(n-1)}+1\ge q_{\pi(j)}(n-1)\ge \floor{q_{\pi(j)}(n-1)}$, thus we have
% \begin{align*}
%     \floor{q_{\pi(j)}(n-1)}+1&\ge q_{\pi(j)}(n-1)\ge (p_{j+1}-p_{j-1})(n-1)\\
%     &\ge \floor{p_{j+1}(n-1)}-\floor{p_{j-1}(n-1)}-1.
% \end{align*}
% % 
% Through a similar argument, we deal with $y_1$ and $y_m$.
% % 

% % 
% We now show the inverse implication, i.e. if $(\pi,\vec v)$ satisfies system \eqref{thm:RM_feasible}, then $\RM$ is feasible.
% % 
% Toward a contradiction, assume that one of the inequalities does not holds.
% % 
% Without loss of generality, assume that $p_2>q_{\pi(1)}$, there then exists a value $N\in\mathbb{N}$ such that $p_2-\frac{2}{N-1}>q_{\pi(1)}$.
% % 
% Let us then consider $n=N$, then it holds $\floor{p_2(N-1)}-1>\floor{q_{\pi(1)}(N-1)}$, hence $\floor{p_2(N-1)}>\floor{q_{\pi(1)}(N-1)}+1$.
% % 
% Let us then consider the instance $\vec x\in\mathbb{R}^N$ defined as $x_i=0$ if $i=1,\dots,\floor{p_2(N-1)}$ and $x_i=1$ otherwise.
% % 
% On this instance $\RM$ place a facility at $y_1=0$ and all the others at $1$, the facility at $0$ has capacity $\floor{q_{\pi(1)}(N-1)}+1$.
% % 
% By definition, the number of agents whose closest facility is $y_1$ is $\floor{p_2(N-1)}>\floor{q_{\pi(1)}(N-1)}+1$, which contradicts the feasibility of the mechanism.
% \end{proof}

% % 
% The feasibility of the ERM ensures also its truthfulness.
% % 

% \begin{theorem}
% \label{thm:truthfulness}
%     Given a p.c.v. $\vec q$, any feasible $\RM$  is truthful. 
%     % 
%     Thus it is also truthful in the Bayesian framework.
% \end{theorem}

% \begin{proof}
% % [Proof of Theorem \ref{thm:truthfulness}]
%     Let $\vec q$ be a p.c.v. and let $\RM$ be a feasible ERM.
%     % 
%     Toward a contradiction, let $\vec x$ be an instance in which an agent is able to manipulate.
%     % 
%     Without loss of generality, let us assume that the manipulative agent's real position is $x_i$.
%     % 
%     Since every agent is assigned to the facility that is closer to the position they report, the manipulation performed by the agent at $x_i$ must alter the position of the facilities, as otherwise the cost of the manipulative agent cannot decrease.
%     % 
%     We notice that the positions of the facilities are determined through the same routine of the Percentile mechanisms, \cite{sui2013analysis}.
%     % 
%     Owing to the truthfulness of the Percentile mechanisms for the $m$-FLP, we infer that no agent can misreport in such a way that a facility gets closer to its position, which concludes the proof.
% \end{proof}



% The truthfulness of any ERM is bound to the fact that every facility $y_j$ can accommodate all the agents between $y_{j-1}$ and $y_{j+1}$.
% % 
% This constraint limits the set of $\vec{p}$ for which there exists a $\pi \in \mathcal{S}_m$ such that $\RM$ is feasible.
% % 


% \begin{corollary}
% \label{crr:sparecapacity}
%     Given a p.c.v. $\vec q\in(0,1)^m$, let us fix $\vec v\in[0,1]^m$.
%     % 
%     Then, if $(\max_{j\in[m]}p_j-\min_{j\in[m]}p_j)>\sum_{j\in[m]}q_j-1$, the mechanism $\RM$ is not feasible for every $\pi\in\mathcal{S}_m$.
% \end{corollary}


% \begin{proof}
%     % [Proof of Corollary \ref{crr:sparecapacity}]
%     It follows from Theorem \ref{thm:RM_feasible}, indeed if $\RM$ is feasible, then \eqref{eq:feas_system} holds.
%     % 
%     If we sum all the inequalities of system \eqref{eq:feas_system}, we get
%     \begin{align*}
%         \sum_{j\in[m]}q_{\pi(j)}=\sum_{j\in[m]}q_j&\ge p_2+(p_3-p_1)+\dots+(p_m-p_{m-2})+(1-p_{m-1})\\
%         &=1+p_m-p_1,
%     \end{align*}
%     since $\vec v$ is ordered increasingly.
%     % 
%     Thus, if 
%     \[
%     p_m-p_1=\big(\max_{j\in[m]}p_j-\min_{j\in[m]}p_j\big)>\sum_{j\in[m]}q_j-1
%     \]
%     holds, system \eqref{eq:feas_system} does not, which concludes the proof.
% \end{proof}


% Finally, we notice that if $\vec v$ has at least two equal entries, not all the feasible ERMs necessarily satisfy system \eqref{eq:feas_system}.
% % 
% For example, the \texttt{all-median} mechanism that places all the facilities at the median agent is always feasible and truthful.
% % 
% Notice that, in this case, we do not need to specify which agent is served by which facility nor $\pi\in\mathcal{S}_m$, since all the agents and all the facilities are served/located at the same place.
% % 
% However, depending on $\vec q$, the vector $\vec v=(0.5,\dots,0.5)$ may not satisfy system \eqref{eq:feas_system} for any $\pi\in\mathcal{S}_m$.
% % 
% Indeed, if $p_j=p_l$ for some indices $j,l\in [m]$, we need to consider all the facilities placed at $x_{\floor{p(n-1)}+1}$ as if they were a unique facility whose capacity is the total capacity of the facilities placed at $x_{\floor{p(n-1)}+1}$.
% % 
% By doing so, we are able to extend Theorem \ref{thm:RM_feasible} and \ref{thm:truthfulness} to the case in which $\vec v$ has at least two equal entries.
% % 
% In particular, given $\vec v\in[0,1]^m$, let $\vec v'\in [0,1]^{m'}$ be the vector containing all the different entries of $\vec v$, then, the mechanism $\texttt{ERM}^{(\pi,\vec v)}$ is feasible if and only if the following system is satisfied
% \[
% \begin{cases}
%         \sum_{l\in[m];\;s.t.\;p_{\pi(l)}=p_1'}q_{\pi(l)}\ge p_2'\\%-\frac{1}{n}\\
%         \sum_{l\in[m];\;s.t.\;p_{\pi(l)}=p_2'}q_{\pi(l)}\ge p_3'-p_1'\\%-\frac{1}{n}\\
%         \quad\quad\vdots\\
%         \sum_{l\in[m];\;s.t.\;p_{\pi(l)}=p_{m-1}'}q_{\pi(l)}\ge p_{m'}'-p_{m'-2}'\\%-\frac{1}{n}\\
%         \sum_{l\in[m];\;s.t.\;p_{\pi(l)}=p_{m'}'}q_{\pi(l)}\ge 1-p_{m'-1}'
% \end{cases}.
% \]


% % 
% Notice that Theorem \ref{thm:RM_feasible}, \ref{thm:truthfulness}, and Corollary \ref{crr:sparecapacity} hold regardless of the objective we are seeking to minimise, that is the Social Cost, the $l_p$ costs, and the Maximum Cost.
% % 
% Lastly, we notice that, except in a few specific cases, the approximation ratio of the Ranking Mechanisms is unbounded.
% % 
% Consequentially, it is impossible to retrieve a bound on the approximation ratio of any ERM for generic $m$-CFLPs.
% % 
% Since the classic worst-case analysis does not give any insight into the performances of the ERMs, we move our attention to the Bayesian analysis.
% % 

% \section{The Bayesian Analysis of the ERMs}
% \label{sec:analysis}
% % 
% In this section, we present our main result, which characterizes the limit of the Bayesian approximation ratio of any feasible ERM as a function of $\vec v$, $\pi$, $\mu$, and $\vec q$.
% % 
% For the sake of exposition, we first study the limit Bayesian approximation ratio of the ERMS with respect to the Social Cost.
% % 
% Indeed, we show that all our techniques can be extended to include both the $l_p$ costs and the Maximum costs.
% % 
% As a preliminary lemma, we relate the $m$-CFLP to a norm minimization problem in the Wasserstein Space.
% % 

% \begin{lemma}
% \label{lemma:equivalenceSC_W1}
%     Given a p.c.v. $\vec q$, let $\vec x\in\erre^n$ be the vector containing the agents' reports.
%     % 
%     Let us fix $\mu_{\vec x}:=\frac{1}{n}\sum_{i\in [n]}\delta_{x_i}$. 
%     % 
%     Then, it holds
%     \begin{equation}
%     \label{eq:min_discreteopt}
%       SC_{opt}(\vec x)=\min_{\sigma\in\mathcal{S}_m}\min_{\zeta\in\PP_{\sigma,\vec q}(\erre)}W_1(\mu_n,\zeta),  
%     \end{equation}
%     where $\PP_{\sigma,\vec q}(\erre)$ is the set of probability measures such that $\zeta=\sum_{j\in[m]}\zeta_j\delta_{y_j}$, where $y_1\le y_2\le\dots\le y_m$ and $\zeta_j\le q_{\sigma(j)}$ for every $j\in[m]$.
%     % 
%     Similarly, given a permutation $\pi\in\mathcal{S}_m$ and a vector $\vec v$ that induce a feasible ERM, it holds 
%     \begin{equation}
%     \label{eq:discrete_proj2}
%     SC_{\pi,\vec v}(\vec x)=\min_{\lambda_j\le q_{\pi(j)},\sum_{j\in[m]\lambda_j=1}}W_1(\mu_n,\lambda),
%     \end{equation}
%     where $SC_{\pi,\vec v}(\vec x)$ is the Social Cost attained by $\RM$ on instance $\vec x$, $\lambda=\sum_{j\in[m]}\lambda_j\delta_{x_{r_j}}$, and $r_j=\floor{p_j(n-1)}+1$.
% \end{lemma}

% \begin{proof}
% % [Proof of Lemma \ref{lemma:equivalenceSC_W1}]
%     First, we show that \eqref{eq:min_proj} holds.
%     % 
%     Given $\vec x$ and $\vec q$, let us consider an optimal solution to the $m$-CFLP.
%     % 
%     In particular, we denote with $\vec y$ be the vector containing $m$ positions on the line, $\sigma$ the permutation that determines how to distribute the facilities among the positions in $\vec y$, and $\Gamma$ a matching that assigns every agent to a facility without overloading the facilities.
%     % 
%     Let us now consider the following transportation plan
%     \[
%     \pi_{x_i,y_j}=\begin{cases}
%         \frac{1}{n}\quad \text{if}\quad (i,j)\in\Gamma,\\
%         0\quad\text{otherwise.}
%     \end{cases}
%     \]
%     By definition of $\Gamma$, we have that $\sum_{j\in[m]}\pi_{x_i,y_j}=\frac{1}{n}$ and 
%     \[
%     \sum_{i\in[n]}\pi_{x_i,y_j}=\frac{k_j}{n}\le\frac{c_{\sigma(j)}}{n}=q_{\sigma(j)},
%     \]
%     where $k_j$ is the degree of $j\in[m]$ according to $\Gamma$.
%     % 
%     Thus, if we set $\nu_{n,m}=\sum_{j\in[m]}\frac{k_j}{n}\delta_{y_j}$, we have that $\nu_{n,m}\in\PP_{\sigma,m}(\erre)$.
%     % 
%     It is easy to see that $SC(\vec x)=\sum_{i\in[n],j\in [m]}|x_i-y_j|\pi_{x_i,y_j}\ge W_1(\mu_n,\nu_{n,m})$, hence
%     \[
%     SC_{opt}(\vec x)\ge \min_{\sigma\in\mathcal{S}_m}\min_{\zeta\in\PP_{\sigma,m}(\erre)} W_1(\mu_n,\zeta).
%     \]
%     To conclude, we show that the inverse inequality holds.
%     % 
    
    
%     % 
%     Let $(\sigma,\nu_{m,n})$ be a minimizer of the right hand side of \eqref{eq:discrete_proj2}, we show that there exists a set of $m$ locations $\vec y$, a permutation $\sigma'$, and a matching $\Gamma$ whose Social Cost is $W_1(\mu_n,\nu_{n,m})$.
%     % 
%     First, let us set $\vec y=(y_1,\dots,y_m)$, where $\{y_j\}_{j\in [m]}$ is the support of $\nu_{m,n}$.
%     % 
%     Without loss of generality, we assume that $q_j=\frac{c_j}{n}$, thus there exists an optimal transportation plan $\pi$ between $\mu_n$ and $\nu_{m,n}$ such that for every $i\in[n]$, there exists a unique $j\in[m]$ such that $\pi_{x_i,y_j}\neq 0$, see \cite{auricchio2022structure}.
%     % 
%     Notice that, by definition of transportation plan, if $\pi_{x_i,y_j}\neq 0$ for only a couple of values $i\in[n]$, $j\in[m]$, then $\pi_{x_i,y_j}=\frac{1}{n}$.
%     % 
%     Thus, the set $\Gamma=\{(i,j)\in [n]\times [m];\; \pi_{x_i,y_j}=\frac{1}{n}\}$ is well defined.
%     % 
%     Since for every $i\in[n]$ we have that there exists a unique $j\in[m]$ for which it holds $\pi_{x_i,y_j}=\frac{1}{n}$, we have that the degree of every $i\in[n]$ is one.
%     % 
%     Since $\sum_{i\in[n]}\pi_{x_i,y_j}=(\nu_{m,n})_j\le \frac{c_{\sigma(j)}}{n}$, we have that the degree of every $j\in[m]$ is less than $c_{\sigma(j)}$.
%     % 
%     Thus the triplet $(\vec y,\sigma,\Gamma)$ is a feasible location for the $m$-CFLP.
%     % 
%     Since the Social Cost of $(\vec y,\sigma,\mu)$ is equal to $\sum_{i\in[n],j\in[m]}|x_i-y_j|\pi_{x_i,y_j}=W_1(\mu_n,\nu_{m,n})$, we have that
%     \[
%     \min_{\sigma\in\mathcal{S}_m}\min_{\zeta\in\PP_{\sigma,m}(\erre)} W_1(\mu_n,\zeta)=W_1(\mu_n,\nu_{m,n})\ge SC_{opt}(\vec x),
%     \]
%     which concludes the proof.
%     % 

%     % 
%     Notice that, since $\min_{\sigma\in\mathcal{S}_m}\min_{\zeta\in\PP_{\sigma,m}(\erre)} W_1(\mu_n,\zeta)= SC_{opt}(\vec x)$ holds, we can refine the previous argument and show that, given an optimal facility location for the $m$-CFLP it is possible to build a solution to the minimization problem in the right hand side of \eqref{eq:min_discreteopt}.
%     % 
%     Vice-versa, given a solution to the minimization problem in the right hand side of \eqref{eq:min_discreteopt}, it is possible to build an optimal facility location for the $m$-CFLP.
%     % 

%     % 
%     Using the same argument and the same constructions, it is possible to show that \eqref{eq:discrete_proj2} holds.
%     % 
% \end{proof}


% % 
% The proof of Lemma \ref{lemma:equivalenceSC_W1} consists in showing that, for any given instance $\vec x$ and given an optimal facility location for the $m$-CFLP, it is possible to construct a measure $\nu$ such that $W_1(\mu_n,\nu)=SC_{opt}(\vec x)$ and, vice-versa, given a measure $\nu$ that minimizes \eqref{eq:min_discreteopt}, it is possible to retrieve an optimal facility location problem for the $m$-CFLP.
% % 
% Since the $m$-CFLP admits a solution, problem \eqref{eq:min_discreteopt} is well-posed and admits a solution.
% % 
% By a similar argument, we infer the same conclusions for problem \eqref{eq:discrete_proj2}.
% % 
% % Lemma \ref{lemma:equivalenceSC_W1} establishes a link between the $m$-CFLP and Optimal Transport theory.
% % 
% The connection between the $m$-CFLP and Optimal Transport theory highlighted in Lemma \ref{lemma:equivalenceSC_W1} enables us to exploit the properties of the Wasserstein distances and to characterize the limit Bayesian approximation ratio of every feasible ERM.
% % 

% % 

% % 



% \begin{theorem}
% \label{thm:limitBAR}
%     Given the p.c.v. $\vec q$, let $\vec v\in (0,1)^m$ and $\pi\in\mathcal{S}_m$ be such that $\RM$ is feasible.
%     % 
%     Then, it holds
%     \begin{equation}
%     \label{eq:bayesianlimitRM}
%         \lim_{n\to +\infty}\frac{\EE[SC_{\pi,\vec v}(\vec x)]}{\EE[SC_{opt}(\vec x)]}=\frac{W_1(\mu,\nu_{\vec v})}{W_1(\mu,\nu_{m})},
%     \end{equation}
%     % 
%     where $\nu_{m}$ is a solution to the following minimization problem
%     \begin{equation}
%     \label{eq:min_proj}
%       \min_{\sigma\in \mathcal{S}_m}\min_{\zeta\in\PP_{\sigma,\vec q}(\erre)}W_1(\mu,\zeta),
%     \end{equation}
%     and $\nu_{\vec v}$ is a solution to 
%     \begin{equation}
%     \label{eq:min_proj2}
%       \min_{\lambda_j\le q_{\pi(j)},\sum_{j\in[m]}\lambda_j=1}W_1\Big(\mu,\sum_{j\in[m]}\lambda_j\delta_{F_\mu^{[-1]}(p_j)}\Big).
%     \end{equation}
% \end{theorem}

% % \begin{proof}[Proof of Theorem \ref{thm:limitBAR}]
% %     To complete the proof of Theorem \ref{thm:limitBAR}, we need to prove the following:
% %     \begin{enumerate*}[label=(\roman*)]
% %         \item First, we need to show that a solution $\nu_m$ to problem \eqref{eq:min_proj} always exists. This would complete the proof of the first step.
% %         \item We need to show that there always exists a solution $\nu_{\vec v}$ to problem \eqref{eq:min_proj2}, and
% %         \item we need to show that $\lim_{n\to\infty}\EE[W_1(\nu_{\vec x, \vec v},\phi)]\to 0$ when $n\to \infty$. 
% %     \end{enumerate*}

% % \textbf{(i) Existence of a solution $\nu_m$.} 

% % \textbf{(ii) Existence of a solution $\nu_{\vec v}$.}


% % \textbf{(iii) Convergence of $\EE [W_1(\nu_{\vec x, \vec v},\phi)]$.}

% % \end{proof}

% \begin{proof}
%     The proof consists of three steps:
%     \begin{enumerate*}[label=(\roman*)]
%         \item First, we show that the expected optimal Social Cost for the $m$-CFLP converges to the objective value of the minimization problem in \eqref{eq:min_proj}.
%         % 
%         \item Second, we show that the expected Social Cost of $\RM$ converges to the objective value of the minimization problem in \eqref{eq:min_proj2}.
%         % 
%         \item We combine the two convergence results to retrieve \eqref{eq:bayesianlimitRM}.
%     \end{enumerate*}

%     \textbf{The limit of the expected optimal Social Cost.}
%     % 
%     First, we show that a solution to problem \eqref{eq:min_proj} always exists.
%     % 
%     For every $m$ the number of permutation is finite, thus it suffices to show that, for every $\sigma\in\mathcal{S}_m$ there exists a solution to the problem
%     \[
%     \min_{\zeta\in\PP_{\sigma,m}(\erre)}W_1(\mu,\zeta).
%     \]
%     Since $\mu$ has finite first moment, i.e. $\int_\erre |x|d\mu<+\infty$, the minimization problem is well-posed and its minimum is finite.
%     % 
%     Moreover, the set $\PP_{\sigma,m}(\erre)$ is a closed set in $\PP(\erre)$, thus a solution to the minimization problem does exist (although it may not be unique).
%     % 
%     Let $\nu_{m}$ be such that $W_1(\mu,\nu_{m})=\min_{\sigma\in \mathcal{S}_m}\min_{\zeta\in\PP_{\sigma,\vec q}(\erre)}W_1(\mu,\zeta)$.
%     % \[
%     % W_1(\mu,\nu_{m})=\min_{\sigma\in \mathcal{S}_m}\min_{\zeta\in\PP_{\sigma,\vec q}(\erre)}W_1(\mu,\zeta).
%     % \]
%     % 
%     From Lemma \ref{lemma:equivalenceSC_W1}, we know that, for every $n\in\mathbb{N}$ and for every  $\vec x\in\erre^n$, there exists a $\nu_{\vec x,m}$ such that $SC_{opt}(\vec x)=W_1(\mu_n,\nu_{\vec x,m})$.
%     % 
%     By definition of $\nu_{m}$, we have that $W_1(\mu,\nu_{m})\le W_1(\mu,\nu_{\vec x,m})$.
%     % 
%     Since $W_1$ is a distance, it holds $W_1(\mu,\nu_{m})\le W_1(\mu,\nu_{\vec x,m})\le W_1(\mu,\mu_n)+W_1(\mu_n,\nu_{\vec x,m})$.
%     % 
%     By rearranging the terms and by taking the expected value with respect to the distribution of $\vec X$, we obtain $\EE [W_1(\mu,\nu_{m})]-\EE [W_1(\mu_n,\nu_{\vec x,m})]\le \EE [W_1(\mu,\mu_n)]$. 
%     % \[
%     % \EE [W_1(\mu,\nu_{m})]-\EE [W_1(\mu_n,\nu_{\vec x,m})]\le \EE [W_1(\mu,\mu_n)].
%     % \]
%     By a similar argument, we have that $W_1(\mu_n,\nu_{\vec x,m})\le W_1(\mu_n,\nu_m)\le W_1(\mu,\mu_n)+W_1(\mu,\nu_m)$, hence $\EE [W_1(\mu_n,\nu_{\vec x,m})]-\EE[W_1(\mu,\nu_{m})]\le \EE [W_1(\mu,\mu_n)]$.
%     % \[
%     % \EE [W_1(\mu_n,\nu_{\vec x,m})]-\EE [W_1(\mu,\nu_{m})]\le \EE [W_1(\mu,\mu_n)].
%     % \]
%     We then infer that 
%     \[
%     |\EE[W_1(\mu,\nu_{m})]-\EE[W_1(\mu_n,\nu_{\vec x,m})]|\le \EE[W_1(\mu,\mu_n)].
%     \]
%     Since the right handside of this inequality converges to $0$ as $n$ goes to $+\infty$ (see \cite{bobkov2019one}), we infer that $ \lim_{n\to\infty}\EE [W_1(\mu_n,\nu_{\vec x,m})]=W_1(\mu,\nu_{m})$,
%     % \[
%     % \lim_{n\to\infty}\EE [W_1(\mu_n,\nu_{\vec x,m})]=W_1(\mu,\nu_{m}),
%     % \]
%     which concludes the first part of the proof.

%     \textbf{The limit of the expected Social Cost of the Mechanism.}
%     First, we retrieve a minimizer to problem \eqref{eq:min_proj2}.
%     % 
%     Given $\vec v$, let us set $y_j=F_\mu^{[-1]}(p_j)$.
%     % 
%     For every $\lambda=\sum_{j\in[m]}\lambda_j\delta_{y_j}$ such that $\sum_{j\in[m]}\lambda_j=1$, we have that
%     \[
%     W_1(\mu,\lambda)=\sum_{j\in[m]}\int_{F_\mu^{[-1]}\big(\sum_{l=1}^{j-1}\lambda_l\big)}^{F_\mu^{[-1]}\big(\sum_{l=1}^{j}\lambda_l\big)}|x-y_j|d\mu\ge \int_{\erre}\min_{j\in[m]}|x-y_j|d\mu.
%     \]
%     % 
%     % 
%     Let us now consider the measure
%     \[
%     \lambda_{min}=\sum_{j\in[m]}\Big(F_\mu(z_j)-F_\mu(z_{j-1})\Big)\delta_{y_j},
%     \]
%     where $z_j=\frac{y_{j+1}+y_j}{2}$ if $j=2,\dots, m-1$, $z_0=-\infty$ and $z_m=+\infty$.
%     % 
%     We then have
%     \begin{align*}
%         W_1(\mu,\lambda_{min})&=\sum_{j\in[m]}\int_{F_\mu^{[-1]}\big(\sum_{l=1}^{j-1}F_\mu(z_l)-F_\mu(z_{l-1})\big)}^{F_\mu^{[-1]}\big(\sum_{l=1}^{j}F_\mu(z_l)-F_\mu(z_{l-1})\big)}|x-y_j|d\mu\\
%         &=\sum_{j\in[m]}\int_{z_{j-1}}^{z_j}|x-y_j|d\mu\\
%         &=\int_{\erre}\min_{j\in[m]}|x-y_j|d\mu.
%     \end{align*}
%     Thus $\lambda_{min}$ is a minimizer.
%     % 
    
%     % 
%     We now study the limit of the expected Social Cost of the mechanism.
%     % 
%     The argument used for this part is similar to the one used for the limit expected optimal Social Cost but more delicate.
%     % 
%     Indeed, in this case, the set on which we minimize the Wasserstein distance does depend on the agents' report $\vec x$.
%     % 
%     In particular, the sets on which are formulated problem \eqref{eq:min_proj2} and \eqref{eq:discrete_proj2} are, in general, different.
%     %
%     To overcome this issue, we need to define two auxiliary probability measures, namely $\phi$ and $\psi$.
%     % 
%     Given $\vec x\in\erre^n$, let $\nu_{\vec v}$ and $\nu_{\vec x, \vec v}$ be the solutions to problem \eqref{eq:min_proj2} and \eqref{eq:discrete_proj2}, respectively.
%     % 
%     We define the measures $\phi=\sum_{j\in[m]}(\nu_{\vec x, \vec v})_j\delta_{y_j}$, where $y_j$ is the support of the measure $\nu_{\vec v}$.
%     % 
%     For every $n\in\mathbb{N}$ and every $\vec x\in \erre^n$, we have that $W_1(\mu,\nu_{\vec v})\le W_1(\mu,\phi)\le W_1(\mu,\mu_n)+W_1(\mu_n,\nu_{\vec x, \vec v})+W_1(\nu_{\vec x, \vec v},\phi).$
%     % \begin{align*}
%     %     W_1(\mu,\nu_{\vec v})&\le W_1(\mu,\phi)\le W_1(\mu,\mu_n)+W_1(\mu_n,\nu_{\vec x, \vec v})+W_1(\nu_{\vec x, \vec v},\phi).
%     % \end{align*}
%     We therefore infer
%     \begin{equation}
%         \label{eq:inequality_1}
%          W_1(\mu,\nu_{\vec v})-W_1(\mu_n,\nu_{\vec x, \vec v})\le W_1(\mu,\mu_n)+W_1(\nu_{\vec x, \vec v},\phi).
%     \end{equation}
% % 
%     Similarly, given $\vec x\in\erre^n$, we define $\psi=\sum_{j\in[m]}(\nu_{\vec v})_j\delta_{y_{\vec x,j}}$, where $\{y_{\vec x,j}\}_{j\in[m]}$ is the support of $\nu_{\vec x, \vec v}$.
%     % 
%     We then have
%     \begin{equation}
%         \label{eq:inequality_2}
%          W_1(\mu_n,\nu_{\vec x, \vec v})-W_1(\mu,\nu_{\vec v})\le W_1(\mu,\mu_n)+W_1(\nu_{\vec v},\psi).
%     \end{equation}
   
%     Since the Wasserstein distance is always non negative, we can combine the estimations in \eqref{eq:inequality_1} and \eqref{eq:inequality_2}, to obtain
%     \[
%     |W_1(\mu_n,\nu_{\vec x, \vec v})-W_1(\mu,\nu_{\vec v})|\le W_1(\mu,\mu_n)+W_1(\nu_{\vec v},\psi)+W_1(\nu_{\vec x, \vec v},\phi).
%     \]
%     If we take the expectation of both sides of the inequality the inequality still holds.
%     % 
%     Thus, if we show that $\lim_{n\to\infty}\EE [W_1(\nu_{\vec v},\psi)]=\lim_{n\to\infty}\EE [W_1(\nu_{\vec x, \vec v},\phi)]=0$, we conclude this second step of the proof since, by \cite{bobkov2019one}, we have that $\lim_{n\to\infty}\EE [W_1(\mu_n,\mu)]=0$.
%     % 
%     Let us consider $\EE [W_1(\nu_{\vec v},\psi)]$, the convergence of $\EE [W_1(\nu_{\vec x, \vec v},\phi)]$ follows by a similar argument.
%     % 
%     We notice that $\psi$ and $\nu_{\vec v}$ have different supports, but $\psi_j=(\nu_{\vec v})_j$, thus it holds $\EE [W_1(\nu_{\vec v},\psi)]\le \sum_{j\in[m]}\psi_j\EE [|y_j-y_{\vec x,j}|]$, where $y_{\vec x,j}$ is the $j$-th point in the support of $\nu_{\vec x, \vec v}$.
%     % 
%     By definition of ERM, it holds $y_{\vec x,j}=x_{\floor{p_j(n-1)}+1}$.
%     % 
%     Since the $\big(\floor{p_j(n-1)}+1\big)$-th order statistics converges to the $p_j$-th quantile of $\mu$ \cite{kiefer1967bahadur,de1979bahadur}, we have that $\EE [|y_j-y_{\vec x,j}|]\to 0$ as $n\to \infty$.
%     % 
%     Indeed, we have that 
%     \[
%     \phi=\sum_{j\in[m]}(\nu_{\vec x, \vec v})_j\delta_{y_j}.
%     \]
%     Since $(\nu_{\vec x, \vec v})_j\le 1$ for every $j\in[m]$, we infer
%     \[
%     \EE[W_1(\nu_{\vec x, \vec v},\phi)]\le \sum_{j\in[m]}\EE[|y_{\vec x,j}-y_j|],
%     \]
%     where $y_{\vec x,j}=x_{\floor{p_j(n-1)}+1}$ and $y_j=F_\mu^{[-1]}(p_j)$.
%     % 
%     Using Bahadur's representation formula (see \cite{10.1214/aoms/1177699450} and \cite{de1979bahadur}), we have that
%     \begin{equation}
%         \label{eq:bahadur}
%         X_{\floor{(n-1)p_j}+1}-F_\mu^{[-1]}(p_j)=\frac{S_n(F_\mu^{[-1]}(p_j))-p_j}{\rho_\mu(F_\mu^{[-1]}(p_j))}+R_n,
%     \end{equation}
%     where $R_n$ is the rest of the Bahadur's formula, for which holds $R_n\le O(n^{-\frac{3}{4}})$ with probability $1$, $\rho_\mu$ is the density of $\mu$, and $S_n(t)=\frac{1}{n}\sum_{i=1}^n \mathbb{I}(X_i)_{\{X_i\le t\}}$ where 
%     \[
%     \mathbb{I}(X_i)_{\{X_i\le t\}}=\begin{cases}
%         1 \quad \text{if}\quad X_i\le t,\\
%         0 \quad \text{otherwise.}    
%     \end{cases}
%     \]
%     Since by hypothesis the density of $\mu$ is always strictly positive on the interior of the support of $\mu$ and $p_j\in (0,1)$ for every $j=1,\dots,m$, we have
%     \begin{align*}
%         \EE[|y_{\vec x,j}-y_j|]&\le K \EE\big[|S_n(F_\mu^{[-1]}(p_j))-p_j|\big]+\EE[|R_n|]\\
%         &\le K\EE\bigg[\frac{1}{n}|\sum_{i=1}^n(\mathbb{I}(X_i)_{\{X_i\le F_\mu^{[-1]}(p_j)\}}-p_j)|\bigg]+ Cn^{-\frac{3}{4}}\\
%         &\le K\EE\Big[\Big|\sum_{i=1}^n\frac{(\mathbb{I}(X_i)_{\{X_i\le F_\mu^{[-1]}(p_j)\}})-p_j)}{n}\Big|\Big]+ Cn^{-\frac{3}{4}}\\
%         % &\le \frac{K}{n}\Big(\EE[\sum_{i=1}^n|\mathbb{I}(X_i)_{\{X_i\le F_\mu^{[-1]}(p_j)\}}-p_j|^2]\Big)^{\frac{1}{2}}+ Cn^{-\frac{3}{4}}\\
%         &\le \frac{K}{\sqrt{n}}Var(\mathbb{I}(X_1)_{\{X_1\le F_\mu^{[-1]}(p_j)\}})+ Cn^{-\frac{3}{4}},
%     \end{align*}
%     since the $X_i$ are i.i.d. and $\mathbb{I}_{\{X_i\le F_\mu^{[-1]}(p_j)\}}(X_i)$ is a Bernoulli variable that with probability $p_j$ is equal to $1$ and equal to $0$ otherwise hence its variance is finite.
%     % 
%     We then conclude that $\EE [W_1(\nu_{\vec x, \vec v},\phi)]$ converges to $0$.
%     % 
%     Similarly, it is possible to show that $\EE [W_1(\nu_{\vec v},\psi)]$ converges to $0$.

    
%     \textbf{Characterizing the Bayesian approximation ratio.}
%     % 
%     To conclude, notice that the distance between an absolutely continuous measure and a discrete measure is always greater than zero, thus $\lim_{n\to\infty}\EE [SC_{opt}(\vec X)]>0$.
%     % 
%     For this reason, we have that the limit of the ratio is equal to the ratio of the limits, which proves \eqref{eq:bayesianlimitRM}.
%     % \[
%     % \lim_{n\to\infty}\frac{\EE [SC_{RM^{(\pi,\vec v)}}(\vec X)]}{\EE [SC_{opt}(\vec X)]}=\frac{\min_{\lambda_j\le c_{\pi(j)}}W_1(\mu_n,\lambda)}{\min_{\sigma\in \mathcal{S}_m}\min_{\zeta\in\PP_{\sigma,\vec q}(\erre)}W_1(\mu,\zeta)},
%     % \]
%     % where $\lambda=\sum_{j\in[m]}\lambda_j\delta_{F_\mu^{[-1]}(p_j)}$, which concludes the proof.
%     %
% \end{proof}

% Notice that our result applies only to feasible $\RM$, such that $\vec v\in(0,1)^m$, since, for general measures $\mu$, the values $F_\mu^{[-1]}(0)$ and $F_\mu^{[-1]}(1)$ might not be finite.
% % 
% %{\color{red} In App. \ref{app:C}, we use Theorem \ref{thm:limitBAR} to study the limit Bayesian approximation ratio of other mechanisms.}
% % 
% % {\color{red} Moreover, in Appendix \ref{app:C}, we show that Theorem \ref{thm:limitBAR} allows to study the limit Bayesian approximation ratio of other mechanisms, such as the InnerPoint Mechanism or the Ranking Mechanisms.}
% % 
% % 
% Finally, we notice that the Bayesian approximation ratio is invariant to positive affine transformation of $\mu$.
% % 
% In particular, the limit of the Bayesian approximation ratio remains the same across all the Gaussian-distributed populations.
% % 

% \begin{corollary}
% \label{crr:scale_invariance}
%     Let $\vec q$ be a p.c.v. and let $X$ be the random variable associated with $\mu$.
%     % 
%     Given $\alpha>0$ and $\beta\in\erre$, let $\mu_{\alpha,\beta}$ be the probability distribution associated with $\alpha X +\beta$.
%     % 
%     Then, the asymptotical Bayesian approximation ratio of any feasible ERM is the same regardless of whether the agent type is distributed according to $\mu$ or $\mu_{\alpha,\beta}$.
% \end{corollary}

% \begin{proof}
% % [Proof of Corollary \ref{crr:scale_invariance}] 
%     Let $\nu_m$ be the solution to \eqref{eq:min_proj} and let $\nu^{(\alpha,\beta)}_m$ be the solution to
%     \[
%     \min_{\sigma\in\mathcal{S}_m}\min_{\zeta\in\PP_{\sigma,m}(\erre)}W_1(\mu_{\alpha,\beta},\zeta)
%     \]
%     Let us fix $L(x)=\alpha x +\beta$.
%     % 
%     Since $\alpha>0$, $L$ is a bijective and monotone-increasing function.
%     % 
%     We denote the inverse function of $L$ with $H$.
%     % 
%     It is well-known that if $X$ is a random variable whose law is $\mu$, then the law of $L(X)=\alpha X+\beta$ is $L_\#\mu$.
%     % 
%     We recall that $L_\#\mu$ is the pushforward of the measure $\mu$, defined as $L_\#\mu(A)=\mu(H(A))$, see \cite{villani2009optimal}.
%     % 
%     By definition, we have that $L_\#\delta_{x}=\delta_{\alpha x + \beta}$, thus $L_\#(\sum_{j\in [m]}\lambda_j\delta_{x_j})=\sum_{j\in [m]}\lambda_j\delta_{\alpha x_j + \beta}$.
%     % 
%     We now show that $\nu^{(\alpha,\beta)}_m=L_\#\nu_m$.
%     % 
%     First, notice that, since $\alpha>0$ the function $L$ is monotone increasing, thus if $\nu_m\in\PP_{\sigma,m}(\erre)$, then $L_\#\nu_m\in\PP_{\sigma,m}(\erre)$.
%     % 
%     Toward a contradiction, let us now assume that $\gamma$ is such that
%     \[
%         W_1(\gamma,L_\#\mu)<W_1(L_\# \nu_m,L_\#\mu).
%     \]
%     Let us now define $\eta=H_\#\gamma\in\PP_k(\erre)$.
%     % 
%     Since $H$ is also monotone increasing, we have $\gamma\in\PP_{\sigma,m}(\erre)$ and $\gamma=L_\#\eta$.
%     % 
%     Furthermore, by the properties of the Wasserstein distance, we have
%     \begin{equation}
%     \label{eq:scalingWopt}
%         W_1(L_\#\eta,L_\#\mu)=\alpha W_1(\eta,\mu)
%     \end{equation}
%     and 
%     \[
%         W_1(L_\#\nu_m,L_\#\mu)=\alpha W_1(\nu_m,\mu).
%     \]
%     In particular, we get
%     \[
%         W_1(\eta,\mu)<W_1(\nu_m,\mu),
%     \]
%     which contradicts the optimality of $\nu_m$.
%     % 
%     We therefore conclude that $L_\#\nu_m=\nu^{(\alpha,\beta)}_m$ and that 
%     \[
%         W_1(\nu^{(\alpha,\beta)}_m\mu_{\alpha,\beta})=\alpha W_1(\nu_m,\mu).
%     \]
%     To conclude, we observe that
%     \begin{align*}
%             \min_{\lambda_j\le q_{\sigma(j)},\sum_{j\in [m]}\lambda_j=1}&W_1\Big(\mu_{\alpha,\beta},\sum_{j\in[m]}\lambda_j\delta_{\alpha y_j+\beta}\Big) = \alpha\min_{\lambda_j\le q_{\sigma(j)},\sum_{j\in [m]}\lambda_j=1}W_1\Big(\mu,\sum_{j\in[m]}\lambda_j\delta_{y_j}\Big),
%     \end{align*}
%     for any set of $m$ values $\{y_j\}_{j\in[m]}$.
%     % 
%     We then observe that $F^{[-1]}_{\mu_{\alpha,\beta}}(p_j)=\alpha F^{[-1]}_{\mu}(p_j) +\beta$, thus
%     \begin{align*}
%         &\min_{\lambda_j\le q_{\sigma(j)},\sum_{j\in [m]}\lambda_j=1}W_1\Big(\mu_{\alpha,\beta},\sum_{j\in[m]}\lambda_j\delta_{\alpha F^{[-1]}_{\mu}(p_j)+\beta}\Big)\\
%         &\quad\quad=\min_{\lambda_j\le q_{\sigma(j)},\sum_{j\in [m]}\lambda_j=1}W_1\Big(\mu_{\alpha,\beta},\sum_{j\in[m]}\lambda_j\delta_{F^{[-1]}_{\mu_{\alpha,\beta}}(p_j)}\Big).
%     \end{align*}
    
%     % 
%     Finally, we notice that by taking the ratio of the two expectations, the factor $\alpha$ evens out.
%     % 
%     Thus the limit of the Bayesian approximation ratio of any ERM does not depend on the values of $\alpha$ nor $\beta$.
% \end{proof}


% \subsection{Extending to the \texorpdfstring{$l_p$}{lp} costs and the Maximum Cost}
% \label{sect:extlpMC}

% In this section, we study under which set of additional conditions it is possible to extend Theorem \ref{thm:limitBAR} to include the $l_p$ costs and the Maximum Cost.
% % 
% First, we show that the optimal $l_p$ and Maximum costs can be phrased as a projection problems with respect to a suitable Wasserstein distance.

% \begin{lemma}
% \label{lemma:equivalenceSC_lpmc}
%     Given a p.c.v. $\vec q$, let $\vec x\in\erre^n$ be the vector containing the agents' reports.
%     % 
%     Let us fix $\mu_{\vec x}:=\frac{1}{n}\sum_{i\in [n]}\delta_{x_i}$. 
%     % 
%     Then, it holds
%     \begin{equation}
%     \label{eq:min_discreteoptlp}
%       (C_{l_p})_{opt}(\vec x)=\min_{\sigma\in\mathcal{S}_m,\zeta\in\PP_{\sigma,\vec q}(\erre)}W_p(\mu_n,\zeta)\quad\quad\text{and}\quad\quad \MCo_{opt}(\vec x)=\min_{\sigma\in\mathcal{S}_m,\zeta\in\PP_{\sigma,\vec q}(\erre)}W_\infty(\mu_n,\zeta),  
%     \end{equation}
%     where $\PP_{\sigma,\vec q}(\erre)$ is the set of probability measures such that $\zeta=\sum_{j\in[m]}\zeta_j\delta_{y_j}$, where $y_1\le y_2\le\dots\le y_m$ and $\zeta_j\le q_{\sigma(j)}$ for every $j\in[m]$.
%     % 
%     Similarly, given a permutation $\pi\in\mathcal{S}_m$ and a vector $\vec v$ that induce a feasible ERM, it holds 
%     \begin{equation}
%     \label{eq:discrete_proj2lp}
%     (C_{l_p})_{\pi,\vec v}(\vec x)=\min_{\lambda_j\le q_{\pi(j)},\sum_{j\in[m]\lambda_j=1}}W_p(\mu_n,\lambda)\quad\quad\text{and}\quad\quad \MCo_{\pi,\vec v}(\vec x)=\min_{\lambda_j\le q_{\pi(j)},\sum_{j\in[m]\lambda_j=1}}W_\infty(\mu_n,\lambda), 
%     \end{equation}
%     where $SC_{\pi,\vec v}(\vec x)$ is the Social Cost attained by $\RM$ on instance $\vec x$, $\lambda=\sum_{j\in[m]}\lambda_j\delta_{x_{r_j}}$, and $r_j=\floor{p_j(n-1)}+1$.
% \end{lemma}

% \begin{proof}
%     The proof of the Lemma follows the same argument used to prove Lemma \ref{lemma:equivalenceSC_W1}.
%     % 
%     Indeed, the construction of solution to the projection problem and the solution to the $m$-CFLP do not depend on the Social Cost.
% \end{proof}

% % 
% Since Lemma \ref{lemma:equivalenceSC_W1} extends to the $l_p$ costs and the Maximum Cost, we can adapt the argument used to prove Theorem \ref{thm:limitBAR}.
% % 
% Notice, however, that the condition under which the convergence happens and the argument used for these two cost functions, slightly change from
% % 

% \begin{theorem}
% \label{thm:limitBAR_p_MC}
%     Given the p.c.v. $\vec q$, let $\vec v\in (0,1)^m$ and $\pi\in\mathcal{S}_m$ be such that $\RM$ is feasible.
%     % 
%     Given $p>1$, then if $\int_{\erre}|x|^p d\mu<+\infty$ holds, we have
%     \begin{equation}
%     \label{eq:bayesianlimitRMlp}
%         \lim_{n\to +\infty}\frac{\EE[(C_{l_p})_{\pi,\vec v}(\vec x)]}{\EE[(C_{l_p})_{opt}(\vec x)]}=\frac{W_p(\mu,\nu_{\vec v})}{W_p(\mu,\nu_{m})},
%     \end{equation}
%     % 
%     where $\nu_{m}$ is a solution to $\min_{\sigma\in \mathcal{S}_m}\min_{\zeta\in\PP_{\sigma,\vec q}(\erre)}W_p(\mu,\zeta)$, while $\nu_{\vec v}$ is a solution to $\min_{\lambda_j\le q_{\pi(j)},\sum_{j\in[m]}\lambda_j=1}W_p\Big(\mu,\sum_{j\in[m]}\lambda_j\delta_{F_\mu^{[-1]}(p_j)}\Big)$.
%     % 

%     % 
%     Similarly, if $\mu$ has a compact support, then we have that 
%     \begin{equation}
%     \label{eq:bayesianlimitRMmc}
%         \lim_{n\to +\infty}\frac{\EE[\MCo_{\pi,\vec v}(\vec x)]}{\EE[\MCo_{opt}(\vec x)]}=\frac{W_\infty(\mu,\nu_{\vec v})}{W_\infty(\mu,\nu_{m})},
%     \end{equation}
%     where $\nu_{m}$ is a solution to $\min_{\sigma\in \mathcal{S}_m}\min_{\zeta\in\PP_{\sigma,\vec q}(\erre)}W_\infty(\mu,\zeta)$, while $\nu_{\vec v}$ is a solution to $\min_{\lambda_j\le q_{\pi(j)},\sum_{j\in[m]}\lambda_j=1}W_\infty\Big(\mu,\sum_{j\in[m]}\lambda_j\delta_{F_\mu^{[-1]}(p_j)}\Big)$.
% \end{theorem}

% \begin{proof}
%     First, we notice that condition $\int_{\erre}|x|^pd\mu<+\infty$, ensures that $\min_{\nu\in\PP_k(\erre)}W_p(\mu,\nu)<+\infty$.
%     % 
%     Similarly, if $\mu$ has compact support to ensure that $\min W_\infty(\mu,)$ is finite.
%     % 
%     In particular, the right-handside of the limits in \eqref{eq:bayesianlimitRMlp} and \eqref{eq:bayesianlimitRMmc} are well-defined.
%     % 

%     % 
%     To prove this theorem, we show that both the numerator and the denominator of the Bayesian approximation ratio do converge as the number of agents goes to infinity.
%     % 
%     The convergence of the denominator of the Bayesian approximation ratio, that is the convergence of the expected optimal cost, follows from the same argument used in the proof of Theorem \ref{thm:limitBAR}.
%     % 
%     The argument used to prove the convergence of the numerator is slightly different.
%     % 
%     In what follows, we denote with $W_p$ the Wasserstein distance associated with $p\in(1,+\infty]$.
%     % 
%     Using the metric properties of $W_p$, we retrieve 
%     \[
%         |W_p(\mu_n,\nu_{\vec x, \vec v})-W_p(\mu,\nu_{\vec v})|\le W_p(\mu,\mu_n)+W_p(\nu_{\vec v},\psi)+W_p(\nu_{\vec x, \vec v},\phi),
%     \]
%     where 
%     \begin{enumerate*}[label=(\roman*)]
%         \item $\nu_{\vec v}=\sum_{j\in[m]}(\nu_{\vec v})_j\delta_{y_{j}}$ is the solution to problem $\min_{\lambda_j\le q_{\pi(j)},\sum_{j\in[m]}\lambda_j=1}W_p\Big(\mu,\sum_{j\in[m]}\lambda_j\delta_{F_\mu^{[-1]}(p_j)}\Big)$,
%         \item $\nu_{\vec x, \vec v}=\sum_{j\in[m]}(\nu_{\vec v})_{\vec x,j}\delta_{y_{\vec x,j}}$ is the solution to problem \eqref{eq:discrete_proj2lp},
%         \item $\psi=\sum_{j\in[m]}(\nu_{\vec v})_j\delta_{y_{\vec x,j}}$, where $\{y_{\vec x,j}\}_{j\in[m]}$ is the support $\nu_{\vec x, \vec v}$, and
%         \item $\phi=\sum_{j\in[m]}(\nu_{\vec x, \vec v})_j\delta_{y_j}$.
%     \end{enumerate*}
%     % 

%     % 
%     Owing to the assumption on $\mu$ and to the results in \cite{bobkov2019one}, we have that $\lim_{n\to\infty}W_p(\mu,\mu_n)=0$.
%     % 
%     We now handle $W_p^p(\nu_{\vec v},\psi)$.
%     % 
%     If $p<\infty$, we have that
%     \begin{align*}
%         \EE[W_p(\nu_{\vec v},\psi)]&\le\EE\Big[\Big(\sum_{j\in[m]}(\nu_{\vec v})_j|y_j-y_{\vec x,j}|^p\Big)^{\frac{1}{p}}\Big]\le \EE\Big[\Big(\sum_{j\in[m]}|y_j-y_{\vec x,j}|^p\Big)^{\frac{1}{p}}\Big]\\
%         & \le \EE\Big[\Big(\big(\sum_{j\in[m]}|y_j-y_{\vec x,j}|\big)^p\Big)^{\frac{1}{p}}\Big]=\EE\Big[\sum_{j\in[m]}|y_j-y_{\vec x,j}|\Big]\\
%         &\le \sum_{j\in[m]}\EE\Big[|y_j-y_{\vec x,j}|\Big].
%     \end{align*}
%     We can then apply the argument use into the proof of Theorem \ref{thm:limitBAR} to conclude that $\lim_{n\to\infty}\EE[W_p(\nu_{\vec v},\psi)]=0$.
%     % 

%     % 
%     If $p=\infty$, we notice that
%     \[
%        \EE[W_\infty(\nu_{\vec v},\psi)]=\EE[\max_{j\in[m]}|y_j-y_{\vec x,j}|]\le \EE\Big[\sum_{j\in[m]}|y_j-y_{\vec x,j}|\Big] \le \sum_{j\in[m]}\EE[|y_j-y_{\vec x,j}|],
%     \]
%     which allows us to conclude the proof for the case $p=\infty$.
    
%     % 
%     Similarly, we have that $W_p(\nu_{\vec x, \vec v},\phi)$ goes to $0$ as the number of agent increases, which concludes the proof.
%     % 
% \end{proof}

% % 
% We close the section by showing that the result presented in Theorem \ref{thm:limitBAR} and \ref{thm:limitBAR_p_MC} are applicable to the study of the Innerpoint and the Extended Endpoint Mechanisms.
% % 
% For the sake of simplicity, we limit our study to the Bayesian approximation ratio of the Social Cost, since the other costs are handled through a similar argument.
% % 
% We omit the study of the InnerGap Mechanism as it is a specific instance of the ERM.

% \subsection{The Bayesian approximation ratio of the Innerpoint Mechanism}
% \label{ex:im}
%     Consider now the $2$-CFLP in which we have an even number of agents, thus $n=2k$, and the two facilities have the same capacity, so that $\vec q=(0.5,0.5)$.
%     % 
%     In this context, the Innerpoint Mechanism (IM) places the two facilities at $y_1$ and $y_2$, where $y_1$ is the $k$-th agent report from the left and $y_2$ the $(k+1)$-th agent report from the left.
%     % 
%     Every agent whose report is on the left of $y_1$ is assigned to the facility at $y_1$, while the others to $y_2$. 
%     % 
%     Since the IM works only for instances with an even number of agents, the limit will taken for $k\to \infty$.
%     % 
%     It is easy to see that, for every given $k\in \mathbb{N}$, the IM can be written as a Ranking Mechanism.
%     % 
%     Indeed, if we set $\vec v=(0.5-\frac{1}{2k},0.5)$ and $\pi=Id$ (where $Id(i)=i$ for every $i\in [2]$), the output of the IM and the output of the ERM associated to $\vec v$ and $\pi$ coincide on every instance.
%     % 
%     However, the vector $\vec v$ determining the output of the ERM depends on $k$, thus we cannot directly apply Theorem \ref{thm:limitBAR} to infer the limit Bayesian approximation ratio of the IM.
%     % 
%     To overcome this issue, we consider the Ranking Mechanism induced by the vector $\vec v=(0.5,0.5)$.
%     % 
%     Since the two facilities have the same capacity the mechanism does not depend on the permutation we choose, thus we will omit it for the sake of simplicity.
%     % 
%     Indeed, for every $k\in\mathbb{N}$ and $\vec x\in\erre^{2k}$, it holds $SC_{IM}(\vec x)\le SC_{RM^{(Id,\vec v)}}(\vec x)$, hence
%     \begin{align}
%     \label{eq:inequalitybound}
%         \lim_{k\to\infty}\frac{\EE [SC_{IM}(\vec X)]}{\EE [SC_{opt}(\vec X)]}&\le\lim_{n\to\infty}\frac{\EE [SC_{Id,\vec v}(\vec X)]}{\EE [SC_{opt}(\vec X)]}=\frac{W_1(\mu,\delta_{med(\mu)})}{W_1(\mu,\nu_{m})},
%     \end{align}
%     where $\nu_{m}$ is a solution to problem \eqref{eq:min_proj}.
%     % 
%     Notice the inequality in \eqref{eq:inequalitybound} allows us to conclude that the Bayesian approximation ratio of the IM is finite.
%     % 
%     We now prove the other inequality.
%     % 
%     Notice that if $k>10$ and $\epsilon\in(0,0.1)$, it holds true the following 
%     \[
%     SC_{IM}(\vec x)\ge SC_{\texttt{ERM}^{(Id,\vec v_\epsilon)}}(\vec x),
%     \]
%     where $\vec v_{\epsilon}=(0.5-\epsilon,0.5)$.
%     % 
%     Notice that the mechanism $\texttt{ERM}^{(Id,\vec v_\epsilon)}$ is not feasible for $\vec q=(0.5,0.5)$, but it is feasible if we consider $\vec q_\epsilon=(0.5+\epsilon,0.5+\epsilon)$.
%     % 
%     Indeed, for $\vec q_\epsilon$ the routine of the IM is still well-defined and the cost of the output of IM does not depend on which $\vec q$ we consider, thus the inequality holds.
%     % 
%     If we take the average and the limits for $k\to \infty$ on both sides, we infer from Theorem
%     \ref{thm:limitBAR} that
%     \begin{align*}
%         \nonumber\lim_{k\to\infty}\frac{\EE [SC_{IM}(\vec X)]}{\EE [SC_{opt}(\vec X)]}&\ge\lim_{n\to\infty}\frac{\EE [SC_{Id,\vec v_\epsilon}(\vec X)]}{\EE [SC_{opt}(\vec X)]}=\frac{W_1(\mu,\eta_\epsilon)}{W_1(\mu,\nu_{m})},
%     \end{align*}
%     where $\eta_\epsilon=\lambda_\epsilon\delta_{F^{[-1]}_\mu(0.5-\epsilon)}+(1-\lambda_\epsilon)\delta_{med(\mu)}$ and
%     \[
%     \lambda_\epsilon=F_\mu\Big(\frac{F^{[-1]}_\mu(0.5-\epsilon)+F^{[-1]}_\mu(0.5)}{2}\Big).
%     \]
%     % 
%     Since the measure $\eta_\epsilon$ converges in probability to $\delta_{med(\mu)}$ when $\epsilon\to 0$, we infer that
%     \[
%     \lim_{k\to\infty}\frac{\EE [SC_{IM}(\vec X)]}{\EE [SC_{opt}(\vec X)]}\ge  \frac{W_1\big(\mu,\delta_{med(\mu)}\big)}{W_1(\mu,\nu_{m})},
%     \]
%     hence the Bayesian approximation ratio of the IM is $\frac{W_1(\mu,\delta_{med(\mu)})}{W_1(\mu,\nu_{m})}$, where $\nu_{m}$ is the solution to problem \eqref{eq:min_proj}.
%     % 
%     % Similarly, we can study the limit Bayesian Approximation ratio of the mechanism with respect to the $l_p$ costs and the Maximum Costs.
%     % 

%     % 
%     Finally, it is worth to notice that the same argument allows to study the limit Bayesian approximation ratio of the InnerChoice Mechanism proposed in \cite{ijcai2022p75} and any truthful Ranking Mechanism have bounded limit Bayesian approximation ratio.
%     % 
%     In particular, the InnerChoice Mechanism has the same limit Bayesian approximation ratio of the IM, with respect to all the cost functions.
% % \end{example}
% % 


% \subsection{The Extended Endpoint Mechanism }
% \label{sec:EEM}

% Given a p.c.v. $\vec q$ , the Extended Endpoint Mechanism (EEM) is a mechanism proposed in \cite{aziz2020capacity} feasible to handle any $2$-CFLP.
% % 
% In our formalism, the routine of the EEM is as follows.
% % 
% Let $\vec x$ be a vector containing the agents' report.
% % 
% Without loss of generality, we assume that $\vec x$ is ordered non decreasingly, i.e. $x_i\le x_{i+1}$.
% % 
% We define $A_1=\{x_i\;\textrm{s.t.}\; |x_i-x_1|\le\frac{1}{2}|x_1-x_n|\}$ and $A_2=\{x_i\;\textrm{s.t.}\; x_i\notin A_1\}$.
% % 
% If $|A_1|\ge |A_2|$, the EEM determines the position of two facilities as follows:

% \begin{enumerate}[label=(\roman*)]
%     \item If $|A_1|\le \floor{q_1(n-1)}+1$ and $|A_2|\le \floor{q_2(n-1)}+1$, we set $y_1=x_1$ and $y_2=x_n$, we place the facility with capacity $q_1$ at $y_1$ and the facility with capacity $q_2$ at $y_2$.

%     \item If $|A_1|> \floor{q_1(n-1)}+1$ and $|A_2|\le \floor{q_2(n-1)}+1$, we set $y_1=2x_{\floor{q_1(n-1)}+2}-x_n$ and $y_2=x_n$, we place the facility with capacity $q_1$ at $y_1$ and the facility with capacity $q_2$ at $y_2$.

%     \item If $|A_1|\le \floor{q_1(n-1)}+1$ and $|A_2|> \floor{q_2(n-1)}+1$, we set $y_1=x_1$ and $y_2=2x_{n-(\floor{q_2(n-1)}+1)}-x_1$, we place the facility with capacity $q_1$ at $y_1$ and the facility with capacity $q_2$ at $y_2$.
% \end{enumerate}

% % 
% In all of the cases above, every agent is assigned to the facility that is closer to the position (break ties arbitrarily without  overloading any facility).
% % 
% Finally, if $|A_1|> |A_2|$, it suffices to switch the roles of the two facilities in the cases described above.

% We now study the limit Bayesian approximation ratio of the EEM when the agents are distributed according to a uniform distribution and $\vec q=(0.8,0.4)$.
% % 
% For the sake of simplicity, we consider only a odd number of agents $n=2k+1$.
% % 
% First, we notice that we can restrict our attention to the class of instances in which $|A_1|>|A_2|$.
% % 
% Indeed, due to the symmetry of the uniform distribution, we have that the every instance for which $|A_1|>|A_2|$ holds, uniquely identifies an instance for which it holds $|A_1|<|A_2|$\footnote{Since $n$ is odd we have that we cannot have $|A_1|=|A_2|$.}.
% %  
% Let us consider the expected Social Cost of the instances for which it holds $|A_1|>|A_2|$, which we denote with $\mathcal{A}$.
% % 
% Using the properties of the expected values, we can compute the expected Social Cost of the EEM as the sum of three conditioned expected values
% \begin{align*}
%     \EE[SC_{\pi,\vec v}(\vec X)]&=\EE[SC_{\pi,\vec v}(\vec X)|\vec X\in C_1]P(\vec X\in C_1)\\
%     % 
%     &\quad+\EE[SC_{\pi,\vec v}(\vec X)|\vec X\in C_2]P(\vec X\in C_2)\\
%     % 
%     &\quad+\EE[SC_{\pi,\vec v}(\vec X)|\vec X\in C_3]P(\vec X\in C_3),
% \end{align*}
% where \begin{enumerate*}[label=(\roman*)]
%     \item $C_1$ contains all the instances for which $|A_1|\le \floor{q_1(n-1)}+1$ and $|A_2|\le\floor{q_2(n-1)}+1$;
%     \item $C_2$ contains all the instances for which $|A_1|> \floor{q_1(n-1)}+1$ and $|A_2|\le \floor{q_2(n-1)}+1$; and
%     \item $C_3$ contains all the instances for which $|A_1|\le \floor{q_1(n-1)}+1$ and $|A_2|>\floor{q_2(n-1)}+1$.
% \end{enumerate*}
% Notice that $\mathcal{A}=C_1\cup C_2 \cup C_3$.
% % 
% Moreover, every $C_i$ is disjoint from the other, hence, since we are restricting our attention to only the instances in $\mathcal{A}$, we have 
% \[
% P(\vec X\in C_3)=1-P(\vec X \in C_1)-P(\vec X \in C_2).
% \]
% % 

% % 
% We first show that both $P(\vec X \in C_1)$ and $P(\vec X \in C_2)$ go to $0$ as the number of agents go to infinity and then show that 
% \[
% \lim_{n\to \infty}\EE[SC_{\pi,\vec v}(\vec X)|\vec X\in C_3]=W_1(\mu,(1-q_2)\delta_{0}+q_2\delta_{1.2}).
% \]
% % 

% % 
% First, let us consider $P(\vec X \in C_1)$.
% % 
% Notice that 
% \begin{align*}
%     P(\vec X \in C_1)&=P(|A_1|\le \floor{q_1(n-1)}+1,|A_2|\le\floor{q_2(n-1)}+1)\\
%     &\le P(|A_2|\le\floor{q_2(n-1)}+1)\\
%     &\le P\Big(X_{\floor{0.55(n-1)}+1}\le \frac{X_1+X_n}{2}\Big),
% \end{align*}
% where the last inequality comes from the fact that if $$|A_2|\le \floor{q_2(n-1)}+1$$ then it must be that $X_{\floor{0.55(n-1)}+1}\le \frac{X_1+X_n}{2}$, since $q_2=0.4$.
% % 
% Let us now set $\epsilon>0$ and $r=\floor{0.55(n-1)}+1$, then we have
% \begin{align*}
%     P(\vec X \in C_1) &\le P\Big(X_{r}\le \frac{X_1+X_n}{2}\Big)\\
%     &=P\Big(X_{r}\le \frac{X_1+X_n}{2}\Big|X_1\le \epsilon, X_n\ge 1-\epsilon\Big)P(X_1\le \epsilon, X_n\ge 1-\epsilon)\\
%     &\quad +P\Big(X_{r}\le \frac{X_1+X_n}{2}\Big|X_1\ge \epsilon, X_n\le 1-\epsilon\Big)P(X_1\ge \epsilon, X_n\le 1-\epsilon)\\
%     &\le P\Big(X_{r}\le \frac{1+\epsilon}{2}\Big)\big(P(X_1\le \epsilon)+P( X_n\ge 1-\epsilon)\big)\\ 
%     &\quad + P(X_1\ge \epsilon)+P( X_n\le 1-\epsilon),
% \end{align*}
% since $P\Big(X_{r}\le \frac{X_1+X_n}{2}\Big|X_1\ge \epsilon, X_n\le 1-\epsilon\Big)\le 1$.
% % 
% Notice that the cumulative distribution function of the $n$-th order statistic of a uniform distributed random variable is
% \[
% t\to \Big(F_\mu(t)\Big)^n=t^n
% \]
% hence 
% \[
% P( X_n\le 1-\epsilon)=(1-\epsilon)^n
% \]
% hence $\lim_{n\to \infty}P( X_n\le 1-\epsilon)=0$.
% % 
% Likewise, we have that 
% \[
% \lim_{n\to \infty} P(X_1\ge \epsilon)=0.
% \]
% % 
% Lastly, we need to show that $P\Big(X_{r}\le \frac{1+\epsilon}{2}\Big)$ goes to $0$ as $n$ goes to infinity.
% % 
% It is well-known that, for a suitable constant $K$, it holds $K\sqrt{n}(X_{\floor{0.55(n-1)}+1}-0.55)$ converges in distribution to the standard Gaussian $Z\sim\mathcal{N}(0,1)$.
% % 
% Given $\epsilon<0.05$, we have that
% \begin{align*}
%     P\Big(X_{r}&\le \frac{1+\epsilon}{2}\Big)=P\Big(K\sqrt{n}(X_{\floor{0.55(n-1)}+1}-0.55)\le K\sqrt{n}\Big(\frac{1+\epsilon}{2}-0.55\Big)\Big).
% \end{align*}
% Thus
% \begin{align*}
%     P\Big(X_{r}\le \frac{1+\epsilon}{2}\Big)&\le \Bigg|P\Big(X_{r}\le \frac{1+\epsilon}{2}\Big)\Big)-P\Big(Z\le K\sqrt{n}\Big(\frac{1+\epsilon}{2}-0.55\Big)\Big)\Bigg|\\
%     &\quad + P\Big(Z\le K\sqrt{n}\Big(\frac{1+\epsilon}{2}-0.55\Big)\Big).
% \end{align*}
% Since $\Big(\frac{1+\epsilon}{2}-0.55\Big)<0$, we have that
% \[
% \lim_{n\to\infty}P\Big(Z\le K\sqrt{n}\Big(\frac{1+\epsilon}{2}-0.55\Big)\Big)=0.
% \]
% Finally, by the convergence in distribution of $X_r$,see \cite{wilks2012mathematical,david2004order}, we have
% \[
% \lim_{n\to\infty}\Bigg|P\Big(X_{r}\le \frac{1+\epsilon}{2}\Big)\Big)-P\Big(Z\le K\sqrt{n}\Big(\frac{1+\epsilon}{2}-0.55\Big)\Big)\Bigg|=0,
% \]
% which allows us to conclude that $\lim_{n\to\infty}P(\vec X\in C_1)=0$.

% % 
% Similarly, we have that $ \lim_{n\to\infty}P(\vec X \in C_2)=0$, hence $\lim_{n\to\infty}P(\vec X\in C_3)=1$.

% % 

% % 
% Lastly, we need to show that 
% \[
% \lim_{n\to \infty}\EE[SC_{\pi,\vec v}(\vec X)|\vec X\in C_3]=W_1(\mu,(1-q_2)\delta_{0}+q_2\delta_{1.2}).
% \]
% % 
% Notice that if $\vec x\in C_3$, the EEM places a facility at $x_1$ and the other one at $2x_{n-(\floor{q_2(n-1)}+2)}-x_1$, the first $n-(\floor{q_2(n-1)}+1)$ agents are assigned to the facility placed at $x_1$, while the others to the facility at $2x_{n-\floor{q_2(n-1)}+2}-x_1$.
% % 
% Since every agent is assigned to its closest facility, we can adapt the argument used to prove Lemma \ref{lemma:equivalenceSC_W1}, and infer that
% \[
% SC_{EEM}(\vec x)=W_1(\mu_n,q_1\delta_{x_1}+(1-q_1)\delta_{2x_{n-\floor{q_2(n-1)}+2}-x_1}).
% \]
% % 
% By the same argument used in the proof of Theorem \ref{thm:limitBAR}, it is possible to show that 
% \begin{align*}
%     \lim_{n\to \infty}W_1(\mu_n,q_1\delta_{x_1}&+(1-q_1)\delta_{2x_{\floor{q_1(n-1)}+2}-x_1})=W_1(\mu,(1-q_2)\delta_{0}+q_2\delta_{1.2}),
% \end{align*}
% which concludes the proof.

% It is important to emphasize that the study of the limit of the Bayesian approximation ratio hinges upon the fact that the support of the uniform distribution is compact.
% % 
% Indeed, following the same argument, it is possible to study the limit Bayesian approximation ratio of any compactly supported measure and any p.c.v. $\vec q$.
% % 






% \section{How to Select an Optimal ERM}
% \label{sec:para}
% As shown in Theorem \ref{thm:limitBAR}, the limit Bayesian approximation ratio of any ERM hinges upon $\mu$, $\vec q$, $\pi$, and $\vec v$.
% % 
% While $\mu$ and $\vec q$ are beyond the control of the mechanism designer, both $\pi$ and $\vec v$ serve as parameters that can be tuned depending upon $\mu$ and $\vec q$.
% % 
% In this section, we study how to determine an optimal ERM tailored to $\mu$ and $\vec q$.
% % 
% Given $\mu$ and $\vec q$, we say that a feasible $\RM$ is optimal if 
% \[
% \lim_{n\to\infty}B_{ar}\big(\RM\big)\le\lim_{n\to\infty}B_{ar}\big(\texttt{ERM}^{(\pi',\vec v')}\big)
% \]
% for any other feasible $\texttt{ERM}^{(\pi',\vec v')}$.
% % 
% The main result of the section assesses that an optimal ERM exists and characterizes its parameters $(\pi,\vec v)$ as the solution to a suitable minimization problem.
% % 

% \begin{theorem}
% \label{thm:existance_problem}
% Given $\mu$ and a p.c.v. $\vec q$, there always exist a tuple $(\pi,\vec v)$ whose associated ERM, that is $\RM$,
% is optimal.
% % 
% Moreover, the couple $(\pi,\vec v)$ is a solution to the following minimization problem
% \begin{align}
% \label{eq:opt:ERM}
%     \min_{\pi\in\mathcal{S}_m}\min_{\vec v\in (0,1)^m} &W_1\Big(\mu,\sum_{j\in[m]}\eta_j\delta_{F_\mu^{[-1]}(p_j)}\Big)\\
%     \nonumber\text{such that}\; &p_{j+1}-p_{j-1}\le q_{\pi(j)}\;\;\text{for} \;\; j=2,\dots,m-1,\\
%     \nonumber&p_1\le q_{\pi(q)}, \;\text{and}\;\; p_m\le 1-q_{\pi(m)},
% \end{align}
% where $\eta_1=F_\mu\Big(\frac{F^{[-1]}_\mu(p_{2})+F^{[-1]}_\mu(p_{1})}{2}\Big)$, $\eta_j=F_\mu\Big(\frac{F^{[-1]}_\mu(p_{j+1})+F^{[-1]}_\mu(p_{j})}{2}\Big)-F_\mu\Big(\frac{F^{[-1]}_\mu(p_{j})+F^{[-1]}_\mu(p_{j-1})}{2}\Big)$ for $j=2,\dots,m-1$, and $\eta_m=1-\eta_{m-1}$.
% \end{theorem}

% \begin{proof}
% % [Proof of Theorem \ref{thm:existance_problem}]
% Since for every $m$ there are a finite number of $\pi\in\mathcal{S}_m$, it suffices to show that for every $\sigma\in\mathcal{S}_m$ there exists a solution to problem
% \begin{align}
% \label{eq:opt:ERM2}
%     \min_{\vec v\in (0,1)^m} &W_1\Big(\mu,\sum_{j\in[m]}\eta_j(\vec v)\delta_{F_\mu^{[-1]}(p_j)}\Big)\\
%     \nonumber\text{such that}\; &p_{j+1}-p_{j-1}\le q_{\pi(j)}\;\;\text{for} \;\; j=2,\dots,m-1,\\
%     \nonumber&p_1\le q_{\pi(q)}, \;\text{and}\;\; p_m\le 1-q_{\pi(m)},
% \end{align}
% where 
% \begin{align*}
%     \eta_j(\vec v)=&F_\mu\Big(\frac{F^{[-1]}_\mu(p_{j+1})+F^{[-1]}_\mu(p_{j})}{2}\Big)-F_\mu\Big(\frac{F^{[-1]}_\mu(p_{j})+F^{[-1]}_\mu(p_{j-1})}{2}\Big)
% \end{align*}

% for $j=2,\dots,m-1$,
% \[
% \eta_1(\vec v)=F_\mu\Big(\frac{F^{[-1]}_\mu(p_{2})+F^{[-1]}_\mu(p_{1})}{2}\Big),
% \]
% and $\eta_m(\vec v)=1-\eta_{m-1}(\vec v)$.
% % 
% By the same argument used during the second step of proof of Theorem \ref{thm:limitBAR}, we have that, given $\vec v$, the measure 
% \[
% \eta(\vec v)=\sum_{j\in[m]}\eta_j(\vec v)\delta_{F_\mu^{[-1]}(p_j)}
% \]
% is such that
% \[
% W_1(\mu,\eta(\vec v))=\min_{\lambda_j\le q_{\sigma(j)},\sum_{j\in[m]}\lambda_j=1}W_1\Big(\mu,\sum_{j\in[m]}\lambda_j\delta_{F_\mu^{[-1]}(p_j)}\Big).
% \]
% % 
% % 
% First, we consider the case in which $\mu$ has a compact support, hence the minimization problem is well defined over the closed set $[0,1]^m$, since the values $F_\mu^{[-1]}(0)$ and $F_\mu^{[-1]}(1)$ are well-defined.
% % 
% Notice that $[0,1]^m$ is compact, thus if we show that the objective function of the problem is continuous with respect to $\vec v$ we conclude the proof for this case.
% % 
% Let $\vec v^{(n)}$ be a succession of feasible vectors that converges to $\vec v$.
% % 
% By the assumptions on $\mu$, we have that both $F_\mu$ and $F_\mu^{[-1]}$ are continuous, hence
% \[
% \vec v\to \eta_j(\vec v)
% \]
% is continuous for every $j\in [m]$.
% % 
% Likewise, the function
% \[
% \vec v\to y_j(\vec v):=F_\mu^{[-1]}(p_j)
% \]
% is continuous for every $j\in[m]$.
% % 
% As a consequence the sequence $\eta_n=\eta(\vec v^{(n)})$ weakly converges to $\eta(\vec v)$ in $\PP(\erre)$, \cite{villani2009optimal}.
% % 
% Since $W_1$ induces the weak convergences \cite{villani2009optimal} over $\PP(\erre)$, we infer
% \[
% \lim_{n\to \infty}W_1(\mu,\eta(\vec v^{(n)}))=W_1(\mu,\eta(\vec v)).
% \]
% To conclude the proof, we need to show that the minimizer, namely $\vec v$, is such that $p_j\neq 0,1$ for every $j\in [m]$.
% % 
% Toward a contradiction, let us assume that $p_1=0$.
% % 
% Without loss of generality, let us assume that $p_2>0$, thus $y_1< y_2$.
% % 
% By definition, we have that $F_\mu^{[-1]}(p_1)=a$ and $F_\mu(F_\mu^{[-1]}(p_1))=p_1=0$.
% % 
% Let us denote with $[a,b]$ the support of $\mu$, then there exists a $\epsilon>0$ such that $a+\epsilon<F_\mu^{[-1]}(p_2)$, thus
% \begin{align*}
%     \mathcal{W}(\vec v)&=\int_{a}^{b}\min_{j\in[m]}|x-F_\mu^{[-1]}(p_j)|d\mu=\int^{\frac{a+F_\mu^{[-1]}(p_2)}{2}}_a(x-a)d\mu+\sum_{j>1}^m\int_{\frac{a+y_2}{2}}^b\min_{j>1}|x-F_\mu^{[-1]}(p_j)|d\mu\\
%     &>\int_{a}^{\frac{a+F_\mu^{[-1]}(p_2)}{2}}|x-(a+\epsilon)|d\mu+\sum_{j>1}^m\int_{\frac{a+F_\mu^{[-1]}(p_2)}{2}}^b\min_{j>1}|x-F_\mu^{[-1]}(p_j)|d\mu\\
%     &>\int_{a}^{b}\min_{j\in[m]}|x-F_\mu^{[-1]}(p^{(\epsilon)}_j)|d\mu=\mathcal{W}(\vec v^{(\epsilon)}),
% \end{align*}
% where $\vec v^{(\epsilon)}=(F_\mu(a+\epsilon),p_2,\dots,p_m)$, which contradicts the optimality of $\vec v$.
% % 

% % 
% Let us now consider the case in which $\mu$ has unbounded support.
% % 
% Let $\vec v^{(n)}$ be a minimizing sequence.
% % 
% Up to a sub-sequence, we can assume that the $\vec v^{(n)}$ converges to $\vec v$ in $[0,1]^m$.
% % 
% We now show that $\vec v\in (0,1)^m$.
% % 
% First, let us assume that there exists a $j\in[m]$ for which $p_j\in (0,1)$.
% % 
% Without loss of generality, let us assume that $p_1=0$ and that $1>p_2>0$ (if there are multiple entries of $\vec v$ that are equal to $0$ the study is the same).
% % 
% {\color{red} Let us now consider $\vec v^{(n)}$ be such that $v^{(n)}_1=p_1^{(n)}$ and $v_j^{(n)}=p_j$ for $j>1$.
% % 
% Since $\vec v^{(n)}$ and $\vec v^{(n)}$ have the same limit and $\mathcal{W}$ is continuous, we have that $\vec v^{(n)}$ is a minimizing sequence.}
% % 
% Since $p^{(n)}_1\to 0$, we have that $F_\mu^{[-1]}(p_1^{(n)})\to -\infty$, thus
% \begin{align*}
%     \mathcal{W}(\vec v^{(n)})=\int_{-\infty}^{\frac{y_1^{(n)}+y_2}{2}}|x-F_\mu^{[-1]}(p_1^{(n)})|d\mu+\int_{\frac{y_1^{(n)}+y_2}{2}}^{+\infty}\min_{j>1}|x-F_\mu^{[-1]}(p_j)|d\mu.
% \end{align*}
% % 
% Since $F_\mu^{[-1]}(p_1^{(n)})\to -\infty$, we have that
% \[
% \mathcal{W}(\vec v)=\int_{-\infty}^{+\infty}\min_{j>1}|x-F_\mu^{[-1]}(p_j)|d\mu.
% \]
% Let us consider the vector $\vec v^{(\epsilon)}=(\epsilon,p_2,\dots,p_m)$, where $p_2>\epsilon>0$, then it holds
% \begin{align*}
%     \mathcal{W}(\vec v)&=\int_{-\infty}^{+\infty}\min_{j>1}|x-F_\mu^{[-1]}(p_j)|d\mu > \int_{-\infty}^{+\infty}\min_{j\in[m]}|x-F_\mu^{[-1]}(p^{(\epsilon)}_j)|d\mu=\mathcal{W}(\vec v^{(\epsilon)}),
% \end{align*}
% which contradicts the optimality of $\vec v$.
% % 
% Through a similar argument, we deal with the case $\vec v\in\{0,1\}^m$.


% Finally, we notice that the case in which the support of $\mu$ is unbounded only from one side is similar.
% \end{proof}

% Notice that the limit Bayesian approximation ratio of the optimal ERM does not necessarily converge to $1$, as the next example shows.

% \begin{example}
% \label{ex:impox_aoerm}
%     Let $\mu$ be the uniform distribution $\mathcal{U}[0,1]$ and let $\vec q=(0.8,0.4)$ be a p.c.v..
%     % 
%     Since $\mu$ is symmetric, one of the solutions to problem \eqref{eq:min_proj} is $\nu_2=(0.4)\delta_{0.2}+(0.6)\delta_{0.7}$ (the other one is $\nu_2'=(0.6)\delta_{0.3}+(0.4)\delta_{0.8}$).
%     % 
%     However, by Corollary \ref{crr:sparecapacity}, there does not exist a permutation $\pi\in\mathcal{S}_m$ such that $\texttt{ERM}^{((0.2,0.7), \pi)}$ is feasible.
%     % 
%     Thus, by Theorem \ref{thm:limitBAR}, no feasible ERM is such that $\lim_{n\to\infty}B_{ar}(\RM)=1$.
%     % 

%     % 
%     This result is extremely interesting if compared to the expected performances of the EEM.
%     % 
%     Indeed, owing to the argument presented in Section \ref{sec:EEM}, we have that the EEM will either 
% \begin{enumerate*}[label=(\roman*)]
%     \item place the facility with capacity $q_2$ at $y_1=x_1$ and the other facility at $y_2=2x_{n-(\floor{q_1(n-1)}+1)}-x_1$ with probability $0.5$ or
%     \item place the facility with capacity $q_2$ at $y_2=x_n$ and the other facility at $y_1=2x_{\floor{q_1(n-1)}+2}-x_n$ with probability $0.5$.
% \end{enumerate*} 
% Since $\mu=\mathcal{U}[0,1]$, we have that $x_1\to 0$, $x_n\to 1$, $x_{n-\floor{q_2(n-1)}+2}\to F_\mu^{[-1]}(1-q_2)=1-q_2$, and $x_{\floor{q_2(n-1)}+1}\to F_\mu^{[-1]}(q_2)=q_2$.
% % 
% In particular, the limit expected Social Cost of the mechanism is then $\frac{1}{2}W_1(\mu,q_2\delta_{2q_2-1}+(1-q_2)\delta_1)+\frac{1}{2}W_1(\mu,(1-q_2)\delta_{0}+q_2\delta_{2-2q_2})$.
% % 
% Since $\mu$ is symmetric with respect to $\frac{1}{2}$, we have that $W_1(\mu,q_2\delta_{2q_2-1}+(1-q_2)\delta_1)=W_1(\mu,(1-q_2)\delta_{0}+q_2\delta_{2-2q_2})=\frac{(1-q_2)^2}{2}+\frac{q_2(2-3q_2)}{2}=0.34$, hence the limit Bayesian approximation ratio of the EEM is $\sim 2.62$.
% \end{example}







% % 
% We now characterize the optimal ERM in two specific cases.
% % 
% In the first one, the total capacity of the facilities is the same as the number of agents.
% % 
% In the second one, we need to place two capacitated facilities and $\mu$ is a uniform distribution.
% % 



% \subsection{The No-Spare Capacity Case}
% \label{sec:case2}

% % It was shown in \cite{aziz2020capacity} that if the total capacity of the facilities matches the number of agents, a Ranking Mechanism is truthful if and only if it places all the facilities at two adjacent agents' reports, namely $x_t$ and $x_{t+1}$.
% % % 
% % However, not all the values of $t$ are feasible, as it must exist $J'\subset [m]$ such that $t=\sum_{j\in J'}c_j$.
% % % 
% % Through the same argument used in Remark \ref{ex:im}, we are able to characterize the limit Bayesian approximation ratio of such mechanisms and to determine the one that achieves the lowest Bayesian approximation ratio.
% % % 
% % % Since $t$ depends on the subset $J'$, there are up to $m!$ different truthful mechanisms.
% % % % 
% % % Unless $m=2$, $c_1=c_2$, and $c_1=t$, the worst-case approximation ratio of all these mechanisms is $+\infty$, regardless of $t$.
% % % % 
% % % From Theorem \ref{thm:limitBAR}, we have that different values of $t$ lead to different Bayesian approximation ratios, in what follows, we show that there is an easy criteria to elicit the best possible ranking mechanism for this case.

% % \begin{lemma}
% % \label{thm:no_spare_capacy}
% %     Let $\vec q$ be a p.v.c. such that $\sum_{j\in [m]}q_j=1$.
% %     % 
% %     The Ranking Mechanism that achieves the lowest Bayesian approximation ratio is induced by the vector $\vec v=(p,\dots,p)$, where $p$ is either $\max_{J'\in \mathcal{P}_{\le 0.5}([m])}\sum_{j\in J'}q_j$ or $\min_{J'\in \mathcal{P}_{\ge 0.5}([m]) }\sum_{j\in J'}q_j$, where $\mathcal{P}_{\le 0.5}([m])$ contains all the subsets of $[m]$ for which it holds $\sum_{j\in J'}q_j\le 0.5$ and $\mathcal{P}_{\ge 0.5}([m])$ contains all the subsets of $[m]$ for which it holds $\sum_{j\in J'}q_j\ge 0.5$. 
% % \end{lemma}



% In the no-spare capacity case, the total capacity of the facilities matches the number of agents, thus $\sum_{j\in[m]}q_j=1$.
% % 
% Due to Corollary \ref{crr:sparecapacity}, we have that the only feasible ERMs are the ones for which it holds $p_j=p\in[0,1]$ for every $j\in[m]$.
% % 
% Thus, owing to the properties of the $W_1$ distance and to Lemma \ref{lemma:equivalenceSC_W1}, the optimal ERM is the $\texttt{all-median}$ mechanism, i.e. $\texttt{ERM}^{(Id,(0.5,\dots,0.5))}$.
% % , which places all the facilities at the median agent, i.e. $\vec v=(0.5,\dots,0.5)$.
% % 
% % Since all the facilities are placed at the same point, any permutation $\pi\in\mathcal{S}_m$ induces the same mechanism.

% \begin{theorem}
% \label{crr:nsc_best_RM}
%     In the no-spare capacity case, the optimal ERM is unique.
%     % 
%     Moreover, we hat that \begin{enumerate*}[label=(\roman*)]
%         \item the $\texttt{all-median}$ mechanism is optimal with respect to the Social Cost,
%         \item the $\RM$ is optimal with respect to the $l_2$ cost if $\vec v=(F_\mu(m),\dots,F_\mu(m))$ where $m$ is the mean of $\mu$, and
%         \item if $\mu$ has compact support, then $\RM$ is optimal with respect to the Maximum Cost if $\vec v=(F_\mu(\frac{a+b}{2}),\dots,F_\mu(\frac{a+b}{2}))$ where $a=\inf\{x\in spt(\mu)\}$ and $b=\sup\{x\in spt(\mu)\}$.
%         \end{enumerate*}
% \end{theorem}

% \begin{proof}
%     % 
%     Owing to Corollary \ref{crr:sparecapacity}, we have that any truthful ERM, namely $\RM$, must be such that $\vec v=(p,p,\dots,p)$ where $p\in(0,1)$.
%     % 
%     Thus to complete the proof it is sufficient to prove that the function
%     \begin{equation}
%         \label{definition:Mfunction}
%         M:y\to\int_{\erre}|x-y|d\mu
%     \end{equation}
%     % 
%     is decreasing on $(-\infty,med(\mu))$ and increasing on $(med(\mu),+\infty)$.
%     % 
%     We do that by computing the derivative of $M$ with respect to $y$.
%     % 
%     Without loss of generality, let us assume that $y\in(-\infty,med(\mu))$ and let us consider
%     \[
%     \lim_{h\to 0^+}\frac{\int_{\erre}|x-(y+h)|d\mu-\int_\erre |x-y|d\mu}{h}.
%     \]
%     By the linearity of the integral, we have that
%     \[
%     \int_\erre |x-y|d\mu=\int_{-\infty}^y (y-x)d\mu+\int_y^{+\infty}(x-y)d\mu,
%     \]
%     similarly $\int_\erre |x-(y+h)|d\mu=\int_{-\infty}^{y+h} (y+h-x)d\mu+\int_{y+h}^{+\infty}(x-y-h)d\mu$, so that
%     \begin{align*}
%         \int_{\erre}|x-(y+h)|d\mu-\int_\erre |x-y|d\mu &=2\int_{y}^{y+h}(y-x)d\mu+\int_{-\infty}^yhd\mu-\int_{y}^{+\infty}hd\mu\\
%         &\le h^2+\int_{-\infty}^yhd\mu -\int_{y}^{+\infty}hd\mu,
%     \end{align*}
%     thus $\partial_y M(y)=F_\mu(y)-(1-F_\mu(y))$.
% % 
%     Since $y<med(\mu)$, we infer that $\partial_y M(y)<0$.
%     % 
%     Similarly, it holds $\partial_y M(y)>0$ if $y>med(\mu)$, which concludes the proof for the Social Cost.
%     % 
%     The results for the $l_2$ costs and the Maximum Cost follow by a similar argument.
%     % 
% \end{proof}

% % 
% % Since the best possible RM or ERM places all the facilities at the median agent, we infer that in the no-spare capacity framework no ERM or Ranking Mechanism can be be asymptotically optimal.
% % 
% % 
% % \begin{corollary}
% %     In the no-spare capacity framework, no Ranking Mechanism can be Asymptotically optimal as long as $m>1$.
% %     % 
% %     Furthermore, no mechanism can achieve a better asymptotic approximation ratio than a mechanism that places all the facilities at the median of the probability distribution.
% % \end{corollary}
% % 
% % \begin{proof}
% %     The fact that no RM can achieve a limit Social Cost that is lower than the one achieved by a mechanism that places all the facility at the median follows directly by Theorem \ref{thm:no_spare_capacy} and by the fact that the median minimizes the function $M$ defined as in \eqref{definition:Mfunction}.
% %     % 
% %     To conclude, notice that the solution of problem \eqref{eq:min_proj} when $m>1$ is always supported over $m$ different points, thus the asymptotic optimal Social Cost is always strictly lower than the limit cost any RM.
% % \end{proof}
% % 
% % Moreover, the Bayesian approximation ratio of the median mechanism gives a lower bound on what the limit of the Bayesian approximation ratio of the mechanism can be in the no-spare capacity framework. 
% % 

% % 
% % In the no-spare capacity case, it is possible to analytically study the limit approximation ratio of the best ERM when the agents are supported according to any distribution.
% % % 
% % In what follows, we showcase this procedure with the uniform distribution.
% % 


% % 
% When the agents are distributed following a uniform distribution, that is $\mu=\mathcal{U}[0,1]$, we can express the limit Bayesian approximation ratio of the $\texttt{all-median}$ mechanism as a function of $\vec q$.
% % 
% Indeed, since $\sum_{j\in[m]}q_j=1$, any solution to problem \eqref{eq:min_proj} separates the interval $[0,1]$ into $m$ intervals whose length is $q_j$.
% % 
% Notice that the order in which $[0,1]$ is divided is irrelevant.
% % 
% Furthermore, the facility is placed at the median of such interval, thus the objective value of \eqref{eq:min_proj} is $\frac{1}{4}\sum_{j\in[m]}q_j^2$.
% % 
% By Theorem \ref{thm:limitBAR}, the limit Bayesian approximation ratio of the \texttt{all-median} mechanism is $\lim_{n\to\infty}B_{ar}(\texttt{all-median})=(\sum_{j\in[m]} q_j^2)^{-1}$, since the asymptotic cost of placing all the facilities at the median point is $\int_0^1|x-0.5|dx=\frac{1}{4}$.
% % 
% Notice that the limit Bayesian approximation ratio gets closer to $1$ as the values of $\vec q$ become concentrated at one index.
% % 
% Conversely, if all the facilities have the same capacity $\frac{1}{m}$, we have that the Bayesian approximation ratio of the \texttt{all-median} becomes the largest possible, that is $\lim_{n\to\infty}B_{ar}(\RM)=m$.
% % 



% \begin{example}[Comparing the Ranking Mechanisms with the ERMs]
% % \textbf{
%     To the best of our knowledge, the only other truthful mechanisms capable of placing more than $2$ facilities in the no-spare capacity case are the Ranking Mechanisms \cite{aziz2020facility}.
%     % 
%     To close the section, we show that the $\texttt{all-median}$ mechanism is also the asymptotically best possible Ranking Mechanism.
%     % 
%     Indeed, by \cite{aziz2020facility}, we know that a truthful Ranking Mechanism either \begin{enumerate*}[label=(\roman*)]
%     \item puts all the facilities at the same position or
%     \item places all the facilities at two adjacent agents' reports, namely $x_t$ and $x_{t+1}$.
%     % % 
%     However, not all the values of $t$ are feasible, as it must exist $J'\subset [m]$ such that $t=\sum_{j\in J'}c_j$.
%     \end{enumerate*}
%     % 
%     Owing to Theorem \ref{crr:nsc_best_RM}, in case (i), the best possible mechanism is the $\texttt{all-median}$ mechanism.
%     % 
%     In case (ii) the limit Bayesian approximation ratio of any mechanism is either equal or higher (see Appendix C).
%     % \ref{app:C}).
%     % 
%     % (see Appendix \ref{app:C}).
%     %
%     Indeed, consider a population distributed as a Uniform distribution, i.e. $\mu=\mathcal{U}[0,1]$, and $\vec q=(\frac{1}{3},\frac{1}{3},\frac{1}{3})$, and the Ranking Mechanism that places $q_1$ at $x_{\floor{\frac{n-1}{3}}+1}$ and the other two facilities at $x_{\floor{\frac{n-1}{3}}+2}$.
%     % 
%     Since every agent is assigned to its closest facility, it is possible to adapt Lemma \ref{lemma:equivalenceSC_W1} and Theorem \ref{thm:limitBAR} and show that the limit of the expected Social Cost of the mechanism is $W_1(\mu,\delta_{\frac{1}{3}})=\frac{5}{18}$. 
%     % 
%     Hence, the limit Bayesian approximation ratio of the considered Ranking Mechanism is $\sim 3.33$, while $\lim_{n\to \infty}B_{ar}(\texttt{all-median})=3$.
% \end{example}

% % 

% % 




% \subsection{Placing two capacitated facilities for a uniform population.}
% \label{section:tobeextended}

% In this section, we retrieve the optimal ERMs when $\mu=\mathcal{U}[0,1]$ and $m=2$ with respect to the Social Cost.
% % 
% For the sake of simplicity, we divide the discussion into three steps.
% % 
% First, we demonstrate that both permutations in $\mathcal{S}_2$ yield equally optimal ERMs.
% % 
% Second, we explicit the objective function of problem \eqref{eq:opt:ERM} as a function of $\vec v$ and compute its derivatives.
% % 
% Lastly, we retrieve the optimal ERM for any given $\vec q$ using Lagrangian multipliers.
% % 
% % {\color{blue} Notice that this procedure can be generalized to the case in which $\mu$ is symmetric.}
% % 
% % In Appendix \ref{sec:case1}
% In Appendix B, we show how to generalize this process to the case in which $\mu$ is symmetric and other relevant frameworks.
% % 

% % 
% First, notice that, since $F_{\mathcal{U}[0,1]}^{[-1]}(p)=p$ for every $p\in [0,1]$, the objective value of problem \eqref{eq:opt:ERM} boils down to
% \begin{equation*}
%     \mathcal{W}(\vec v):=W_1\Big(\mu, \frac{p_1+p_2}{2}\delta_{p_1}+\big(1-\frac{p_1+p_2}{2}\big)\delta_{p_2}\Big).
% \end{equation*}

% % 
% \textbf{Step $1$.} Since $m=2$, $\mathcal{S}_2=\{Id,\theta\}$, where the permutation $Id$ is such that $Id(i)=i$, and $\theta$ switches $1$ and $2$.
% % 
% First, we show if $(Id,\vec v)$ satisfies system \eqref{eq:feas_system}, there exists a vector $\vec v'$ such that $(\theta,\vec v')$ satisfies \eqref{eq:feas_system} and $\mathcal{W}(\vec v)=\mathcal{W}(\vec v')$.
% % 
% Given $\vec v=(p_1,p_2)$, let us define $\vec v'=(p_1',p_2')=(1-p_2,1-p_1)$.
% % 
% If $(Id,\vec v)$ satisfies system \eqref{eq:feas_system}, we have that $p_2\le q_{Id(1)}=q_1$ and $1-p_1\le q_{Id(2)}=q_2$.
% % 
% It is then easy to see that $p_2'= 1-p_1 \le q_2=q_{\theta(1)}$ and, likewise $1-p_1'\le q_{\theta(2)}$.
% % 
% Thus, $(\theta,\vec v')$ satisfies \eqref{eq:feas_system}.
% % 
% Finally, due to the symmetry of $\mu$ with respect to $0.5$, we have that $\mathcal{W}(\vec v)=\mathcal{W}(\vec v')$.
% % 
% Therefore, for both $Id$ and $\theta$, there exists a vector $\vec v$ that induces an optimal ERM.
% % 
% % For this reason, in what follows, we fix $\pi=Id\in\mathcal{S}_2$. 
% % 


% % 
% \textbf{Step $2$.} Let us fix $\pi=Id$. 
% % 
% Due to the properties of the optimal transportation plan on the line \cite{santambrogio2015optimal}, have that $\mathcal{W}(\vec v)=\int_0^1 \min\{|x-p_1|,|x-p_2|\}dx$, thus $\mathcal{W}(\vec v)=\frac{p_1^2}{2}+\frac{(1-p_2)^2}{2}+\frac{(p_2-p_1)^2}{4}$.
% % 
% From a simple computation, we infer that the objective function $\mathcal{W}(\vec v)$ is differentiable and retrieve the formula of its gradient as $\nabla \mathcal{W}(\vec v)=\frac{1}{2}\big(3p_1-p_2,3p_2-2-p_1\big)$.
% % 
% Notice that the set of points on which the first derivative of $\mathcal{W}$ nullifies is the line $p_2=3p_1$, while the set of points on which the second derivative of $\mathcal{W}$ nullifies is $p_2=\frac{1}{3}(p_1+2)$, thus $\nabla \mathcal{W}(\vec v)=(0,0)$ if and only if $\vec v=(0.25,0.75)$.
% % 
% % A simple computation reveals that the only point for which it holds $\nabla \mathcal{W}(\vec v)=(0,0)$ is $(0.25,0.75)$.




% \textbf{Step $3$.} Lastly, to detect an optimal ERM, we need to implement the feasibility constraints described in Theorem \ref{thm:RM_feasible}.
% % 
% From Step $1$, we focus on the set of constraints induced by $Id\in\mathcal{S}_m$.
% % 
% In this case, we have that $\vec v$ must satisfy the following constraints \begin{enumerate*}[label=(\roman*)]
%     \item $p_2\le q_1$,
%     \item $1-p_1\le q_2$ that is $1-q_2\le p_1$, and
%     \item $p_1\le p_2$.
% \end{enumerate*}
% Thus the set of feasible $\vec v$ is a triangle, namely $T(\vec q)$, whose vertexes are $(q_1,q_1)$, $(1-q_2,1-q_2)$, and $(1-q_2,q_1)$.
% % 
% Finally, we retrieve the best vector $\vec v$ depending on the value of $\vec q$.
% % 
% First, notice that if $(0,25,0.75)\in T(\vec q)$, i.e. if and only if $q_1,q_2\ge 0.75$, then the minimum is attained in $\vec v=(0,25,0.75)$ as it is the only point in which the gradient $\nabla \mathcal{W}$ nullifies and the Hessian matrix is positive definite.
% % 
% For all the other values of $\vec q$, we need to search the minimum over the boundary of $T(\vec q)$, since the gradient is never null on the interior of $T(\vec q)$.
% % 
% First, notice that the minimum cannot lay in the segment connecting the vertexes $(1-q_2,1-q_2)$ and $(q_1,q_1)$.
% % 
% In this case, we have that $\nabla \mathcal{W}(\vec v)= \frac{1}{2}(2p,2p-2)$, hence the gradient is never perpendicular to the line $p_1=p_2$.
% % 
% We then need to search for the minimum in the sets $\{(1-q_2,t)\;\text{s.t.}\;t\in[1-q_2,q_1]\}$ and $\{(t,q_1)\;\text{s.t.}\;t\in[1-q_2,q_1]\}$.
% % 
% % We therefore infer the following theorem.

% \begin{theorem}
% \label{thm:bestuniform}
%     Let $\vec q$ be a p.c.v. such that $q_2\le q_1$, then an optimal ERM for a uniformly distributed population is induced by $(Id,\vec v)$ where
%     \begin{enumerate*}[label=(\roman*)]
%         \item $\vec v=(0.25,0.75)$ if $q_2\ge 0.75$, 
%         \item $\vec v=(1-q_2,q_1)$ if $3q_2-2-q_1\le 0$, and
%         \item $\vec v=(1-q_2,1-\frac{q_2}{3})$ otherwise.
%     \end{enumerate*}
%     % Alternatively, the optimal ERM is induced by $(\theta,\vec v')$ in the equi-capacitated case, the best $\vec v$ is $()$.
% \end{theorem}


% \begin{proof}
% % [Proof of Theorem \ref{thm:bestuniform}] 
%     Let $\vec q$ be such that $0.75 \ge q_2$.
%     % 
%     Then $\vec v=(0.25,0.75)$ is a feasible vector and it holds $\nabla \mathcal{W}(0.25,0.75)=(0,0)$.
%     % 
%     By computing the Hessian of $\mathcal{W}$ we have that
%     \[
%     H\mathcal{W}(\vec v)=\frac{1}{2}\begin{pmatrix}
%     3 & -1 \\
%     -1 & 3 
%     \end{pmatrix},
%     \]
%     hence the matrix is definite positive and thus $(0.25,0.75)$ is the minimum for this case.
%     % 
%     Let us now consider the case in which $3q_2-2-q_1\le 0$, in this case we have that $\partial_{y_1} \mathcal{W}(\vec v)>0$ and $\partial_{y_2} \mathcal{W}(\vec v)<0$.
%     % 
%     Thus the gradient cannot be perpendicular to either $\{(1-q_2,t)\;\text{s.t.}\;t\in[1-q_2,q_1]\}$ and $\{(t,q_1)\;\text{s.t.}\;t\in[1-q_2,q_1]\}$, hence the minimum is at the vertex $(1-q_2,q_1)$, which concludes the proof for this case.
%     % 
%     In the remaining cases, we have that the boundary of $T(\vec q)$ intersect the line on which $\partial_{y_2}\mathcal{W}=0$.
%     % 
%     In particular, $\{\partial_{y_2}\mathcal{W}=0\}$ intersects with the edge $\{(1-q_2,t)\;\text{s.t.}\;t\in[1-q_2,q_1]\}$ at the point $(1-q_2,1-\frac{q_2}{3})$.
%     % 
%     On such point, we have that the gradient is perpendicular to the boundary of $T(\vec q)$ and points inward, thus is a relative minimum.
%     % 
%     To conclude, we show that this is the only possible relative minimum.
%     % 
%     Indeed, it is easy to see that if the boundary of $T(\vec q)$ intersect the line $p_2=3p_1$, the gradient points outward due to the sign of $\nabla \mathcal{W}$.
%     % 
%     We then conclude the proof.
% \end{proof}

% \subsection{Placing \texorpdfstring{$2$}{m} Facilities among Symmetrically Distributed Agents}
% \label{sec:case1}


% We now generalize the procedure described in Section \ref{section:tobeextended} by considering the case in which $m=2$ and $\mu$ is symmetric.
% % 
% Since $\mu$ is symmetric, the asymptotic expected Social Cost of any feasible $\RM$ does not depend on $\pi\in\mathcal{S}_2$.
% % 
% For this reason, in what follows, we fix $\pi=Id$ and search for the best vector $\vec p=(p_1,p_2)$, with $p_1\le p_2$, that induces the optimal ERM.
% % 
% Again, for the sake of simplicity, we restrict our self to consider the Social Cost case.
% % 
% First, we rewrite the objective value of problem \eqref{eq:opt:ERM} in terms of $y_i=F_\mu^{[-1]}(p_i)$ for $i=1,2$.
% % 
% Since $F_\mu^{[-1]}$ is monotone, we have that $y_1\le y_2$.
% % 
% We then have
% \begin{equation}
%     % \label{eq:Wchanged}
%     \mathcal{W}(y_1,y_2)=W_1\Bigg(\mu,F_\mu\Big(\frac{y_1+y_2}{2}\Big)\delta_{y_1}+\Big(1-F_\mu\Big(\frac{y_1+y_2}{2}\Big)\Big)\delta_{y_2}\Bigg).    
% \end{equation}
% Since both $F_\mu$ and $F_\mu^{[-1]}$ are bijective, any $\vec y=(y_1,y_2)$ identifies a unique $\vec p$ and vice-versa.
% % 
% Using the properties of the Wasserstein distances on the line \cite{santambrogio2015optimal}, we obtain
% \begin{equation}
%     \label{eq:Wchanged}
%     \mathcal{W}(y_1,y_2)=\int_{-\infty}^{\frac{y_1+y_2}{2}}|x-y_1|\rho_\mu(x)dx+\int_{\frac{y_1+y_2}{2}}^{+\infty}|x-y_2|\rho_\mu(x)dx.    
% \end{equation}

% We now show that $\mathcal{W}$ is differentiable and compute its gradient.


% \begin{theorem}
% % \label{thm:bestpercsym}
%     Let $\mu$ be a symmetric probability measure.
%     % 
%     Then we have that the function $\mathcal{W}$ is differentiable and its gradient is defined by the formula
%     \[
%     \nabla \mathcal{W}(y_1,y_2)=\Bigg(2F_\mu(y_1)-F_\mu\Big(\frac{y_1+y_2}{2}\Big),2F_\mu(y_2)-1-F_\mu\bigg(\frac{y_1+y_2}{2}\bigg)\Bigg).
%     \]
%     % 
%     Furthermore, $\mathcal{W}$ is twice differentiable.
%     % 
%     Lastly, it holds
%     \[
%     \nabla \mathcal{W}(F_\mu^{[-1]}(0.25),F_\mu^{[-1]}(0.75))=(0,0).
%     \]
% \end{theorem}



% % In general, however, determining the optimal ERM is less trivial.

% % \begin{theorem}
% % % \label{thm:bestpercsym}
% %     Let $\vec q=(q_1,q_2)$ be such that $q_2\le q_1$ and let $\mu$ be a symmetric probability measure.
% %     % 
% %     \begin{enumerate*}[label=(\roman*)]
% %         \item If $0.75\le q_2$, then $\vec p=(0.25,0.75)$ induces the optimal ERM. Moreover, the induced mechanism is asymptotically optimal.
% %         \item If $q_2\in(0.5,0.75)$ and $q_1+q_2\ge \frac{3}{2}$, then $\vec p=(1-q_1,q_2)$ induces the optimal ERM.
% %         \item If $q_2\le 0.5$, then we have that second entry of the best $\vec p$ is $p_2=q_2$. The value of $p_1$ can assume two values: $p_1=F_\mu(\bar y_1)$ if there exists $\bar y_1$ such that $2F_\mu(\bar y_1)=F_\mu(\frac{\bar y_1+F_\mu^{[-1]}(q_2)}{2})$, and $p_1=q_1$ otherwise.
% %     \end{enumerate*}
% % \end{theorem}


% \begin{proof}
% % [Proof of Theorem \ref{thm:bestpercsym}]
%     % 
%     Let $\vec q$ be a p.c.v., due to the symmetry of $\mu$, without loss of generality, we assume that $y_1\le y_2$ are the positions of the facility and that $y_1$ has capacity $q_1$ and $y_2$ has capacity $q_2$.
% % 
%     We then define
%     \begin{align*}
%         \mathcal{W}(y_1,y_2)&=\int_{\erre}\min\{|x-y_1|,|x-y_2|\}\rho_\mu(x)dx\\
%         &=\int_{-\infty}^{y_1}(y_1-x)\rho_\mu(x)dx+\int_{y_1}^{\frac{y_1+y_2}{2}}(x-y_1)\rho_\mu(x)dx\\
%         &\quad +\int_{\frac{y_1+y_2}{2}}^{y_2}(y_2-x)\rho_\mu(x)dx+\int_{y_2}^{+\infty}(x-y_2)\rho_\mu(x)dx\\
%         &=A(y_1,y_2)+B(y_1,y_2)+C(y_1,y_2)+D(y_1,y_2),
%     \end{align*}
%     where
%     \begin{align*}
%         A(y_1,y_2)&=\int_{-\infty}^{y_1}(y_1-x)\rho_\mu(x)dx\\
%         B(y_1,y_2)&=\int_{y_1}^{\frac{y_1+y_2}{2}}(x-y_1)\rho_\mu(x)dx\\
%         C(y_1,y_2)&=\int_{\frac{y_1+y_2}{2}}^{y_2}(y_2-x)\rho_\mu(x)dx\\
%         D(y_1,y_2)&=\int_{y_2}^{+\infty}(x-y_2)\rho_\mu(x)dx.
%     \end{align*}
%     We now compute the derivative of $\mathcal{W}$ with respect to $y_1$ and $y_2$.
%     % 
%     Let us consider the derivative $\partial_{y_1}\mathcal{W}(y_1,y_2)$.
%     % 
%     By definition, we have
%     \[
%     \partial_{y_1}\mathcal{W}(y_1,y_2)=\partial_{y_1}A(y_1,y_2)+\partial_{y_1}B(y_1,y_2)+\partial_{y_1}C(y_1,y_2),
%     \]
%     since $\partial_{y_1}D(y_1,y_2)=0$.
%     % 
%     First, let us consider $\partial_{y_1}A(y_1,y_2)$.
%     % 
%     We have that
%     \begin{align*}
%         \frac{1}{h}\Big(&\int_{-\infty}^{y_1+h}(y_1+h-x)\rho_\mu(x)dx-\int_{-\infty}^{y_1}(y_1-x)\rho_\mu(x)dx\Big)\\
%         &=\frac{1}{h}\Big(h\int_{-\infty}^{y_1+h}\rho_\mu(x)dx-\int_{y_1}^{y_1+h}(y_1-x)\rho_\mu(x)dx\Big)\\
%         &=\int_{-\infty}^{y_1+h}\rho_\mu(x)dx+\frac{1}{h}\int_{y_1}^{y_1+h}(y_1-x)\rho_\mu(x)dx.
%     \end{align*}
%     By the Lebesgue's theorem, we have that 
%     \[
%     \lim_{h\to 0}\frac{1}{h}\int_{y_1}^{y_1+h}(y_1-x)\rho_\mu(x)dx=0,
%     \]
%     thus $\partial_{y_1}A(y_1,y_2)=F_\mu(y_1)$.
%     % 

%     % 
%     Second, let us compute $\partial_{y_1}B(y_1,y_2)$.
%     % 
%     We have that
%     \begin{align*}
%         \frac{1}{h}\Big(&\int_{y_1+h}^{\frac{y_1+y_2}{2}+\frac{h}{2}}(x-y_1-h)\rho_\mu(x)dx-\int_{y_1}^{\frac{y_1+y_2}{2}}(x-y_1)\rho_\mu(x)dx\Big)\\
%         &\frac{1}{h}\Big(-h\int_{y_1+h}^{\frac{y_1+y_2}{2}+\frac{h}{2}}\rho_\mu(x)dx+\int_{\frac{y_1+y_2}{2}}^{\frac{y_1+y_2}{2}+\frac{h}{2}}(x-y_1)\rho_\mu(x)dx\\
%         &\quad\quad\quad -\int_{y_1}^{y_1+h}(x-y_1)\rho_\mu(x)dx \Big).
%     \end{align*}
%     Owing again to Lebesgue's theorem, we have
%     \[
%     \partial_{y_1}B(y_1,y_2)=-\Big(F_\mu\big(\frac{y_1+y_2}{2}\big)-F_\mu(y_1)\Big)+\frac{(y_2-y_1)}{4}\rho_\mu\Big(\frac{y_1+y_2}{2}\Big).
%     \]
%     Finally, we compute $\partial_{y_1}C(y_1,y_2)$.
%     % 
%     We have that
%     \begin{align*}
%         \frac{1}{h}\Big(&\int_{\frac{y_1+y_2}{2}+\frac{h}{2}}^{y_2}(y_2-x)\rho_\mu(x)dx-\int_{\frac{y_1+y_2}{2}}^{y_2}(y_2-x)\rho_\mu(x)dx\Big)\\
%         &\frac{1}{h}\Big(-\int_{\frac{y_1+y_2}{2}}^{\frac{y_1+y_2}{2}+\frac{h}{2}}(y_2-x)\rho_\mu(x)dx \Big).
%     \end{align*}
%     Owing again to the Lebesgue's theorem, we have that
%     \[
%     \partial_{y_1}C(y_1,y_2)=-\frac{y_2-y_1}{4}\rho_\mu\Big(\frac{y_1+y_2}{2}\Big).
%     \]
%     Putting all together, we infer
%     \[
%     \partial_{y_1}\mathcal{W}(y_1,y_2)=2F_\mu(y_1)-F_\mu\Big(\frac{y_1+y_2}{2}\Big).
%     \]
%     Through a similar argument, we have that
%     \[
%     \partial_{y_2}\mathcal{W}(y_1,y_2)=2F_\mu(y_2)-1-F_\mu\bigg(\frac{y_1+y_2}{2}\bigg),
%     \]
%     % 
%     which concludes the first part of the proof.
%     % 

%     % 
%     Since $\mu$ is absolutely continuous, we have that $F_\mu$ is differentiable, thus $\mathcal{W}$ is twice differentiable.
%     % 

%     % 
%     Finally, due to the properties of cumulative distribution functions of symmetric measures, we infer that 
%     \[
%     \nabla \mathcal{W}\Big(F_\mu^{[-1]}(0.25),F_\mu^{[-1]}(0.75)\Big)=(0,0).
%     \]
% \end{proof}

% Now that we have an explicit formula for the gradient of $\mathcal{W}$, we need to express the set of feasible $\vec y$.
% % 
% From Theorem \ref{thm:RM_feasible}, we have that $p_2\le q_1$ and $1-p_2\le q_2$, i.e. $1-q_2\le p_2$.
% % 
% Since $F_\mu^{[-1]}$ is monotone, we have that $y_2=F_\mu^{[-1]}(p_2)\le F_\mu^{[-1]}(q_1)$ and that $F_\mu^{[-1]}(1-q_2)\le y_1$.
% % 
% Therefore we have that the set of feasible $\vec y$ lays in a triangle, namely $T(\vec q)$, whose vertexes are $(F_\mu^{[-1]}(1-q_2),F_\mu^{[-1]}(q_1))$, $(F_\mu^{[-1]}(q_1),F_\mu^{[-1]}(q_1))$, and $(F_\mu^{[-1]}(1-q_2),F_\mu^{[-1]}(1-q_2))$.
% % 

% % To conclude, we retrieve the optimal ERM under the additional assumption that both the facilities are equicapacitated, i.e. $\vec q=(q,q)$ for some $q\in[0.5,1)$.

% % \begin{theorem}
% % \label{thm:sym_distribution}
% %     Given a symmetric probability distribution $\mu$, let $\vec q$ be such that $q_1=q_2=q$.
% %     % 
% %     Then the optimal ERM is induced by the vector $\vec p=(\max\{0.25,1-q\},\min\{0.75,q\})$.
% % \end{theorem}

% % \begin{proof}
% % % [Proof of Theorem \ref{thm:sym_distribution}]
% % Let $\vec q=(q,q)$ be a p.c.v. and let $\mu$ be a symmetric probability measure.
% % % 
% % By Corollary \ref{crr:scale_invariance}, we can assume without loss of generality that the median (or equivalently the mean) of $\mu$ is $0$.
% % % 
% % First, we consider the case $q\ge 0.75$.
% % % 
% % Consider the following minimization problem
% % \begin{equation}
% %     \label{pr:unconstraint}
% %     \min_{\zeta\in\PP_2(\erre)}W_1(\mu,\zeta).
% % \end{equation}
% % Since the set of feasible measures in problem \eqref{pr:unconstraint} contains the set of feasible measures in problem \eqref{eq:min_proj}, we infer
% % \begin{equation}
% %     \label{eq:twoproblemscomaprison}
% %     \min_{\sigma\in \mathcal{S}_2}\min_{\zeta\in\PP_{\sigma,\vec q}(\erre)}W_1(\mu,\zeta)\ge \min_{\zeta\in\PP_2(\erre)}W_1(\mu,\zeta).
% % \end{equation}
% % Since $\mu$ is symmetric, the solution to the left hand side problem has to be symmetric, thus the solution minimizes the function
% % \[
% % y\to\int_0^{+\infty}|x-y|d\mu.
% % \]
% % By Theorem \ref{crr:nsc_best_RM}, we have that the minimum is attained at $y=F_\mu^{[-1]}(0.75)$, since it is the median of $\mu$ restricted on $[0,+\infty)$.
% % % 
% % Then, the solution to problem \eqref{pr:unconstraint} is $\nu=0.5\delta_{F_\mu^{[-1]}(0.25)}+0.5\delta_{F_\mu^{[-1]}(0.75)}$.
% % % 
% % Lastly, since $0.5\le q$ and since $\vec p=(0.25,0.75)$ satisfies \eqref{eq:feas_system}, we infer that $Id$ and $\vec p=(0.25,0.75)$ is feasible for the left hand side problem in \eqref{eq:twoproblemscomaprison}, thus it is also a solution to it.
% % % 
% % Finally, by Theorem \ref{thm:suff_condition_asymptoticopt}, we infer that $\texttt{ERM}^{(Id,(0.25,0.75))}$ is optimal when $\vec q=(q,q)$ with $q\ge 0.75$.
% % % 


% % % 
% % Let us now consider the case in which $\vec q=(q,q)$ with $q\in[0.5,0.75)$.
% % % 
% % First, let us define $z=F_\mu^{[-1]}(q)$.
% % % 
% % Since $a\mu$ is symmetric and its mean is $0$, we have that $F_\mu^{[-1]}(1-q)=-z$.
% % % 
% % Consider the following minimization problem 
% % \begin{equation}
% %     \label{pr:unconstraint_add}
% %     \min_{\zeta\in\PP_{2,z}(\erre)}W_1(\mu,\zeta),
% % \end{equation}
% % where $\PP_{2,z}(\erre)$ is the set of measures $\zeta\in\PP_{2}(\erre)$ such that $spt(\zeta)\subset [-z,z]$.
% % % 
% % Since $\mu$ is symmetric, we have that the solution to this problem is such that $\nu=0.5\delta_{-r}+0.5\delta_{r}$, where $r\in[0,z]$.
% % % 
% % By the same argument used to prove Theorem \ref{crr:nsc_best_RM}, we infer that the solution to problem \eqref{pr:unconstraint_add} is $\nu=0.5\delta_{-z}+0.5\delta_{z}$.
% % % 
% % To conclude, we notice that, by Theorem \ref{thm:limitBAR}, the limit expected Social Cost of $\texttt{ERM}^{(Id,(1-q,q)}$ is equal to $W_1(\mu,0.5\delta_{-z}+0.5\delta_{z})$, which concludes the proof.
% % \end{proof}

% % 
% % When $q_2\in(0.5,0.75)$ and $q_1+q_2<1.5$, to retrieve the optimal vector $\vec p$ we need to solve the minimization problem in \eqref{eq:opt:ERM}. \newline
% % 

% \textbf{Asymmetric probability distributions $\mu$.} Finally, we want to stress that the procedure outlined above, it is applicable also for non-symmetric measures as long as the two facilities have the same capacity.
% % 
% Indeed, in this case, the permutation we chose is irrelevant, since the facilities have the same capacity and thus are interchangeable.
% % 
% In this case, we can still compute the derivative of the objective function and retrieve the optimal $\vec p$ based on how the set $T(\vec q)$ intersects the set of points in which the derivatives of $\mathcal{W}$ are equal to $0$.
% % 
% Of course, in this case, the point $(F_\mu^{[-1]}(0.25),F_\mu^{[-1]}(0.75))$ is no longer necessarily a point on which the gradient $\nabla \mathcal{W}$ nullifies.


% \subsection{Optimal Extended Ranking Mechanisms in the Generic Framework}

% Lastly, we propose a sufficient and necessary condition that guarantees the existence of an optimal ERM whose limit Bayesian approximation ratio converges to $1$ that is applicable regardless of $m$ and $\mu$.


% \begin{theorem}
% \label{thm:suff_condition_asymptoticopt}
%     Give $\mu$ and $\vec q$, let $(\pi,\nu_{m})$ be a solution to Problem \eqref{eq:min_proj}.
%     % 
%     We denote with $\{y_j\}_{j\in[m]}$ the points in the support of $\nu_{m}$ ordered non-decreasingly, and set $y_0=-\infty$ and $y_{m+1}=+\infty$.
%     % 
%     Finally, we define $\zeta_j=F_\mu(y_{j+1})-F_\mu(y_{j-1})$ and denote with $\hat \pi\in\mathcal{S}_m$ a permutation that orders the values $\zeta_j$ in a non-increasing order.
%     % 
%     Then, the optimal ERM has limit Bayesian approximation ratio equal to $1$ if and only if $\zeta_{\hat \pi(j)}\le q_j$ for every $j\in [m]$.
% \end{theorem}


% \begin{proof}[Proof of Theorem \ref{thm:suff_condition_asymptoticopt}]
%     Let $(\sigma,\nu_{m})$ be a solution to \eqref{eq:min_proj}.
%     % 
%     Since $\nu_{m}\in\PP_m(\erre)$, we have $spt(\nu_{m})=\{y_j\}_{j\in[m]}$.
%     % 
%     Let us define $p_j=F_\mu(y_j)$.
%     % 
%     Furthermore, let us fix $\gamma=\hat \pi^{-1}\in\mathcal{S}_m$.
%     % 
%     By definition of $p_j$ and by hypothesis, we have that $p_{j+1}-p_{j-1}=F_\mu(y_{j+1})-F_\mu(y_{j-1})\le q_{\gamma(j)}$ for every $j\in[m]$, hence $\texttt{ERM}^{(\gamma,\vec p)}$ is feasible (Theorem \ref{thm:RM_feasible}).
%     % 
%     Owing to Theorem \ref{thm:limitBAR}, the asymptotic expected Social Cost of $\texttt{ERM}^{(\gamma,\vec p)}$ converges to $W_1(\mu,\nu_{\vec p})$, where $\nu_{\vec p}$ is a solution to 
%     \begin{equation}
%     \label{eq:probl_+contrst}
%       \min_{\lambda_j\le q_{\gamma(j)},\sum_{j\in[m]\lambda_j=1}}W_1\Big(\mu,\sum_{j\in[m]}\lambda_j\delta_{y_j}\Big)  
%     \end{equation}
%     % 
%     since, by definition, we have $p_j=F_\mu(y_j)$.
%     % 

%     % 
%     To conclude, we need to show that $(\gamma,\nu_{\vec p})$ is a solution to \eqref{eq:min_proj}.
%     % 
%     Due to the optimality of $\sigma\in\mathcal{S}_m$, it suffices to show that 
%     \[
%     \min_{\zeta\in\PP_{\sigma,m}(\erre)}W_1(\mu,\zeta)\ge W_1(\mu,\nu_{\vec p}).
%     \]
%     % 
%     First, let us consider the following minimization problem 
%     \begin{equation}
%         \label{eq:unconstr_pr}
%         \min_{\sum_{j\in [m]}\lambda_j=1}W_1\Big(\mu,\sum_{j\in[m]}\lambda_j\delta_{y_j}\Big).
%     \end{equation} 
%     % 
%     Notice that the only difference between problem \eqref{eq:unconstr_pr} and problem \eqref{eq:probl_+contrst} are the constraints $\lambda_j\le q_{\sigma(j)}$.
%     % 
%     Let us now consider the probability measure $\nu=\sum_{j\in[m]}(F_\mu(z_j)-F_\mu(z_{j-1}))\delta_{y_j}$, where $z_j=\frac{y_{j}+y_{j+1}}{2}$ for every $j\in[m-1]$, $z_0=-\infty$, and $z_m=+\infty$.
%     % 
%     Since the optimal transportation plan between two measures on a line is monotone (see Theorem 2.9, \cite{santambrogio2015optimal}), we infer
%     \[
%         W_1(\mu,\nu)=\int_{\erre\times \erre}\min_{j\in[m]}|x-y_j|\,d\mu,
%     \]
%     thus $\nu$ is a minimizer of problem \eqref{eq:unconstr_pr}.
%     % 
%     Finally, since $F_\mu$ is monotone increasing, it holds $F_\mu(z_j)-F_\mu(z_{j-1})\le F_\mu(y_{j+1})-F_\mu(y_{j-1})\le q_{\gamma(j)}$.
%     % 
%     In particular, $\nu$ is feasible for problem \eqref{eq:probl_+contrst}, thus $W_1(\mu,\nu)=W_1(\mu,\nu_{\vec p})$.
%     % 
%     Likewise, $\nu_m$ is feasible for problem \eqref{eq:unconstr_pr}, thus $W_1(\mu,\nu_{\vec p})=W_1(\mu,\nu)\le W_1(\mu,\nu_{m})$, which concludes the proof.
% \end{proof}







% \section{Extension to Higher Dimension}

% % 
% In this section, we study under which assumptions it is possible to adapt the ERM to define a mechanism capable of locating $m$ capacitated facilities in higher dimensional spaces.
% % 
% In this case, we denote with $x^{(i)}\in\erre^d$ the position of the $i$-th agent.
% % 
% We denote with $x^{(i)}_\ell$ the $\ell$-th coordinate of $x^{(i)}$.
% % 
% Given a p.c.v. $\vec q\in[0,1]^m$ and a permutation $\pi\in\mathcal{S}_m$, we denote with $y^{(j)}$ the position of the facility whose capacity is $q_{\pi(j)}$.
% % 
% We denote with $y^{(j)}_r$ the $r$-th coordinate of the location $y^{(j)}$.
% % 
% Lastly, we denote with $\Gamma\subset [n]\times [m]$ the agents-to-facility matching.
% % 

% \begin{mechanism}
%     Let $\vec q\in[0,1]^m$ be a p.c.v. and $\pi\in\mathcal{S}_m$ be a permutation. 
%     % 
%     Given $d$ $m$-dimensional vectors $\vec v^{(j)}\in[0,1]^m$, the High-dimensional Extended Ranking Mechanism (HERM) associated with $\vec V=\{\vec v^{(j)}\}_{j\in[m]}$ is a mechanism whose routine is defined as follows
%     \begin{enumerate}[label=(\roman*)]
%         \item the mechanism gathers the reports of the $n$ agents, namely $\{x^{(i)}\}$.
%         \item For every $l\in[d]$, it defines the vectors $\vec z^{(l)}$ containing the $l$-th coordinate of all the agents' reports.
%         \item Then the mechanism defines the position of  $j$-th facility, namely $y^{(j)}$, by setting $y_i^{(j)}=z_{\floor{v_j^{(i)} (n-1)}+1}^{(i)}$. then it assigns to this location the capacity $q_{\pi(j)}$.
%         \item Finally, every agent is assigned to the facility that is closer to the position they reported.
%     \end{enumerate}
% \end{mechanism}

% Unlike what happens for the mechanisms used for the $m$-FLP, applying truthful $1$-dimensional mechanisms along each set of coordinates does not guarantee that the resulting mechanism is truthful.
% % 
% This is due to the fact that, in the $m$-CFLP, we need to place the facilities and also assign the agents to them.
% % 
% While the line has a total ordering over them, this is no longer true for higher dimensional spaces, as the next example shows.

% \begin{example}
%     Let us consider the following instance $q_1=q_2=0.7$, $n=20$, and $m=2$.
%     % 
%     Let us consider the vector $\vec v=(0.5,0.55)$.
%     % 
%     Notice that the ERM induced by $\vec v$ is truthful and well-defined.
%     % 
%     However, the HERM induced by $\vec V=\{\vec v,\vec v\}$ and $\pi=Id$ does not always return a feasible facility location.
%     % 
%     Consider for example the instance $\vec x ^{(1)}=\dots=\vec x^{(9)}=(-1,1.5)$, $\vec x^{(10)}=(0,1)$, $\vec x^{(11)}=(1,0)$, and $\vec x^{(12)}=\dots=\vec x^{(20)}=(1.5,-1)$.
%     % 
%     It is easy to check that the HERM induced by $\vec V$ places the facilities at $\vec y^{(1)}=(0,0)$ and $\vec y^{(2)}=(1,1)$, hence at least $18$ agents are closer to $\vec y^{(1)}$ than to $\vec y^{(2)}$.
%     % 
%     Finally, notice that both the capacities of the facilities are equal to $14$, thus the output of the HERM is not feasible, even though the ERM associated with $\vec v$ and $Id$ is feasible (see Theorem \ref{}).
%     % 
%     It is also worth of notice that the ERM induced by $\vec v$ coincides with the Innerpoint mechanism, proving that trivially extending one dimensional truthful mechanisms do not define a truthful and feasibile mechanism.
% \end{example}

% In what follows, we characterize the set of conditions under which the HERM are truthful.
% % 
% For the sake of simplicity, we consider only the case in which $d=2$, when $d>2$, the conditions are easy to generalize.
% % 


% \subsection{Case \texorpdfstring{$m=2$}{}}

% First, we assume that we have to facilities to prove.
% % 
% In example \ref{}, we have shown that there are instances in which all the agents are closer to the same facility.
% % 
% The next theorem shows that this is always the case for HERM induced by $\vec V$ such that $v^{(1)}_1\neq v_1^{(2)}$ and $v^{(1)}_2\neq v^{(2)}_2$.
% % 

% \begin{theorem}
% \label{thm:feasiblitycondhigherdim}
%     Let $\vec q\in [0,1]^2$ a p.c.v. and let $\pi\in\mathcal{S}_m$ be a permutation.
%     % 
%     Then the HERM induced by $\vec V=\{\vec v^{(1)},\vec v^{(2)}\}$ and $\pi$ is feasible if and only if one of the following two holds
%     % 
%     \begin{itemize}
%         \item $v_1^{(1)}=v_1^{(2)}$, $v_2^{(2)}\le q_{\pi(1)}$, and $1-v_2^{(1)}\le q_{\pi(2)}$; or
%         \item $v_2^{(1)}=v_2^{(2)}$, $v_1^{(2)}\le q_{\pi(1)}$, and $1-v_1^{(1)}\le q_{\pi(2)}$.
%     \end{itemize}
%     % 
% \end{theorem}

% \begin{proof}
%     blablabla
% \end{proof}

% % 
% We now study the Bayesian approximation ratio of any feasible HERM.
% % 
% We recall that for higher dimensional problems, the cost
% % 

% \begin{theorem}
% \label{thm:higherdimensionalSC}
%     Given $\vec q\in[0,1]^2$, let $\pi\in\mathcal{S}_m$ and $\vec V$ induce a feasible HERM according to the conditions of Theorem \ref{thm:feasiblitycondhigherdim}.
%     % 
%     We denote with $\mu\in\PP(\erre^2)$ be a probability measure and let $\mu_1$ and $\mu$ be the marginal of $\mu$ with respect to the first and second variable, respectively.
%     % 
%     Then, we have that
%     \begin{equation}
%         \lim_{n\to\infty}\frac{\EE[\SCo_{(\pi,\vec V)}(\vec x)]}{\EE[\SCo_{opt}(\vec x)]}=\frac{W_1(\mu,\nu_{\vec V})}{W_1(\mu,\nu_2)},
%     \end{equation}
%     where $\nu_{\vec V}=\alpha\delta_{\vec y_1}+(1-\alpha)\delta_{\vec y^{(2)}}$ with $\vec y^{(i)}=(F_{\mu_1}^{[-1]}(\vec v_1^{(i)}),F_{\mu_2}^{[-1]}(\vec v_2^{(i)}))$, and 
%     \[
%         \alpha=\begin{cases}
%                     F_{\mu_2}(\frac{y_2^{(1)}+y_2^{(2)}}{2}) \quad &\text{if } \quad v_1^{(1)}=v_1^{(2)}\\
%                     F_{\mu_1}(\frac{y_1^{(1)}+y_1^{(2)}}{2}) \quad &\text{if } \quad v_2^{(1)}=v_2^{(2)}
%                 \end{cases}.
%     \]
%     While $\nu_2$ is the solution to $\min_{\sigma\in\mathcal{S}_2}\min_{\nu\in\PP_{2,\sigma}(\erre^2)}W_1(\mu,\nu)$.
%     %
% \end{theorem}

% \begin{proof}
%     sad
% \end{proof}


% Before we move to analyse the case in which we have more than $2$ facilities to place, we want to stress two points
% \begin{enumerate}
%     \item We can extend everything to other mechanisms that can places two capacitated facilities on a line.
%     \item Theorem \ref{thm:higherdimensionalSC} is stated only for the Social Cost, however, following the arguments used in Section \ref{sect:extlpMC}, it is possible to extend the theorem to encompass the $l_p$ cost and the Maximum Cost. Again, notice that in order to have a bounded limit Bayesian approximation ratio, we need to assume that either
%     \[
%         \int_{\erre^d}|x|^pd\mu<+\infty
%     \]
%     or that the support of $\mu$ is compact.
% \end{enumerate}


% \subsection{Case \texorpdfstring{$m>2$}{}}





% \section{Numerical Experiments}
% \label{sec:experiment}

% In this section, we complement our theoretical study of the ERMs by running several numerical experiments.
% % 
% Indeed, most of our results pertain to the limit analysis of the mechanism. For this reason, we want to test two aspects of the ERMs.
% % 
% First, we want to compare the Bayesian approximation ratio of the ERMs with the Bayesian approximation ratios of other truthful mechanisms when the number of agents $n$ is small.
% % 
% Since the Ranking Mechanisms are a subset of the ERMs and have been discussed in Section \ref{sec:case2}, we only consider the EEM and, when possible, the IG.
% % 
% Second, we want to evaluate the convergence speed of the Bayesian approximation ratio of $\RM$.
% % 
% More specifically, we want to assess how close the Bayesian approximation ratio of an ERM and the limit detected in Theorem \ref{thm:limitBAR} are when the number of agents is small. 
% % 
% We run our experiments for different distributions $\mu$ and percentage capacity vector $\vec{q}$. 
% % 
% All the experiments are performed in Matlab 2023a on macOS Monterey system with Apple M1 Pro CPU and 16GB RAM.
% % 
% The code is available on \url{https://anonymous.4open.science/r/Bayesian-CFLP-38D5/}. 

% \paragraph{Experiment setup}
% Throughout our experiments, we sample the agents' positions from three probability distributions: the uniform distribution $\mathcal{U}[0,1]$, the standard normal distribution $\mathcal{N}(0,1)$, and the exponential distribution $\text{Exp}(1)$.
% % 
% Owing to Corollary \ref{crr:scale_invariance}, we do not consider other parameter choices since testing the mechanisms over the standard Gaussian distribution is the same as testing over $\mathcal{N}(\mathfrak{m},\sigma^2)$. 
% % 
% % Since our goal is to compare the performances of the ERMs to other relevant mechanisms, we limit our tests to cases in which $m=2$, as all the known truthful mechanisms different from the Ranking Mechanisms operate only under this restriction.
% % 
% To compare the ERMs to other mechanisms, we limit our tests to cases in which $m=2$, as all the known truthful mechanisms different from the Ranking Mechanisms operate only under this restriction.
% % 
% We consider different percentage capacity vectors $\vec q\in (0,1)^2$. 
% % 
% Specifically, we consider balanced capacities $\vec{q}=(q,q)$ and unbalanced capacities $\vec{q}=(q_1, q_2), q_1 \neq q_2$. For the case of balanced capacities, we set $q=0.7,0.8$ and $0.9$. 
% % 
% For the case of unbalanced capacities, we consider the slightly unbalanced capacities i.e. $\vec{q}=(0.85,0.75)$, and extremely unbalanced capacities i.e. $\vec{q}=(0.8,0.4)$, $(0.85,0.35)$.
% % 
% As benchmark mechanisms, we consider the EEM \cite{aziz2020facility} and, when possible, the IG \cite{ijcai2022p75}.


% \paragraph{Experiment results -- Comparison with the EEM and the IG} 
% % 
% We first consider the case of balanced capacities $\vec q=(q,q)$, in which we are able to compare the Bayesian approximation ratio of three different mechanisms for the $m$-CFLP: the EEM, the IG, and the ERMs.
% % 
% Regardless of the distribution, we consider the optimal ERM with respect to the uniform distribution, i.e. $\RM$, with $\pi=Id$ and $\vec v=(\max\{0.25,1-q\},\min\{0.75,q\})$.
% % 
% Figure~\ref{fig:EQ} (and Table 1 in Appendix D) 
% % 
% % Figure~\ref{fig:EQ} (and Table ~\ref{table:equicapacitated_test} in \ref{sec:results})
% % 
% shows the average and the $95\%$ confidence interval (CI) of Bayesian approximation ratio for $n=10,20,30,40,50$.
% % 
% Each average is computed over $500$ instances.
% % 
% We observe that, in most cases, the ERM achieves the lowest Bayesian approximation ratio comparing to the other two mechanisms. 
% % 
% When $q=0.7$, the ERM is still better than the EEM but slightly worse than the IG. However, the empirical Bayesian approximation ratio of the ERM and IG converges to the same value as the number of agents increases.
% % 

% % 
% % We then consider the  unbalanced capacities case $q_1\neq q_2$, in particular $\vec q=(0.85,0.75),(0.8,0.4),(0.85,0.35)$.
% Next, we consider the case of unbalanced capacities, where $q_1\neq q_2$, specifically $\vec q=(0.85,0.75),(0.8,0.4),(0.85,0.35)$.
% % 
% Since the IG requires the two capacities to be identical, we compare only the ERM and the EEM.
% % 
% Amongst the possible ERMs, we select the one optimal with respect to the Uniform distribution, obtained via Theorem \ref{thm:bestuniform}.
% % 
% Thus the parameters of $\RM$ are
% \begin{enumerate*}[label=(\roman*)]
%     \item $\pi=Id$ for every $\vec q$ and
%     \item $\vec v=(0.25,0.75)$ for $\vec q=(0.85,0.75)$, $\vec v=(0.6,0.8)$ for $\vec q=(0.8,0.4)$, and $\vec v=(0.65,0.85)$ for $\vec q=(0.85,0.35)$.
% \end{enumerate*}
% % 
% In this case, we consider only symmetric probability distributions, i.e. the Gaussian and the Uniform distribution.
% % 
% Figure~\ref{fig:NE} (and Table 2 in Appendix D)
% % Figure~\ref{fig:NE} (and Table ~\ref{table:nonequitest} in \ref{sec:results}) 
% shows the average and the $95\%$ CI of Bayesian approximation ratio computed over 500 instances.
% % 
% Whenever $n\ge 20$, the ERM has a much lower approximation ratio.
% % 
% Notice that when $\vec q=(0.75,0.85)$, the ERM is optimal in both cases, and its limit Bayesian approximation ratio is $1$.
% % 
% Indeed, the Bayesian approximation ratio of the ERM is almost equal to $1$ for every $n\ge  10$ and gets closer as $n$ increases, however the Bayesian approximation ratio of the EEM is always $\ge 1.79$ and gets worse as $n$ increases. 
% % 
% % In Appendix ~\ref{sec:results} we report theThe numbers can be found in Table ~\ref{table:equicapacitated_test} and \ref{table:nonequitest} of .}


% \begin{figure}[t!]
%      \centering
%      \includegraphics[width=\columnwidth]{figs/figEQ_CI.png}
%      \caption{The Bayesian approximation ratio of ERM, IG, and EEM in the balanced case, i.e. $q_1=q_2$ for $n=10,20,\dots,50$.
% % 
% Every column contains the results for different vector $\vec q$.
% %
% The first row contains the results for the Uniform distribution, the second row the results for the Gaussian distribution, and the third one the results for the Exponential distribution. 
% % 
% % Every value is computed as the average of $500$ runs.
% }
%      \label{fig:EQ}
% \end{figure}
% \vspace{-0.1cm}

% \begin{figure}[t!]
%      \centering
%      \includegraphics[width=0.975\columnwidth]{figs/figNE_CI.png}
%      \caption{The Bayesian approximation ratio of ERM and EEM in the unbalanced case, i.e. $q_1\neq q_2$ for $n=10,20,\dots,50$. 
% % 
% Every column contains the results for a different vector $\vec q$.
% % 
% The first row contains the results for the Uniform distribution.
% % 
% The second row contains the results for the Gaussian distribution.
% %
% % Every value is computed as the average of $500$ runs.
% }
%      \label{fig:NE}
% \end{figure}


% \paragraph{Experiment results -- Convergence speed of the limit Bayesian approximation ratio.} 

% Lastly, we test how close the Bayesian approximation ratio of the ERM is to the limit detected in Theorem \ref{thm:limitBAR}. 
% % 
% That is, we calculate the relative error as $err_{rel}=\frac{\text{empirical } B_{ar}-\text{limit of } B_{ar}}{\text{limit of } B_{ar}}.$
% % 
% Figure~\ref{fig:RE} (and Table 3 in Appendix D)
% % 
% % Figure~\ref{fig:RE} (and Table \ref{table:percenterrtest} in Appendix ~\ref{sec:results}) 
% show the relative error for the six cases.
% % 
% Each average is computed over $500$ instances.
% % 
% % In all the cases, w
% % 
% We observe that the relative error decreases as the number of agents increases, regardless of the distribution or the p.c.v. $\vec q$.
% % 
% Moreover, in all cases but $\vec q=(0.8,0.4),(0.85,0.35)$, the relative errors of the ERM are less than $0.05$ as long as $n \ge 20$, which validates Theorem~\ref{thm:limitBAR} as a tool to predict the Bayesian approximation ratio for small values of $n$.
% % 
% In other cases, we observe a slower convergence, as the percentage error is slightly larger and its highest value is $0.33$. 
% % 

% \section{Additional Experimental Results}
% \label{sec:results}

% In this Appendix, we report the values plotted in Figure \ref{fig:EQ}, \ref{fig:NE}, and \ref{fig:RE}.
% % 
% In particular, Table \ref{table:equicapacitated_test} reports the Bayesian approximation ratios for the balanced case, plotted in Figure \ref{fig:EQ}.
% % 
% Table \ref{table:nonequitest} reports the values of the Bayeisan approximation ratios for the unbalanced case, plotted in Figure \ref{fig:NE}.
% % 
% Finally, in Table \ref{table:percenterrtest}, we report the values of the relative error of the Bayesian approximation ratios, plotted in Figure \ref{fig:RE}.



% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[ht]
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{c|c|c|ccc|ccc|ccc|ccc|ccc}
% \toprule
% \multirow{2}{*}{p.c.v. $\vec{q}$} & \multirow{2}{*}{Measure $\mu$} & \multirow{2}{*}{Mech.} & \multicolumn{3}{c|}{$n=10$} & \multicolumn{3}{c|}{20} & \multicolumn{3}{c|}{30} & \multicolumn{3}{c|}{40} & \multicolumn{3}{c}{50} \\ 
%                                   &                                &                        & lb      & mean    & ub     & lb     & mean  & ub    & lb     & mean  & ub    & lb     & mean  & ub    & lb     & mean  & ub    \\ \hline
% \multirow{9}{*}{$(0.7,0.7)$}      & \multirow{3}{*}{Uniform}                        & ERM                    & 1.12    & 1.14    & 1.16   & 1.09   & 1.10  & 1.11  & 1.07   & 1.08  & 1.09  & 1.07   & 1.07  & 1.08  & 1.06   & 1.06  & 1.07  \\
%                                   &                                & IG                     & 1.04    & 1.04    & 1.05   & 1.04   & 1.05  & 1.05  & 1.04   & 1.05  & 1.05  & 1.05   & 1.05  & 1.05  & 1.04   & 1.05  & 1.05  \\
%                                   &                                & EEM                    & 1.77    & 1.81    & 1.85   & 1.87   & 1.90  & 1.93  & 1.91   & 1.93  & 1.95  & 1.95   & 1.97  & 1.99  & 1.95   & 1.96  & 1.98  \\ \cline{2-18}
%                                   & \multirow{3}{*}{Gaussian}                       & ERM                    & 1.11    & 1.13    & 1.15   & 1.07   & 1.08  & 1.09  & 1.06   & 1.06  & 1.07  & 1.06   & 1.06  & 1.07  & 1.05   & 1.06  & 1.06  \\
%                                   &                                & IG                     & 1.04    & 1.05    & 1.06   & 1.04   & 1.05  & 1.05  & 1.04   & 1.04  & 1.05  & 1.04   & 1.05  & 1.05  & 1.04   & 1.04  & 1.05  \\
%                                   &                                & EEM                    & 2.05    & 2.10    & 2.14   & 2.60   & 2.65  & 2.71  & 2.87   & 2.93  & 2.98  & 3.04   & 3.09  & 3.15  & 3.19   & 3.24  & 3.30  \\ \cline{2-18}
%                                   & \multirow{3}{*}{Exp. }                          & ERM                    & 1.26    & 1.30    & 1.34   & 1.15   & 1.16  & 1.17  & 1.14   & 1.15  & 1.16  & 1.12   & 1.13  & 1.14  & 1.12   & 1.13  & 1.14  \\
%                                   &                                & IG                     & 1.08    & 1.09    & 1.10   & 1.07   & 1.08  & 1.09  & 1.09   & 1.10  & 1.11  & 1.09   & 1.09  & 1.10  & 1.09   & 1.10  & 1.11  \\ 
%                                   &                                & EEM                    & 2.60    & 2.72    & 2.84   & 3.82   & 4.01  & 4.20  & 4.81   & 5.00  & 5.20  & 5.67   & 5.89  & 6.11  & 6.05   & 6.28  & 6.52  \\ \hline \hline
% \multirow{9}{*}{$(0.8,0.8)$}      & \multirow{3}{*}{Uniform}                        & ERM                    & 1.15    & 1.18    & 1.20   & 1.04   & 1.05  & 1.06  & 1.03   & 1.04  & 1.04  & 1.02   & 1.02  & 1.03  & 1.02   & 1.02  & 1.02  \\
%                                   &                                & IG                     & 1.18    & 1.19    & 1.20   & 1.12   & 1.12  & 1.13  & 1.09   & 1.09  & 1.10  & 1.08   & 1.08  & 1.08  & 1.07   & 1.07  & 1.07  \\
%                                   &                                & EEM                    & 1.74    & 1.78    & 1.81   & 1.88   & 1.91  & 1.94  & 1.91   & 1.93  & 1.95  & 1.93   & 1.95  & 1.97  & 1.95   & 1.97  & 1.99  \\ \cline{2-18}
%                                   & \multirow{3}{*}{Gaussian}                       & ERM                    & 1.13    & 1.15    & 1.17   & 1.04   & 1.04  & 1.05  & 1.03   & 1.04  & 1.04  & 1.02   & 1.02  & 1.03  & 1.02   & 1.02  & 1.03  \\
%                                   &                                & IG                     & 1.19    & 1.20    & 1.21   & 1.11   & 1.12  & 1.12  & 1.09   & 1.09  & 1.10  & 1.07   & 1.08  & 1.08  & 1.07   & 1.07  & 1.07  \\
%                                   &                                & EEM                    & 2.00    & 2.04    & 2.08   & 2.47   & 2.51  & 2.56  & 2.82   & 2.86  & 2.91  & 2.99   & 3.04  & 3.08  & 3.16   & 3.21  & 3.26  \\ \cline{2-18}
%                                   & \multirow{3}{*}{Exp.}                           & ERM                    & 1.29    & 1.33    & 1.37   & 1.13   & 1.15  & 1.17  & 1.11   & 1.12  & 1.13  & 1.08   & 1.09  & 1.09  & 1.08   & 1.09  & 1.10  \\
%                                   &                                & IG                     & 1.14    & 1.15    & 1.16   & 1.11   & 1.12  & 1.12  & 1.09   & 1.10  & 1.10  & 1.07   & 1.08  & 1.08  & 1.07   & 1.08  & 1.08  \\
%                                   &                                & EEM                    & 1.85    & 1.92    & 2.00   & 2.66   & 2.79  & 2.93  & 3.51   & 3.70  & 3.88  & 4.18   & 4.40  & 4.63  & 4.36   & 4.56  & 4.76  \\ \hline \hline
% \multirow{9}{*}{$(0.9,0.9)$}      & \multirow{3}{*}{Uniform}                        & ERM                    & 1.14    & 1.16    & 1.18   & 1.04   & 1.05  & 1.05  & 1.03   & 1.04  & 1.04  & 1.02   & 1.02  & 1.03  & 1.02   & 1.02  & 1.02  \\
%                                   &                                & IG                     & 1.72    & 1.75    & 1.78   & 1.52   & 1.54  & 1.55  & 1.46   & 1.48  & 1.49  & 1.44   & 1.45  & 1.46  & 1.42   & 1.43  & 1.44  \\
%                                   &                                & EEM                    & 1.72    & 1.75    & 1.78   & 1.86   & 1.88  & 1.91  & 1.92   & 1.94  & 1.97  & 1.93   & 1.96  & 1.98  & 1.96   & 1.98  & 2.00  \\ \cline{2-18}
%                                   & \multirow{3}{*}{Gaussian}                       & ERM                    & 1.12    & 1.14    & 1.16   & 1.04   & 1.04  & 1.05  & 1.03   & 1.04  & 1.04  & 1.02   & 1.03  & 1.03  & 1.02   & 1.02  & 1.02  \\
%                                   &                                & IG                     & 1.99    & 2.03    & 2.06   & 1.67   & 1.69  & 1.71  & 1.58   & 1.60  & 1.61  & 1.54   & 1.56  & 1.57  & 1.51   & 1.53  & 1.54  \\
%                                   &                                & EEM                    & 1.99    & 2.03    & 2.06   & 2.48   & 2.53  & 2.57  & 2.77   & 2.82  & 2.86  & 3.00   & 3.05  & 3.09  & 3.09   & 3.14  & 3.18  \\ \cline{2-18}
%                                   & \multirow{3}{*}{Exp.}                           & ERM                    & 1.35    & 1.39    & 1.43   & 1.14   & 1.15  & 1.17  & 1.12   & 1.13  & 1.15  & 1.08   & 1.09  & 1.10  & 1.09   & 1.10  & 1.11  \\
%                                   &                                & IG                     & 1.64    & 1.67    & 1.70   & 1.41   & 1.42  & 1.44  & 1.36   & 1.38  & 1.39  & 1.32   & 1.33  & 1.34  & 1.31   & 1.32  & 1.32  \\
%                                   &                                & EEM                    & 1.64    & 1.67    & 1.70   & 2.00   & 2.08  & 2.16  & 2.20   & 2.31  & 2.42  & 2.49   & 2.63  & 2.76  & 2.68   & 2.83  & 2.97  \\
% \bottomrule
% \end{tabular} }
% \caption{The Bayesian approximation ratio of ERM, IG, and EEM in the balanced case, i.e. $q_1=q_2$. 
% Every row contains the results for different mechanism, measure $\mu$, and vector $\vec q$. 
% Every column contains the results for different $n\in \{10,20,\ldots,50\}$.
% Every value is computed as the average of $500$ runs.}
% \label{table:equicapacitated_test}
% \end{table*}

% %\begin{table}[ht]
% %\centering
% %\begin{adjustbox}{max width=\columnwidth}
% %\begin{tabular}{c|c|c|ccccc}
% %\toprule
% %p.c.v. $\vec{q}$             & Measure $\mu$             & Mech. & $n=10$ & 20   & 30   & 40   & 50   \\ \hline
% %\multirow{9}{*}{$(0.7,0.7)$} & \multirow{3}{*}{Uniform}  & ERM   & 1.14   & 1.10 & 1.08 & 1.07 & 1.06 \\
% %                             &                           & IG    & 1.04   & 1.05 & 1.05 & 1.05 & 1.05 \\
% %                             &                           & EEM   & 1.81   & 1.90 & 1.93 & 1.97 & 1.96 \\ \cline{2-8} 
% %                             & \multirow{3}{*}{Guassian} & ERM   & 1.13   & 1.08 & 1.06 & 1.06 & 1.06 \\
% %                             &                           & IG    & 1.05   & 1.05 & 1.04 & 1.05 & 1.04 \\
% %                             &                           & EEM   & 2.10   & 2.65 & 2.93 & 3.09 & 3.24 \\ \cline{2-8} 
% %                             & \multirow{3}{*}{Exp.}     & ERM   & 1.30   & 1.16 & 1.15 & 1.13 & 1.13 \\
% %                             &                           & IG    & 1.09   & 1.08 & 1.10 & 1.09 & 1.10 \\
% %                             &                           & EEM   & 2.72   & 4.01 & 5.00 & 5.89 & 6.28 \\ \hline \hline
% %\multirow{9}{*}{$(0.8,0.8)$} & \multirow{3}{*}{Uniform}  & ERM   & 1.18   & 1.05 & 1.04 & 1.02 & 1.02 \\
% %                             &                           & IG    & 1.19   & 1.12 & 1.09 & 1.08 & 1.07 \\
% %                             &                           & EEM   & 1.78   & 1.91 & 1.93 & 1.95 & 1.97 \\ \cline{2-8} 
% %                             & \multirow{3}{*}{Gaussian} & ERM   & 1.15   & 1.04 & 1.04 & 1.02 & 1.02 \\
% %                             &                           & IG    & 1.20   & 1.12 & 1.09 & 1.08 & 1.07 \\
% %                             &                           & EEM   & 2.04   & 2.51 & 2.86 & 3.04 & 3.21 \\ \cline{2-8} 
% %                             & \multirow{3}{*}{Exp.}     & ERM   & 1.33   & 1.15 & 1.12 & 1.09 & 1.09 \\
% %                             &                           & IG    & 1.15   & 1.12 & 1.10 & 1.08 & 1.08 \\
% %                             &                           & EEM   & 1.92   & 2.79 & 3.70 & 4.40 & 4.56 \\ \hline \hline
% %\multirow{9}{*}{$(0.9,0.9)$} & \multirow{3}{*}{Uniform}  & ERM   & 1.16   & 1.05 & 1.04 & 1.02 & 1.02 \\
% %                             &                           & IG    & 1.75   & 1.54 & 1.48 & 1.45 & 1.43 \\
% %                             &                           & EEM   & 1.75   & 1.88 & 1.94 & 1.96 & 1.98 \\ \cline{2-8} 
% %                             & \multirow{3}{*}{Gaussian} & ERM   & 1.14   & 1.04 & 1.04 & 1.03 & 1.02 \\
% %                             &                           & IG    & 2.03   & 1.69 & 1.60 & 1.56 & 1.53 \\
% %                             &                           & EEM   & 2.03   & 2.53 & 2.82 & 3.05 & 3.14 \\ \cline{2-8} 
% %                             & \multirow{3}{*}{Exp.}     & ERM   & 1.39   & 1.15 & 1.13 & 1.09 & 1.10 \\
% %                             &                           & IG    & 1.67   & 1.42 & 1.38 & 1.33 & 1.32 \\
% %                             &                           & EEM   & 1.67   & 2.08 & 2.31 & 2.63 & 2.83 \\
% %\bottomrule
% %\end{tabular}
% %\end{adjustbox}
% %\caption{The Bayesian approximation ratio of ERM, IG, and EEM in the balanced case, i.e. $q_1=q_2$. Every row contains the results for different mechanism, measure $\mu$, and vector $\vec q$.  Every column contains the results for different $n\in \{10,20,\ldots,50\}$. Every value is computed as the average of $500$ runs.}
% %\label{table:equicapacitated_test}
% %\end{table}


% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}

% \begin{table*}[ht]
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{c|c|c|ccc|ccc|ccc|ccc|ccc}
% \toprule
% \multirow{2}{*}{p.c.v. $\vec{q}$} & \multirow{2}{*}{Measure $\mu$} & \multirow{2}{*}{Mech.} & \multicolumn{3}{c|}{$n=10$} & \multicolumn{3}{c|}{20} & \multicolumn{3}{c|}{30} & \multicolumn{3}{c|}{40} & \multicolumn{3}{c}{50} \\
%                                   &                                &                        & lb      & mean    & ub     & lb     & mean  & ub    & lb     & mean  & ub    & lb     & mean  & ub    & lb     & mean  & ub    \\
% \hline                                 
% \multirow{4}{*}{$(0.85,0.75)$}    & \multirow{2}{*}{Uniform}       & ERM                    & 1.15    & 1.17    & 1.20   & 1.04   & 1.05  & 1.05  & 1.03   & 1.04  & 1.04  & 1.02   & 1.02  & 1.03  & 1.02   & 1.02  & 1.02  \\
%                                   &                                & EEM                    & 1.75    & 1.79    & 1.82   & 1.89   & 1.92  & 1.95  & 1.90   & 1.92  & 1.94  & 1.93   & 1.95  & 1.97  & 1.96   & 1.97  & 1.99  \\ \cline{2-18} 
%                                   & \multirow{2}{*}{Gaussian}      & ERM                    & 1.14    & 1.16    & 1.18   & 1.04   & 1.05  & 1.05  & 1.03   & 1.04  & 1.04  & 1.02   & 1.03  & 1.03  & 1.02   & 1.02  & 1.03  \\
%                                   &                                & EEM                    & 1.99    & 2.02    & 2.06   & 2.48   & 2.53  & 2.58  & 2.75   & 2.80  & 2.84  & 3.01   & 3.06  & 3.11  & 3.15   & 3.20  & 3.24  \\ \hline \hline
% \multirow{4}{*}{$(0.8,0.4)$}      & \multirow{2}{*}{Uniform}       & ERM                    & 2.09    & 2.17    & 2.24   & 1.85   & 1.89  & 1.93  & 1.78   & 1.82  & 1.85  & 1.74   & 1.76  & 1.78  & 1.71   & 1.73  & 1.76  \\
%                                   &                                & EEM                    & 1.89    & 1.95    & 2.00   & 2.10   & 2.14  & 2.18  & 2.21   & 2.25  & 2.28  & 2.23   & 2.27  & 2.30  & 2.26   & 2.29  & 2.32  \\ \cline{2-18}
%                                   & \multirow{2}{*}{Gaussian}      & ERM                    & 1.77    & 1.82    & 1.87   & 1.59   & 1.62  & 1.64  & 1.53   & 1.55  & 1.57  & 1.51   & 1.52  & 1.54  & 1.49   & 1.51  & 1.52  \\
%                                   &                                & EEM                    & 2.10    & 2.14    & 2.19   & 2.63   & 2.68  & 2.73  & 2.88   & 2.93  & 2.98  & 3.11   & 3.16  & 3.21  & 3.26   & 3.31  & 3.35  \\ \hline \hline
% \multirow{4}{*}{$(0.85,0.35)$}    & \multirow{2}{*}{Uniform}       & ERM                    & 2.10    & 2.17    & 2.24   & 1.96   & 2.00  & 2.03  & 1.86   & 1.89  & 1.92  & 1.85   & 1.87  & 1.89  & 1.82   & 1.85  & 1.87  \\
%                                   &                                & EEM                    & 1.88    & 1.93    & 1.97   & 2.25   & 2.30  & 2.35  & 2.34   & 2.38  & 2.42  & 2.42   & 2.46  & 2.49  & 2.46   & 2.50  & 2.53  \\ \cline{2-18}
%                                   & \multirow{2}{*}{Gaussian}      & ERM                    & 1.78    & 1.83    & 1.88   & 1.69   & 1.71  & 1.74  & 1.60   & 1.62  & 1.64  & 1.59   & 1.61  & 1.62  & 1.55   & 1.57  & 1.58  \\
%                                   &                                & EEM                    & 2.11    & 2.16    & 2.21   & 2.68   & 2.73  & 2.78  & 2.96   & 3.01  & 3.06  & 3.17   & 3.22  & 3.27  & 3.33   & 3.38  & 3.43 \\
% \bottomrule                                 
% \end{tabular}
% }
% \caption{The Bayesian approximation ratio of ERM and EEM in the unbalanced case, i.e. $q_1\neq q_2$.
% % 
% Every row contains the results for different mechanism, measure $\mu$, and vector $\vec q$.
% %
% Every column contains the results for different $n\in \{10,20,\ldots,50\}$.
% %
% %
% Every value is computed as the average of $500$ runs.}
% \label{table:nonequitest}
% \end{table*}

% %\begin{table}[ht]
% %\centering
% %\begin{adjustbox}{max width=\columnwidth}
% %\begin{tabular}{c|c|c|ccccc}
% %\toprule
% %p.c.v. $\vec{q}$               & Measure $\mu$             & Mech. & $n=10$ & 20   & 30   & 40   & 50   \\ \hline
% %\multirow{4}{*}{$(0.85,0.75)$} & \multirow{2}{*}{Uniform}  & ERM   & 1.17   & 1.05 & 1.04 & 1.02 & 1.02 \\
% %                               &                           & EEM   & 1.79   & 1.92 & 1.92 & 1.95 & 1.97 \\ \cline{2-8} 
% %                               & \multirow{2}{*}{Guassian} & ERM   & 1.16   & 1.05 & 1.04 & 1.03 & 1.02 \\
% %                               &                           & EEM   & 2.02   & 2.53 & 2.80 & 3.06 & 3.20 \\ \hline \hline
% %\multirow{4}{*}{$(0.8,0.4)$}   & \multirow{2}{*}{Uniform}  & ERM   & 2.17   & 1.89 & 1.82 & 1.76 & 1.73 \\
% %                               &                           & EEM   & 1.95   & 2.14 & 2.25 & 2.27 & 2.29 \\ \cline{2-8} 
% %                               & \multirow{2}{*}{Gaussian} & ERM   & 1.82   & 1.62 & 1.55 & 1.52 & 1.51 \\
% %                               &                           & EEM   & 2.14   & 2.68 & 2.93 & 3.16 & 3.31 \\ \hline \hline
% %\multirow{4}{*}{$(0.85,0.35)$} & \multirow{2}{*}{Uniform}  & ERM   & 2.17   & 2.00 & 1.89 & 1.87 & 1.85 \\
% %                               &                           & EEM   & 1.93   & 2.30 & 2.38 & 2.46 & 2.50 \\ \cline{2-8} 
% %                               & \multirow{2}{*}{Gaussian} & ERM   & 1.83   & 1.71 & 1.62 & 1.61 & 1.57 \\
% %                               &                           & EEM   & 2.16   & 2.73 & 3.01 & 3.22 & 3.38 \\ 
% %\bottomrule
% %\end{tabular}
% %\end{adjustbox}
% %\caption{The Bayesian approximation ratio of ERM and EEM in the unbalanced case, i.e. $q_1\neq q_2$. Every row contains the results for different mechanism, measure $\mu$, and vector $\vec q$. Every column contains the results for different $n\in \{10,20,\ldots,50\}$. Every value is computed as the average of $500$ runs.}
% %\label{table:nonequitest}
% %\end{table}

% \begin{table*}[h]
% \centering
% \begin{tabular}{c|c|ccccc}
% \toprule
% p.c.v. $\vec{q}$             & Measure $\mu$   & $n=10$ & 20   & 30   & 40   & 50   \\ \hline
% \multirow{2}{*}{$(0.7,0.7)$} & Uniform     &  0.10  & 0.06   & 0.04  & 0.03  & 0.02  \\
%                              & Gaussian &  0.10   & 0.05 & 0.03 & 0.03 & 0.03 \\
%                              % & Exponential &    &   &   &   &   \\
%                             \hline
% \multirow{2}{*}{$(0.8,0.8)$} & Uniform     & 0.18   & 0.05 & 0.04 & 0.02 & 0.02 \\
%                              & Gaussian    & 0.15   & 0.04 & 0.04 & 0.02 & 0.02 \\
%                              % & Exponential &    &  &  &  &  \\
%                              \hline
% \multirow{2}{*}{$(0.9,0.9)$} & Uniform     & 0.16   & 0.05 & 0.04 & 0.02 & 0.02 \\
%                              & Gaussian    & 0.14   & 0.04 & 0.04 & 0.03 & 0.02 \\
%                              % & Exponential &    &  &  &  &  \\
%                              \hline\hline
% \multirow{2}{*}{$(0.85,0.75)$} & {Uniform}     & 0.17   & 0.05 & 0.04 & 0.02 & 0.02 \\
%                                & {Gaussian}    & 0.16   & 0.05 & 0.04 & 0.03 & 0.02 \\
%                                 \hline
% \multirow{2}{*}{$(0.8,0.4)$}   & {Uniform}  &  0.33  & 0.16   & 0.12  & 0.08  & 0.07\\
%                                & {Gaussian} &  0.28  & 0.14 & 0.09 & 0.07 & 0.06 \\
%                                 \hline
% \multirow{2}{*}{$(0.85,0.35)$} & {Uniform}     &  0.23  & 0.14 & 0.07 & 0.06 & 0.05 \\
%                                & {Gaussian}    &  0.24  & 0.16 & 0.09 & 0.09 & 0.06  \\
% \bottomrule
% \end{tabular}
% \caption{The relative error of ERM. For every row, we compute the relative error of the ERM for different $\vec q$, different probability distributions, while for every column we compute the relative error for different $n\in \{10,20,\dots,50\}$.}
% \label{table:percenterrtest}
% \end{table*}




% % \noindent{Comparison experiments. } We conduct two sets of experiments: (1) when the capacities of two facilities are equal, we compare the performance of ERM, IG and EEM; (2) when the capacities of the two facilities are not equal, then IG cannot be applied and thus we compare the performance of ERM and EEM. For each setup, we change the number of agents from $10$ to $50$. Also, we generate $100$ random location vector $\vec{x}$ drawn from normal, Gaussian and exponential distributions. Then we calculate the average Social Cost of these $100$ runs. The Figures~\ref{fig:EQ} and \ref{fig:NE} show the Bayesian Social Cost of ERM, IG and EEM when $\vec{q}=(0.6,0.6), (0.8,0.8),(0.9,0.9)$ and those of ERM and EEM when $\vec{q}=(0.4,0.8), (0.75,0.85)$, respectively. 


% % \begin{figure}[h]
% %   \centering
% %   \includegraphics[width=0.75\linewidth]{figRE}
% %   \caption{The logo of AAMAS 2024}
% %   \label{fig:logo}
% %   \Description{Logo of AAMAS 2024 -- The 23rd International Conference on Autonomous Agents and Multiagent Systems.}
% % \end{figure}

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.975\columnwidth]{figs/figRE.png}
%     \caption{The relative error of ERM for $n=10,20,\dots,50$ for the Uniform and Gaussian distributions. The first row shows the results for the balanced case while the second row shows the results for unbalanced case. }
%     \label{fig:RE}
% \end{figure}



% \section{Conclusion and Future Works}

% % 
% In this paper, we introduced the Extended Ranking Mechanisms, a generalization of Ranking Mechanisms introduced in \cite{aziz2020facility}.
% %
% After establishing the conditions under which ERMs remain truthful, we characterized the limit Bayesian approximation ratio of truthful ERM in terms of the probability distribution $\mu$, the p.c.v. $\vec q$, and the mechanism's parameters, namely $\pi$ and $\vec v$.
% % examined them from a Bayesian Mechanism Design perspective. 
% % 
% % Specifically, 
% % We characterized the limit of the Bayesian approximation ratio for every truthful ERM in terms of the probability distribution $\mu$, the p.c.v. $\vec q$, and the mechanism's parameters, namely $\pi$ and $\vec v$.
% % 
% % We also delved into the study of optimal ERMs. 
% % % 
% % We have shown that such a mechanism exists and characterized it via a minimization problem, which we solved in two relevant frameworks.
% % 
% We have shown that, given $\mu$ and $\vec q$, there exists an optimal ERM and characterized it via a minimization problem, which we solved in two relevant frameworks.
% % 
% Lastly, we conducted extensive numerical experiments to validate our findings, from which we inferred that a well-tuned ERM consistently outperforms all other known mechanisms.
% % 

% % 


% % 
% For future works, we aim to extend our studies to include other relevant metrics, such as the Maximum Cost or the $l_p$-costs.
% % 
% Another interesting extension would be to extend the ERMs to handle problems in higher dimensions using the decomposition proposed in \cite{auricchio2018computing}.
% % 
% Lastly, we plan to study the connections between the Optimal Transportation problem and other Mechanism Design problems.


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%% The next two lines define, first, the bibliography style to be 
% %%% applied, and, second, the bibliography file to be used.

% % \clearpage

% % \begin{acks}
% %     Gennaro Auricchio and Jie Zhang are partially supported by a Leverhulme Trust Research Project Grant (2021 -- 2024). Jie Zhang is also supported by the EPSRC grant (EP/W014912/1). Mengxiao Zhang is supported by EPSRC Grant (EP/X01357X/1).
% % \end{acks}


% \acks{The authors wish to thank Hans-Martin Adorf, Don Rosenthal, 
% Richard Franier, Peter Cheeseman and Monte Zweben for their assistance
% and advice.  We also thank Ron Musick and our anonymous reviewers for
% their comments.  The Space Telescope Science Institute is operated by
% the Association of Universities for Research in Astronomy for NASA.
% }

% \appendix
% \section*{Appendix A. Probability Distributions for N-Queens}


% [section ommitted]



% \vskip 0.2in
% \bibliography{sample}
% \bibliographystyle{theapa}

% \end{document}
